Candidate high-z proto-clusters among the Planck compact sources, as revealed by Herschel-SPIRE

By determining the nature of all the Planck compact sources within 808.4 deg^2 of large Herschel surveys, we have identified 27 candidate proto-clusters of dusty star forming galaxies (DSFGs) that are at least 3{\sigma} overdense in either 250, 350 or 500 $\mu$mm sources. We find roughly half of all the Planck compact sources are resolved by Herschel into multiple discrete objects, with the other half remaining unresolved by Herschel. We find a significant difference between versions of the Planck catalogues, with earlier releases hosting a larger fraction of candidate proto-clusters and Galactic Cirrus than later releases, which we ascribe to a difference in the filters used in the creation of the three catalogues. We find a surface density of DSFG candidate proto-clusters of (3.3 $\pm$ 0.7) x 10^(-2) sources deg^(-2), in good agreement with previous similar studies. We find that a Planck colour selection of S_{857}/S_{545} < 2 works well to select candidate proto-clusters, but can miss proto-clusters at z < 2. The Herschel colours of individual candidate proto-cluster members indicate our candidate proto-clusters all likely all lie at z > 1. Our candidate proto-clusters are a factor of 5 times brighter at 353 GHz than expected from simulations, even in the most conservative estimates. Further observations are needed to confirm whether these candidate proto-clusters are physical clusters, multiple proto-clusters along the line of sight, or chance alignments of unassociated sources.

==> Discussion/TableSources.tex <==
\begin{tabular}{|l|r|r|l|l|r|r|r|r|r|r|r|}
\hline
  \multicolumn{1}{|c|}{Name} &
  \multicolumn{1}{c|}{RA} &
  \multicolumn{1}{c|}{DEC} &
  \multicolumn{1}{c|}{Field} &
  \multicolumn{1}{c|}{Associations} &
  \multicolumn{1}{c|}{Planck\_Aperflux} &
  \multicolumn{1}{c|}{PlanckAperflux\_err} &
  \multicolumn{1}{c|}{N\_Sources} &
  \multicolumn{1}{c|}{Sum\_Herschel\_Sources} &
  \multicolumn{1}{c|}{Sum\_Herschel\_Sources\_Err} &
  \multicolumn{1}{c|}{Herschel\_Aperture\_Flux} &
  \multicolumn{1}{c|}{Herschel\_Aperture\_Flux\_error} \\
\hline
  PLCKERC857 G261.89-40.69 & 70.1684348814836 & -53.733782579009 & ADFS & (Cluster Candidate) & 794.778381347656 & 133.817794799804 & 22.0 & 899.77174949646 & 27.4542355833619 & 1446.12121017877 & 109.946254031945\\
  PLCKERC857 G060.37+66.55 & 218.578623261217 & 35.5591645712351 & Bootes & (Cluster Candidate) & 1241.43408203125 & 150.806030273437 & 24.0 & 963.561216000000 & 32.7787094320968 & 1414.99830434601 & 108.804046949453\\
  PCCS1 857 G222.56-53.84 & 53.6714840622968 & -27.129584391834 & CDFS & (Cluster Candidate) & 227.254165649414 & 184.522430419921 & 14.0 & 443.169090270996 & 16.7169829445152 & 581.951007315511 & 79.9351738660441\\
  PLCKERC857 G224.76-54.44 & 53.2192774115406 & -28.496873061547 & CDFS & (Cluster Candidate) & 807.061157226562 & 102.111312866210 & 17.0 & 596.270673751831 & 18.1774444944401 & 1284.68376538372 & 101.737453410134\\
  PLCKERC857 G095.44+58.94 & 216.127899349764 & 52.9357383105850 & EGS & (Cluster Candidate) & 1140.99645996093 & 176.373519897460 & 31.0 & 1034.53882789611 & 24.1926829842658 & 0.0 & 0.0\\
  PCCS2 857 G083.61+44.14 & 243.975575403086 & 54.2600270431211 & ELAIS-N1 & (Cluster Candidate) & 457.618072509765 & 190.756927490234 & 14.0 & 474.843969345092 & 20.5921969048933 & 750.202900421666 & 84.0878648688593\\
  PCCS1 857 G085.48+43.36 & 244.656873054259 & 55.7707097121897 & ELAIS-N1 & (Cluster Candidate) & 747.82275390625 & 128.417358398437 & 21.0 & 857.368076324462 & 24.6420335951006 & 1244.38353024333 & 102.557116700892\\
  PCCS1 857 G085.24+46.30 & 239.831238072632 & 54.7117070008195 & ELAIS-N1 & (Cluster Candidate) & 637.029357910156 & 167.762573242187 & 13.0 & 487.209493637084 & 19.9609609707261 & 955.773495385088 & 92.6962503749384\\
  PCCS1 857 G089.66+36.10 & 256.828279626279 & 60.4485740673563 & FLS & (Cluster Candidate) & 886.245056152343 & 194.049926757812 & 16.0 & 584.008153915405 & 25.5229211906784 & 1085.94483351409 & 96.5877876318554\\
  PCCS1 857 G285.70+60.28 & 184.415363859710 & -1.4523076707112 & G12 & (Cluster Candidate) & 462.855682373046 & 185.153610229492 & 11.0 & 413.422209892667 & 27.8400917742740 & 298.654119148850 & 91.7326910900803\\
  PCCS1 857 G279.25+59.97 & 181.268146617031 & -0.7447327265385 & G12 & (Cluster Candidate) & 518.946716308593 & 258.796630859375 & 12.0 & 460.627888432542 & 28.8507629361859 & 435.590729564428 & 92.8945196511507\\
  PCCS1 857 G266.28+58.43 & 174.648193926942 & 0.84139069621084 & G12 & (Cluster Candidate) & 643.172790527343 & 401.66650390625 & 13.0 & 646.730351093645 & 30.2539102596672 & 536.813975308090 & 95.1783817194539\\
  PCCS2 857 G138.41-61.22 & 20.2444762292202 & 0.75995635128703 & Hers & (Cluster Candidate) & 797.49462890625 & 245.823837280273 & 8.0 & 367.063374 & 31.4462025543678 & 940.917037732424 & 250.345469870082\\
  PLCKERC857 G149.81+50.11 & 158.364305340163 & 59.1961427418483 & Lockman & (Cluster Candidate) & 1249.49768066406 & 130.866653442382 & 25.0 & 819.568323135376 & 25.1286761297437 & 1796.25912185700 & 124.273232382758\\
  PCCS1 857 G074.62+80.41 & 201.405917043367 & 33.2403177620437 & NGP & (Cluster Candidate) & 425.062652587890 & 270.2255859375 & 14.0 & 506.771000000000 & 25.1237968866172 & 317.988664492964 & 86.0609199767274\\
  PCCS1 857 G036.04+80.21 & 203.865039914586 & 27.2302707637996 & NGP & (Cluster Candidate) & 118.569610595703 & 473.568908691406 & 6.0 & 245.718000000000 & 16.9347215211824 & 165.301081351935 & 83.6394198371644\\
  PCCS1 857 G058.53+82.57 & 200.606674853476 & 30.1244413052635 & NGP & (Cluster Candidate) & 827.377319335937 & 196.814788818359 & 15.0 & 754.558999999999 & 25.7729264151357 & 571.752951925620 & 89.7923685334506\\
  PCCS1 857 G058.69+81.03 & 202.258204234931 & 30.7118098330279 & NGP & (Cluster Candidate) & 845.204528808593 & 298.120727539062 & 13.0 & 670.377000000000 & 24.2275560674204 & 566.750880433246 & 89.8793952801458\\
  PCCS2 857 G069.76+76.61 & 205.856615569938 & 34.5468536036619 & NGP & (Cluster Candidate) & 571.981628417968 & 296.969787597656 & 10.0 & 431.078000000000 & 21.591075656391 & 272.476363830268 & 85.8619422792169\\
  PLCKERC857 G014.88+80.31 & 202.928757420299 & 23.7713484786122 & NGP & (Cluster Candidate) & 1243.09106445312 & 157.721267700195 & 12.0 & 516.569 & 23.3667059723872 & 138.611399397254 & 84.6033671380594\\
  PLCKERC857 G062.48+78.89 & 204.275873171919 & 32.1419149383755 & NGP & (Cluster Candidate) & 813.656127929687 & 108.920631408691 & 17.0 & 695.464 & 27.3105153191952 & 576.144923573359 & 89.9991954100202\\
  PLCKERC857 G063.13+78.00 & 205.172385360824 & 32.6214161553710 & NGP & (Cluster Candidate) & 912.494750976562 & 168.991821289062 & 20.0 & 785.405 & 27.5005146860926 & 510.955814935267 & 85.0457764642290\\
  PCCS1 857 G029.92+79.80 & 204.218190168989 & 26.1358443272059 & NGP & (Cluster Candidate) & 515.317687988281 & 190.061370849609 & 15.0 & 622.812 & 25.6831019543979 & 421.423761561512 & 87.1450016956933\\
  PLCKERC857 G077.25+80.72 & 200.800839431526 & 33.3866354374969 & NGP & (Cluster Candidate) & 1065.11962890625 & 96.5612106323242 & 12.0 & 466.806 & 23.2324073010095 & 369.313158269971 & 86.7059910001914\\
  PLCKERC857 G102.51+85.22 & 194.813888915784 & 31.5915858538685 & NGP & (Cluster Candidate) & 860.626770019531 & 140.871246337890 & 14.0 & 529.164 & 25.1025373020338 & 297.867936026304 & 85.4867039520186\\
  PCCS1 857 G343.37-84.34 & 8.56772134713321 & -31.364213626808 & SGP & (Cluster Candidate) & 462.691650390625 & 511.874542236328 & 14.0 & 534.262 & 24.9194493719263 & 313.679799452424 & 85.787585890932\\
  PCCS1 857 G354.81-79.56 & 3.04937331448215 & -33.227571429963 & SGP & (Cluster Candidate) & 1013.97845458984 & 233.191314697265 & 15.0 & 648.658999999999 & 23.6574116293393 & 685.061812020372 & 87.9611897868551\\
  PCCS2 857 G020.34-88.13 & 10.8069241805520 & -27.519795365764 & SGP & (Cluster Candidate) & 617.783996582031 & 411.783447265625 & 13.0 & 470.661 & 24.4906809623579 & 390.56982421875 & 87.3961972567843\\
  PCCS1 857 G013.37-62.85 & 342.100004553578 & -32.798138027793 & SGP & (Cluster Candidate) & 392.470092773437 & 246.035812377929 & 17.0 & 694.977999999999 & 28.1479669603330 & 509.303864696994 & 90.3181345744206\\
  PCCS1 857 G293.47-84.07 & 14.0173254265301 & -32.965128419745 & SGP & (Cluster Candidate) & 138.387496948242 & 221.3515625 & 9.0 & 354.462999999999 & 20.4771609848631 & 261.536652263253 & 85.6020589033936\\
  PCCS1 857 G230.86-80.29 & 23.4971317334980 & -29.712345205334 & SGP & (Cluster Candidate) & 424.248901367187 & 211.086730957031 & 12.0 & 555.511 & 23.8262849810875 & 370.594732314348 & 88.0512357400723\\
  PLCKERC857 G239.13-78.19 & 25.3325996784826 & -31.786486966911 & SGP & (Cluster Candidate) & 1109.88854980468 & 144.675369262695 & 12.0 & 531.595 & 24.1569011464633 & 614.709849577397 & 92.2826892937763\\
  PCCS1 857 G004.31-80.79 & 3.40938913945500 & -31.217346341872 & SGP & (Cluster Candidate) & 369.095184326171 & 291.953704833984 & 11.0 & 499.898999999999 & 22.4393074536626 & 423.496916390955 & 87.2215420958672\\
  PLCKERC857 G007.34-65.24 & 345.365628470100 & -35.102732879972 & SGP & (Cluster Candidate) & 920.15185546875 & 132.061950683593 & 22.0 & 942.189 & 31.5033756286528 & 690.228822402656 & 93.4407306613557\\
  PLCKERC857 G014.99-59.64 & 338.259914878371 & -32.138909771451 & SGP & (Cluster Candidate) & 943.417419433593 & 114.829971313476 & 14.0 & 720.271999999999 & 31.0121581319327 & 444.866071820259 & 102.546983659240\\
  PLCKERC857 G017.86-68.67 & 348.789573585237 & -30.591342047164 & SGP & (Cluster Candidate) & 1656.91162109375 & 166.919555664062 & 18.0 & 859.295999999999 & 28.3671052100844 & 650.572136999107 & 92.0556133076051\\
  PLCKERC857 G221.31-79.84 & 24.2726837303431 & -28.146645503413 & SGP & (Cluster Candidate) & 1327.89831542968 & 191.104934692382 & 15.0 & 649.250999999999 & 26.4755862258043 & 436.394314397126 & 88.9708098913028\\
  PLCKERC857 G006.96-67.92 & 348.604194604889 & -34.679349045899 & SGP & (Cluster Candidate) & 939.835998535156 & 106.041282653808 & 13.0 & 604.319 & 24.5305797118616 & 535.391342774848 & 89.8652523553491\\
  PCCS2 857 G170.56-57.15 & 36.5263620515889 & -3.3135133916901 & XMM-LSS & (Cluster Candidate) & 693.299621582031 & 211.362945556640 & 16.0 & 588.790073394775 & 31.4105257037048 & 754.792547393659 & 86.6181983308504\\
  PCCS1 857 G231.57+30.82 & 138.393209730214 & -0.6103902131650 & G09 & (Lens Candidate) & 730.453552246093 & 250.880126953125 & 11.0 & 552.405700971419 & 25.5378631643291 & 636.831004053354 & 96.4000108140599\\
  PCCS1 857 G267.52+59.32 & 175.659242979050 & 1.26395703172685 & G12 & (Lens Candidate) & 333.35791015625 & 447.884979248046 & 14.0 & 576.167865081390 & 31.5898274290949 & 575.221669025719 & 95.6992771640031\\
  PCCS1 857 G151.39-61.73 & 25.9065560505111 & -1.7832754801690 & Hers & (Lens Candidate) & 444.607299804687 & 274.142730712890 & 6.0 & 331.546089 & 27.9245130149842 & 0.0 & 0.0\\
  PCCS1 857 G088.71+81.15 & 198.868921981301 & 34.3137471637601 & NGP & (Lens Candidate) & 427.316253662109 & 158.859924316406 & 8.0 & 375.552 & 17.5663049330244 & 348.603960987180 & 80.6638022374387\\
  PCCS1 857 G044.43+78.90 & 205.288139945378 & 28.7912723173947 & NGP & (Lens Candidate) & 512.08837890625 & 233.325347900390 & 9.0 & 453.138999999999 & 20.5833595168524 & 263.489147886633 & 85.4460184684602\\
  PCCS1 857 G014.92-58.26 & 336.634603878017 & -32.177052768652 & SGP & (Lens Candidate) & 302.219451904296 & 238.781890869140 & 15.0 & 649.511 & 32.2065431706043 & 647.529174804687 & 105.711935328723\\
  PLCKERC857 G013.68-79.70 & 1.61383773976010 & -30.070988993883 & SGP & (Lens Candidate) & 1065.66772460937 & 138.877410888671 & 12.0 & 502.701999999999 & 23.2936389385600 & 360.464415268274 & 86.5260490619429\\
  PCCS2 857 G270.56+58.54 & 176.637264157385 & -0.1871238844100 & G12 & (Lens Candidate) H-ATLAS J114637.9-001132 & 1148.49658203125 & 336.779418945312 & 19.0 & 1010.91637014755 & 33.0927973130105 & 1081.67190504819 & 107.686288050232\\
  PLCKERC857 G047.32+82.53 & 201.116403655163 & 28.7421152976082 & NGP & (Lens Candidate) H-ATLAS J132427.0+284452 & 1302.75158691406 & 151.825454711914 & 13.0 & 822.936 & 24.0045742307586 & 618.663827706128 & 90.5995747895234\\
  PCCS2 857 G148.42+53.62 & 164.478259229056 & 57.5162268747458 & Lockman & (Lens Candidate) HERMES J105751.1+573027 & 223.132980346679 & 382.138488769531 & 3.0 & 99.9673767089843 & 10.816471707919 & 375.665180514807 & 77.4425442727387\\
  PCCS1 857 G076.18+79.96 & 201.638701377592 & 33.7316343557593 & NGP & (Lens Candidate) SDSS J132630.26+334406.5 & 281.641540527343 & 397.424285888671 & 5.0 & 421.102000000000 & 15.9369099890788 & 499.161379085853 & 88.7693940318084\\
  PCCS2 857 G052.27+77.90 & 206.125127624447 & 30.5057926510397 & NGP & (Lens candidate) H-ATLAS J134429.4+303036 & 354.921966552734 & 250.207153320312 & 5.0 & 603.947000000000 & 16.1063874596384 & 296.038993097841 & 86.1852547232845\\
  PCCS1 857 G020.48-64.90 & 344.404523934828 & -29.622178730146 & SGP & (Star) Fomalhaut & 985.878601074218 & 243.609024047851 & 10.0 & 1031.25 & 21.8552913043958 & 1303.41924694553 & 111.649126401067\\
  PLCKERC857 G167.74-57.97 & 34.8362090067661 & -2.9703878665471 & XMM-LSS & (Star) omicron Cet & 4750.98193359375 & 167.368789672851 & 2.0 & 67.0706939697265 & 12.8969897722401 & 4144.01541995469 & 240.301635131066\\
  PCCS1 857 G272.66-83.32 & 16.8561230381995 & -32.834669370213 & SGP & 2MASX J01072341-3249443 & 863.31494140625 & 665.857849121093 & 2.0 & 569.988 & 11.6145700307846 & 608.681347087025 & 91.0762276082970\\
  PCCS2 857 G134.60-61.96 & 18.3181142782606 & 0.41552187569318 & Hers & 2MASX J01131527+00261367 & 963.583618164062 & 315.869659423828 & 5.0 & 365.567135 & 24.0312857162547 & 908.745530835475 & 198.097413112187\\
  PLCKERC857 G138.92-60.96 & 20.5436005594301 & 0.94566373279972 & Hers & 2MASX J01221811+0100262 & 2074.06713867187 & 124.070281982421 & 5.0 & 445.972765000000 & 26.2425590504733 & 2229.91014797876 & 306.823014249871\\
  PCCS1 857 G160.59-56.74 & 32.4316989802617 & 0.28535202533377 & Hers & 2MASX J02094125+0015587 & 876.816711425781 & 374.748352050781 & 6.0 & 1086.888677 & 26.3038321600429 & 0.0 & 0.0\\
  PCCS1 857 G086.97+83.70 & 197.220354540703 & 32.1545173044768 & NGP & 2MASX J13085045+3209540 & 637.67626953125 & 381.957855224609 & 10.0 & 944.216 & 20.0252048678659 & 847.246245654299 & 92.8340649501018\\
  PCCS1 857 G072.04+80.82 & 201.310807573232 & 32.6614073035029 & NGP & 2MASX J13251511+3240167 & 418.416229248046 & 247.248474121093 & 15.0 & 826.081999999999 & 25.7803108592584 & 654.204441413283 & 91.5738648762053\\
  PCCS1 857 G071.93+78.54 & 203.575533002817 & 33.9245576394579 & NGP & 2MASX J13342124+3356185, KUG 1331+342 & 930.659240722656 & 230.435821533203 & 15.0 & 1144.42 & 26.0299638877966 & 884.885873757302 & 97.7619596371343\\
  PCCS1 857 G083.03+45.68 & 241.641837474 & 53.4437181189889 & ELAIS-N1 & 2MASX J16063296+5326319 & 473.348571777343 & 315.501647949218 & 6.0 & 330.607177734375 & 14.3324864851161 & 0.0 & 0.0\\
  PCCS2 857 G006.33-68.95 & 349.882055829536 & -34.655675764801 & SGP & 2MASX J23192682-3437467 & 423.222747802734 & 249.201049804687 & 12.0 & 721.01 & 23.5083502398615 & 459.745987020432 & 88.4127789561701\\
  PCCS2 857 G357.79-75.05 & 357.949016147388 & -34.937657950505 & SGP & 2MASX J23514878-3455460, ESO 349- G 002 & 574.001708984375 & 251.914474487304 & 12.0 & 1089.271 & 23.2740241041380 & 849.748092427849 & 96.2168356953409\\
  PCCS1 857 G223.04-78.74 & 25.4919223406917 & -28.535865094082 & SGP & 2MFGC 01281 & 773.984741210937 & 431.003753662109 & 13.0 & 996.291 & 24.9717204653584 & 922.495421789586 & 99.9203800417838\\
  PLCKERC857 G307.24-86.67 & 12.5696185478453 & -30.442452942214 & SGP & AM 0047-304 & 1051.87329101562 & 179.165466308593 & 14.0 & 689.006000000000 & 23.4726295075775 & 678.690033569932 & 88.8841798410574\\
  PCCS1 857 G249.29-87.97 & 14.7131684875383 & -28.317577598159 & SGP & AM 0056-283 NED01, AM 0056-283 NED02 & 260.855255126953 & 392.785827636718 & 8.0 & 756.942000000000 & 19.4367545644842 & 667.758719299919 & 91.9160321220230\\
  PLCKERC857 G219.43-78.58 & 25.7086818779900 & -27.834826297718 & SGP & AM 0140-280 & 870.839477539062 & 123.214431762695 & 10.0 & 845.707999999999 & 22.2189175703948 & 693.177334800362 & 94.3015430564441\\
  PCCS1 857 G225.10-55.12 & 52.4795840522367 & -28.775832693775 & CDFS & AM 0327-285, ESO 418- G 007, ESO 418- G 007, ESO 418- G 007 NOT... & 248.739334106445 & 208.308731079101 & 16.0 & 878.657508850097 & 21.2079237494201 & 518.010783946206 & 78.5447288854368\\
  PLCKERC857 G274.04+60.90 & 179.271482842255 & 1.11529015202508 & G12 & CGCG 013-009, CGCG 013-010 & 1447.92370605468 & 109.531173706054 & 7.0 & 1392.18305519631 & 30.7530350534707 & 1275.42566443979 & 114.259454374811\\
  PLCKERC857 G280.29+58.41 & 181.218059967704 & -2.3966863686975 & G12 & CGCG 013-066, NGC 4079 & 2204.3076171875 & 150.308578491210 & 9.0 & 1993.52163305661 & 42.9761835788149 & 1918.67763031274 & 137.573272085662\\
  PLCKERC857 G281.52+60.68 & 182.564202851404 & -0.4628567506387 & G12 & CGCG 013-092 & 1237.08898925781 & 172.721878051757 & 11.0 & 736.495680093332 & 30.1730106220774 & 971.245700221508 & 97.3255922655497\\
  PCCS2 857 G341.22+56.12 & 213.069615022859 & -0.6166269626344 & G15 & CGCG 018-077 & 1027.3701171875 & 337.719696044921 & 8.0 & 1028.90517938856 & 32.9069157624958 & 733.389260105788 & 98.2815066452568\\
  PCCS1 857 G344.28+57.82 & 213.471801967380 & 1.73050250121489 & G15 & CGCG 018-084 & 628.426879882812 & 406.575164794921 & 14.0 & 979.318337655350 & 31.3033578550289 & 698.605921268463 & 97.4333745083826\\
  PCCS1 857 G223.97+26.09 & 130.926044902151 & 2.71985845575213 & G09 & CGCG 033-001 & 545.821960449218 & 347.284912109375 & 12.0 & 529.952219569392 & 34.1361459160228 & 663.648432649672 & 97.5138483149604\\
  PLCKERC857 G064.15+86.19 & 196.580098135082 & 29.0510406500537 & NGP & CGCG 160-137, NGC 4966 & 1157.83447265625 & 135.161956787109 & 13.0 & 909.458000000000 & 23.2734576288096 & 897.855321289971 & 95.3116328400021\\
  PLCKERC857 G066.56+83.87 & 198.766633334953 & 30.3937118592013 & NGP & CGCG 160-170 & 1056.26574707031 & 151.803619384765 & 12.0 & 688.026999999999 & 23.2841590786525 & 608.686684107407 & 90.5485613667076\\
  PCCS1 857 G060.81+67.75 & 217.103258712337 & 35.4213738941845 & Bootes & CGCG 192-027, (Lens Candidate) 1HERMES S250 J142823.9+352619 & 423.940582275390 & 322.944183349609 & 16.0 & 790.113745000000 & 28.9741132549040 & 612.041186040830 & 83.1690097114804\\
  PCCS1 857 G085.81+43.85 & 243.701672333028 & 55.8589217997059 & ELAIS-N1 & CGCG 276-004 & 649.75439453125 & 160.351165771484 & 23.0 & 985.832632064819 & 27.6163864469844 & 987.075545147148 & 93.7162248260152\\
  PCCS1 857 G137.65-62.31 & 19.6391958025167 & -0.2216171597411 & Hers & CGCG 385-062, CGCG 385-062 NED02, CGCG 385-062 NED01, CGCG 385-062 & 996.777221679687 & 383.822601318359 & 13.0 & 988.185705 & 37.3448112305081 & 1013.62113008767 & 194.718878268745\\
  PLCKERC857 G227.75+30.24 & 136.179655197674 & 1.88570212238121 & G09 & Cirrus & 3524.02270507812 & 481.571807861328 & 10.0 & 418.345890474140 & 26.4245917470828 & 1632.46246170438 & 121.052432854548\\
  PLCKERC857 G230.55+31.91 & 138.859161181136 & 0.71063895586971 & G09 & Cirrus & 1216.17211914062 & 86.2462310791015 & 12.0 & 408.110031920610 & 29.0972841172505 & 518.567663013935 & 94.8159716475020\\
  PLCKERC857 G230.97+32.31 & 139.380653184572 & 0.61442335350175 & G09 & Cirrus & 1538.84948730468 & 280.215454101562 & 11.0 & 372.742478086749 & 27.8096769308814 & 642.498311955481 & 96.6365362633428\\
  PLCKERC857 G224.33+24.38 & 129.582759448063 & 1.60154142072681 & G09 & Cirrus & 2927.81787109375 & 420.526519775390 & 10.0 & 321.815566397199 & 26.8306707892292 & 906.580778969451 & 103.186839934831\\
  PLCKERC857 G226.70+24.89 & 131.101463051832 & -0.0134782872889 & G09 & Cirrus & 2089.59326171875 & 194.145675659179 & 16.0 & 600.858610044109 & 33.2196498325915 & 914.499256052076 & 103.240223794730\\
  PLCKERC857 G224.73+23.79 & 129.253141018362 & 0.99826253091120 & G09 & Cirrus & 2289.181640625 & 293.210601806640 & 7.0 & 250.126194157978 & 22.7602137292249 & 845.598898362368 & 93.8036058016530\\
  PLCKERC857 G224.70+24.60 & 129.939657374357 & 1.41494712471145 & G09 & Cirrus & 2905.30102539062 & 317.491119384765 & 12.0 & 514.819708562076 & 29.0769970595314 & 1358.95917755365 & 117.039267821015\\
  PLCKERC857 G227.26+24.72 & 131.206420178363 & -0.5401599562316 & G09 & Cirrus & 3180.07421875 & 438.260192871093 & 11.0 & 402.316002675122 & 28.0507195807879 & 353.996468603611 & 92.1546918951948\\
  PLCKERC857 G231.43+32.10 & 139.413140397474 & 0.17253483082052 & G09 & Cirrus & 2806.98608398437 & 430.055297851562 & 22.0 & 1091.73559138323 & 38.7372402088739 & 2024.77513520419 & 143.076686398045\\
  PLCKERC857 G231.25+32.05 & 139.284387413411 & 0.27936612708333 & G09 & Cirrus & 1803.81701660156 & 324.198852539062 & 18.0 & 801.765759552377 & 35.2705068718894 & 983.527135234326 & 105.589874474187\\
  PLCKERC857 G223.40+22.96 & 127.934743506943 & 1.65897212615582 & G09 & Cirrus & 2072.2646484375 & 313.929138183593 & 7.0 & 302.839601323701 & 22.8403092360852 & 1580.58239573985 & 124.173415634858\\
  PLCKERC857 G227.24+24.51 & 131.017514475656 & -0.6285590085344 & G09 & Cirrus & 2761.44409179687 & 387.436737060546 & 14.0 & 545.568311788445 & 31.2786627271691 & 1291.97365970164 & 114.776292526539\\
  PLCKERC857 G227.58+24.57 & 131.221615157319 & -0.8629732786220 & G09 & Cirrus & 3135.98217773437 & 276.499237060546 & 14.0 & 561.704294314774 & 31.2942721755914 & 1171.83295615017 & 110.848475130270\\
  PCCS1 857 G228.60+29.58 & 135.998343119109 & 0.91941706859254 & G09 & Cirrus & 1416.72924804687 & 348.369537353515 & 11.0 & 500.466487361500 & 27.8435634572875 & 1080.55251239985 & 107.363893310964\\
  PLCKERC857 G231.38+32.24 & 139.510716665112 & 0.29073886648945 & G09 & Cirrus & 2476.7802734375 & 435.253173828125 & 14.0 & 662.826274813091 & 31.3688691699270 & 715.762972310185 & 98.3508044943910\\
  PLCKERC857 G226.98+26.25 & 132.398090008380 & 0.45408257654530 & G09 & Cirrus & 2374.84057617187 & 314.941253662109 & 11.0 & 388.240989431286 & 28.0510354889084 & 789.273822724819 & 100.239025228224\\
  PCCS1 857 G229.23+33.59 & 139.709545513751 & 2.53175514992687 & G09 & Cirrus & 1991.06958007812 & 529.965637207031 & 10.0 & 523.353916606831 & 26.7977630782869 & 817.316073268652 & 100.473824456024\\
  PCCS1 857 G223.82+24.63 & 129.579873128244 & 2.12713729057284 & G09 & Cirrus & 1621.90588378906 & 281.697967529296 & 19.0 & 682.721323971046 & 36.2552006476312 & 1017.09207443543 & 106.197206816995\\
  PCCS1 857 G223.74+24.66 & 129.571664548357 & 2.21268764388471 & G09 & Cirrus & 2091.0771484375 & 653.86181640625 & 15.0 & 584.942877614741 & 32.4077166273713 & 648.254490874707 & 97.2702951723070\\
  PLCKERC857 G287.82+60.54 & 185.490855832826 & -1.4633556888992 & G12 & Cirrus & 2124.11547851562 & 240.490280151367 & 21.0 & 813.084348213294 & 38.0032395329661 & 1136.26018620654 & 109.701399370732\\
  PLCKERC857 G266.26+58.99 & 174.940419047252 & 1.32315295245128 & G12 & Cirrus & 1276.52734375 & 210.749481201171 & 7.0 & 294.888644140841 & 22.7770810245738 & 858.509387068159 & 101.657188541085\\
  PLCKERC857 G145.33-60.97 & 23.5128697885885 & 0.02797639265208 & Hers & Cirrus & 1786.02038574218 & 279.638031005859 & 6.0 & 212.624355 & 25.8175463604356 & 1746.44748767151 & 208.108435138366\\
  PCCS1 857 G140.38-62.74 & 20.7561574532986 & -0.9484795624538 & Hers & Cirrus & 1380.42956542968 & 439.614807128906 & 5.0 & 230.145131000000 & 25.9925224115220 & 1586.03578825626 & 284.185999811612\\
  PCCS1 857 G141.28-60.26 & 21.8478371892435 & 1.31798404968516 & Hers & Cirrus & 564.728393554687 & 359.986389160156 & 7.0 & 271.120782 & 30.6052238293885 & 758.571779368304 & 272.412423305197\\
  PLCKERC857 G131.56-63.86 & 16.6503188801177 & -1.2508628434371 & Hers & Cirrus & 5437.56982421875 & 921.43408203125 & 7.0 & 316.086111 & 30.4841485027304 & 5684.18044071702 & 392.651468899876\\
  PLCKERC857 G131.96-63.35 & 16.8980826910407 & -0.7699274161102 & Hers & Cirrus & 1666.37048339843 & 252.126296997070 & 7.0 & 261.492943999999 & 27.8697053131740 & 2401.51370204209 & 210.661632628424\\
  PLCKERC857 G147.26-60.62 & 24.5212805422662 & 0.02202021911053 & Hers & Cirrus & 2196.2099609375 & 238.062850952148 & 6.0 & 216.393456 & 27.2897494120710 & 2365.69141292755 & 274.687911686870\\
  PLCKERC857 G159.09-55.91 & 32.1745226275860 & 1.43251425081342 & Hers & Cirrus & 1421.85925292968 & 239.953887939453 & 6.0 & 245.788192 & 27.6875728838716 & 1683.21028167525 & 242.262893816285\\
  PLCKERC857 G126.90-63.28 & 14.6441511293538 & -0.4731449337870 & Hers & Cirrus & 2763.31958007812 & 313.402984619140 & 7.0 & 289.980094 & 30.2115027998976 & 3299.90019250149 & 300.999445943673\\
  PCCS1 857 G131.85-64.10 & 16.7445047385371 & -1.5066174993653 & Hers & Cirrus & 3258.68432617187 & 1192.36193847656 & 5.0 & 177.797310000000 & 25.9572619793168 & 3036.26554164495 & 287.906690521892\\
  PCCS1 857 G134.53-63.43 & 18.0206095907507 & -1.0261153442415 & Hers & Cirrus & 1365.24145507812 & 1889.2744140625 & 5.0 & 214.598454 & 25.7302047046475 & 2703.86267628822 & 295.904628435929\\
  PCCS1 857 G139.80-62.24 & 20.6273929810562 & -0.3952720312431 & Hers & Cirrus & 1591.7841796875 & 939.885559082031 & 8.0 & 334.030247000000 & 29.5002922431565 & 1860.77831082035 & 210.158441592147\\
  PCCS1 857 G131.08-64.08 & 16.4153650608363 & -1.4355434627805 & Hers & Cirrus & 2187.85986328125 & 709.384643554687 & 2.0 & 66.748936 & 17.2908057063601 & 2242.82815803262 & 272.012567568843\\
  PCCS1 857 G138.16-60.62 & 20.2649389102910 & 1.36719000969500 & Hers & Cirrus & 599.984985351562 & 374.305389404296 & 3.0 & 156.121123 & 20.5392510139575 & 894.424730372116 & 284.295000047518\\
  PCCS2 857 G156.60-56.71 & 30.5807707045216 & 1.44842232436700 & Hers & Cirrus & 1032.77673339843 & 291.753723144531 & 4.0 & 166.243735 & 23.4403419500933 & 971.733525199924 & 259.443466883904\\
  PLCKERC857 G144.37-59.70 & 23.4879030806208 & 1.38545681042065 & Hers & Cirrus & 1752.78564453125 & 125.069389343261 & 8.0 & 358.347463999999 & 32.0821753619069 & 1785.94783668991 & 285.536420273113\\
  PLCKERC857 G136.06-63.48 & 18.6815036443119 & -1.2099822138134 & Hers & Cirrus & 5602.98095703125 & 394.982391357421 & 2.0 & 75.326728 & 17.1492520983913 & 5922.61718791017 & 418.531297384643\\
  PLCKERC857 G126.80-63.90 & 14.5637617879550 & -1.0799868095037 & Hers & Cirrus & 2996.52099609375 & 368.950042724609 & 3.0 & 236.521842 & 22.0977225394533 & 0.0 & 0.0\\
  PLCKERC857 G139.61-62.17 & 20.5624752363463 & -0.3024679405608 & Hers & Cirrus & 3444.69384765625 & 362.984588623046 & 5.0 & 184.742298999999 & 23.6756217383465 & 3502.88013334571 & 267.277734137966\\
  PLCKERC857 G126.28-63.31 & 14.3632290779309 & -0.4777629150239 & Hers & Cirrus & 4489.302734375 & 469.141906738281 & 5.0 & 232.088767 & 26.3898651031712 & 4585.85670331413 & 342.656651324562\\
  PLCKERC857 G027.36+84.83 & 198.607993457569 & 26.5104362394166 & NGP & Cirrus & 792.045288085937 & 92.8774490356445 & 18.0 & 713.237 & 27.9916507551805 & 531.641102343797 & 88.8705507925571\\
  PLCKERC857 G028.53+83.67 & 199.904651564355 & 26.4676637299920 & NGP & Cirrus & 1300.63244628906 & 166.429031372070 & 15.0 & 653.362000000000 & 23.0741022577260 & 561.500300992280 & 84.1355434552471\\
  PLCKERC857 G042.54+81.51 & 202.358498378794 & 28.2242824603162 & NGP & Cirrus & 1696.83251953125 & 250.724731445312 & 21.0 & 908.614000000000 & 30.4621505314381 & 774.174027331173 & 94.4744272463680\\
  PLCKERC857 G068.89+81.23 & 201.226231152155 & 32.0273782708726 & NGP & Cirrus & 1801.75915527343 & 183.202423095703 & 15.0 & 730.413999999999 & 24.0843374208218 & 662.712449226528 & 88.4056485859136\\
  PLCKERC857 G070.09+80.54 & 201.793800362115 & 32.5549678850692 & NGP & Cirrus & 1692.23193359375 & 239.748992919921 & 17.0 & 804.107 & 25.6673821999829 & 874.781794331967 & 93.9702769345455\\
  PCCS1 857 G338.93-84.48 & 9.06259436327692 & -31.534645390207 & SGP & Cirrus & 400.106872558593 & 243.995239257812 & 12.0 & 507.897 & 23.3465777791949 & 373.124888308346 & 86.8013460914132\\
  PLCKERC857 G259.96-87.61 & 14.7168690416016 & -28.862360957095 & SGP & Cirrus & 2320.04956054687 & 329.410980224609 & 11.0 & 414.666000000000 & 22.3563063362443 & 597.153843358159 & 90.0497285644507\\
  PLCKERC857 G257.09-87.10 & 15.2326433871961 & -29.122001112221 & SGP & Cirrus & 2403.23876953125 & 197.540161132812 & 20.0 & 768.834999999999 & 26.8914470603573 & 687.103256909176 & 88.0245276041601\\
  PLCKERC857 G244.96-80.43 & 22.4033305237628 & -31.874045845187 & SGP & Cirrus & 1367.16735839843 & 164.618728637695 & 11.0 & 394.432 & 22.2842864817341 & 337.781893581151 & 86.5527685743914\\
  PLCKERC857 G339.76-85.56 & 9.76774975080467 & -30.647834401970 & SGP & Cirrus & 1539.4658203125 & 222.564331054687 & 9.0 & 349.366 & 19.4711149398281 & 387.014883101917 & 84.0197883460426\\
  PLCKERC857 G272.23-87.16 & 14.5254453396206 & -29.559675865773 & SGP & Cirrus & 1843.48547363281 & 323.967590332031 & 12.0 & 493.423000000000 & 23.3542977843479 & 481.799032477661 & 88.6984732635797\\
  PLCKERC857 G251.68-86.96 & 15.5691879246600 & -29.004733564707 & SGP & Cirrus & 2100.56494140625 & 361.756774902343 & 15.0 & 573.502999999999 & 26.1929658496322 & 534.011391016654 & 89.7679113002466\\
  PLCKERC857 G249.60-85.50 & 17.0068013408746 & -29.748817675506 & SGP & Cirrus & 1389.6259765625 & 215.112594604492 & 9.0 & 358.43 & 20.6208024819598 & 350.836610171943 & 86.9078459859943\\
  PCCS1 857 G252.98-85.59 & 16.7490048463562 & -29.909791757096 & SGP & Cirrus & 619.443664550781 & 817.460388183593 & 18.0 & 725.882999999999 & 28.5512217251731 & 561.978132506832 & 90.3266437459935\\
  PCCS1 857 G008.30-68.26 & 348.868278162408 & -34.119278500269 & SGP & Cirrus & 98.7950363159179 & 390.674346923828 & 11.0 & 531.273 & 22.6286095905161 & 453.663319848477 & 88.5139283190477\\
  PLCKERC857 G222.32-80.00 & 24.0736472858123 & -28.311932113875 & SGP & Cirrus & 971.944213867187 & 128.258438110351 & 16.0 & 626.811000000000 & 27.3517343691401 & 475.303364489227 & 89.6232117924126\\
  PCCS1 857 G311.06-73.30 & 9.64026906857268 & -43.622250149622 & ELAIS-S1 & ESO 242- G 021 & 901.016662597656 & 288.038665771484 & 4.0 & 127.673055648803 & 12.0209494845090 & 1083.06154133997 & 97.0903115523812\\
  PCCS1 857 G310.95-73.87 & 9.81662433984342 & -43.064443602454 & ELAIS-S1 & ESO 242- G 023 & 1400.224609375 & 212.262817382812 & 16.0 & 1260.87343978881 & 21.3641032459826 & 1371.25441577290 & 107.119162498042\\
  PCCS1 857 G357.76-75.78 & 358.749271623851 & -34.601801398255 & SGP & ESO 349- G 005 & 542.855346679687 & 284.972991943359 & 9.0 & 864.75 & 19.0759095196008 & 782.488557415083 & 91.1012836891545\\
  PCCS1 857 G356.25-76.69 & 359.916843030254 & -34.480501329200 & SGP & ESO 349- G 015, ESO 349- G 016 & 761.628479003906 & 198.772933959960 & 12.0 & 870.535 & 23.1918573426105 & 637.623988792300 & 91.1280290134258\\
  PCCS1 857 G353.76-79.19 & 2.80890060056760 & -33.594169159213 & SGP & ESO 349- G 038 & 426.270629882812 & 214.080001831054 & 7.0 & 594.800999999999 & 17.1249095764036 & 650.464368466287 & 87.7524608364427\\
  PCCS1 857 G259.62-82.44 & 18.9956285450550 & -32.491105362059 & SGP & ESO 352- G 030 & 821.906127929687 & 421.333312988281 & 15.0 & 866.928000000000 & 26.0055053594426 & 810.538060881197 & 95.6901079257705\\
  PCCS1 857 G254.41-81.05 & 20.8247371016961 & -32.825591793018 & SGP & ESO 352- G 063 & 487.249694824218 & 382.004364013671 & 10.0 & 959.305000000000 & 21.6218806998836 & 851.4086208269 & 97.1372382834257\\
  PCCS1 857 G255.18-80.62 & 21.1383365026818 & -33.184412442048 & SGP & ESO 352- G 071 & 592.479309082031 & 280.899261474609 & 14.0 & 929.917999999999 & 25.1858900180239 & 805.253424663096 & 95.9246850527802\\
  PLCKERC857 G249.83-79.43 & 22.9420292080645 & -33.109223491821 & SGP & ESO 353- G 009 & 2089.44262695312 & 154.972351074218 & 11.0 & 1199.65799999999 & 21.2557896348265 & 1540.96704390272 & 117.375776851970\\
  PLCKERC857 G014.32-65.00 & 344.602243440285 & -32.225314899447 & SGP & ESO 406- G 035 & 1014.15716552734 & 133.250335693359 & 11.0 & 882.600999999999 & 21.2831004790185 & 965.127568503376 & 97.1672419795677\\
  PLCKERC857 G009.50-65.08 & 344.980760746780 & -34.238306888944 & SGP & ESO 406- G 039 & 1309.26721191406 & 107.912231445312 & 14.0 & 1436.70899999999 & 25.4602420844735 & 1221.57544936239 & 108.597081059663\\
  PLCKERC857 G006.28-68.56 & 349.425700838103 & -34.773997056498 & SGP & ESO 407- G 014 & 1297.87512207031 & 112.861938476562 & 13.0 & 959.651 & 24.5644318069846 & 1042.60742305964 & 102.394100182131\\
  PCCS2 857 G010.95-86.53 & 9.20403065873973 & -28.378601933404 & SGP & ESO 410- G 027 & 438.357208251953 & 324.321136474609 & 10.0 & 633.88 & 21.5820399638217 & 556.392204884439 & 89.5656591121211\\
  PLCKERC857 G359.78-81.31 & 4.32363788409928 & -31.616599170889 & SGP & ESO 410-IG 006 & 953.021667480468 & 134.535018920898 & 13.0 & 900.153 & 23.9702718173991 & 910.821553211659 & 97.7954868323968\\
  PCCS1 857 G319.26-85.76 & 11.4669675450997 & -31.190239853059 & SGP & ESO 411- G 010 & 583.370849609375 & 168.530349731445 & 11.0 & 538.439999999999 & 22.4639624064856 & 427.081102829426 & 87.3805448504734\\
  PCCS1 857 G294.36-85.05 & 13.7274947012738 & -32.017353745984 & SGP & ESO 411- G 030, ESO 411- G 029, AM 0052-321 & 654.666870117187 & 287.853363037109 & 13.0 & 1338.55299999999 & 24.1763808085494 & 1065.67277225106 & 102.689610304524\\
  PCCS1 857 G253.13-83.53 & 18.6324097419184 & -31.185540183600 & SGP & ESO 412- G 021 & 1130.83862304687 & 293.395782470703 & 16.0 & 1269.271 & 24.9486713874707 & 1105.37821348011 & 101.136726482969\\
  PLCKERC857 G247.41-81.38 & 21.2116192444459 & -31.758466977377 & SGP & ESO 413- G 004 & 1174.833984375 & 175.572799682617 & 15.0 & 738.338000000000 & 26.2518678764007 & 926.338612549006 & 99.2473307165668\\
  PLCKERC857 G224.07-79.17 & 24.9878396758533 & -28.697467197735 & SGP & ESO 413- G 016 & 1064.91174316406 & 111.796478271484 & 11.0 & 1015.322 & 21.5100301487468 & 955.658854611218 & 97.2971675403396\\
  PCCS1 857 G220.52-79.20 & 24.9989781162361 & -28.030653301097 & SGP & ESO 413- G 018 & 662.473571777343 & 172.401428222656 & 11.0 & 958.031 & 21.5197584094245 & 1077.10445275902 & 101.213009415299\\
  PLCKERC857 G016.48-57.99 & 336.338499556597 & -31.349576301631 & SGP & ESO 467-IG 055, ESO 467-IG 055 NED01, ESO 467-IG 055 NED02 & 1532.98950195312 & 129.553253173828 & 11.0 & 1332.78900000000 & 28.1728373792914 & 1337.79089355468 & 123.861196693311\\
  PLCKERC857 G018.03-66.69 & 346.485228550831 & -30.615730877654 & SGP & ESO 469- G 011 & 1120.31018066406 & 139.212097167968 & 11.0 & 927.794 & 22.6692329601157 & 779.658592231571 & 95.3832445544393\\
  PCCS1 857 G015.37-71.81 & 352.512597343467 & -31.131052004144 & SGP & ESO 470- G 013, (Lens Candidate) 2MASX J23300478-3107468 & 606.292907714843 & 289.868133544921 & 9.0 & 839.265000000000 & 20.6162761428925 & 971.368648294359 & 99.9297571957205\\
  PCCS1 857 G014.42-76.50 & 357.957753441135 & -30.619438550373 & SGP & ESO 471- G 028 & 929.214965820312 & 196.229705810546 & 16.0 & 952.971999999999 & 26.6316835367199 & 829.889602907933 & 95.8506302330647\\
  PCCS2 857 G221.37-54.48 & 52.8300136250143 & -26.557541296191 & CDFS & ESO 482- G 001 & 749.10400390625 & 301.406677246093 & 13.0 & 851.408851623535 & 15.9265388381002 & 1223.14071097725 & 99.5686437236491\\
  PCCS1 857 G354.65+51.85 & 221.871451331813 & 1.03479334236612 & G15 & FGC 1806 & 826.847229003906 & 307.862091064453 & 11.0 & 774.678301932124 & 36.3908705859038 & 546.949372708797 & 94.3745974105001\\
  PCCS1 857 G231.90+31.90 & 139.457021375888 & -0.2665752484655 & G09 & IC 0531 & 722.972534179687 & 196.435684204101 & 8.0 & 745.981689362675 & 31.5694764289812 & 722.920825986191 & 98.6638866600368\\
  PCCS1 857 G140.74+87.22 & 191.881302870995 & 29.767998259321 & NGP & IC 0821 & 730.034423828125 & 156.005798339843 & 13.0 & 672.789999999999 & 24.2224671328087 & 596.392356965690 & 90.3858658743981\\
  PCCS1 857 G002.19+85.13 & 197.459054621257 & 24.5660378797922 & NGP & IC 0854 & 389.026000976562 & 233.040283203125 & 7.0 & 592.286 & 18.3638069582535 & 315.223157592117 & 85.7300822752209\\
  PLCKERC857 G008.90+84.11 & 198.767689469048 & 24.6109648178756 & NGP & IC 0860 & 2051.61767578125 & 156.499725341796 & 17.0 & 2176.09199999999 & 27.2240685607423 & 1778.40766917914 & 128.899423509758\\
  PLCKERC857 G082.93+80.60 & 200.138465827809 & 34.1326495617089 & NGP & IC 0883 & 2553.11547851562 & 147.372756958007 & 13.0 & 2768.33699999999 & 24.2961041938826 & 2200.53513591736 & 147.526156295889\\
  PLCKERC857 G339.69-83.51 & 8.27500254055224 & -32.248959419103 & SGP & IC 1554 & 1159.24291992187 & 103.499389648437 & 9.0 & 1015.744 & 20.4514347907426 & 902.653217393904 & 97.5897751626152\\
  PCCS1 857 G251.82-84.57 & 17.7543899650863 & -30.447848148590 & SGP & IC 1637 & 560.050048828125 & 213.865951538085 & 8.0 & 825.218000000000 & 18.4794991274114 & 1147.90387142077 & 102.673685037733\\
  PLCKERC857 G262.57-82.60 & 18.5368759134403 & -32.645076802388 & SGP & IC 1657, ESO-LV 3520242, ESO-LV 3520241 & 1847.79077148437 & 180.092102050781 & 12.0 & 1579.47100000000 & 21.8413544680727 & 2055.78412442468 & 138.818444706394\\
  PLCKERC857 G225.15-79.05 & 25.0949600620052 & -28.911402828170 & SGP & IC 1720 & 1834.95874023437 & 165.348739624023 & 14.0 & 1224.65099999999 & 25.4161993028068 & 1523.14753797277 & 119.363439189844\\
  PCCS1 857 G057.74+87.73 & 195.192445865713 & 28.0608194332605 & NGP & IC 4040, NGC 4908 GROUP, IC 4051 & 433.958129882812 & 182.404953002929 & 8.0 & 658.779000000000 & 19.3769342260327 & 355.621226198971 & 86.4162182203486\\
  PLCKERC857 G010.62-64.19 & 343.833905212076 & -33.887058683663 & SGP & IC 5262, MCG -06-50-011, v2MCG 79 & 1032.45422363281 & 102.745300292968 & 19.0 & 1442.749 & 29.6793218251360 & 1105.09862317889 & 105.103085439398\\
  PLCKERC857 G010.78-64.76 & 344.509118488156 & -33.744199744195 & SGP & IC 5271 & 3848.01318359375 & 142.237121582031 & 10.0 & 1498.17199999999 & 21.9983926230986 & 3184.78141731768 & 194.816344016697\\
  PCCS2 857 G326.23-88.15 & 12.0285180428906 & -28.816577736818 & SGP & IRAS F00456-2904NE & 69.3863677978515 & 237.743133544921 & 6.0 & 570.857000000000 & 17.1284791502339 & 232.269726552069 & 85.3439966846791\\
  PLCKERC857 G054.78+83.32 & 199.971908515046 & 29.4322246461036 & NGP & KUG 1317+296 & 1212.89880371093 & 136.556198120117 & 22.0 & 956.482 & 28.8100531412213 & 769.806535374838 & 91.0466486298966\\
  PCCS1 857 G071.66+80.96 & 201.211116356620 & 32.5308413113046 & NGP & KUG 1322+328 & 701.956848144531 & 308.087280273437 & 7.0 & 597.538000000000 & 17.4826689038029 & 389.104806978255 & 84.6685412353363\\
  PLCKERC857 G052.87+68.36 & 217.091090944403 & 32.3971234982807 & Bootes & KUG 1426+326 & 1256.8212890625 & 111.902008056640 & 11.0 & 665.392218000000 & 24.5126548976122 & 0.0 & 0.0\\
  PLCKERC857 G059.17+66.46 & 218.821587717897 & 35.1141694022986 & Bootes & KUG 1433+353 & 999.050048828125 & 112.322486877441 & 1.0 & 31.34081 & 9.56506491275566 & 1080.77014154804 & 95.5095439423376\\
  PCCS1 857 G131.83-60.95 & 17.1680924028736 & 1.61878477761794 & Hers & LBQS 0106+0119 (QSO) & 656.981811523437 & 268.581024169921 & 2.0 & 268.89847 & 17.4139748764058 & 536.182421748328 & 281.607528076181\\
  PCCS1 857 G062.57+78.53 & 204.656622204193 & 32.3031755090510 & NGP & MCG +06-30-064 & 786.864685058593 & 402.267303466796 & 13.0 & 733.597999999999 & 23.8605256647878 & 427.519744351506 & 86.3495449340010\\
  PCCS1 857 G054.16+67.86 & 217.596337028036 & 32.9442954237591 & Bootes & MCG +06-32-051, MCG +06-32-052 & 448.324829101562 & 159.483245849609 & 20.0 & 786.463694999999 & 31.8986439174241 & 864.964300992957 & 89.7250737261871\\
  PLCKERC857 G060.85+67.13 & 217.836483999550 & 35.5984667938567 & Bootes & MCG +06-32-056 & 1018.02447509765 & 97.8320007324218 & 20.0 & 1281.47083499999 & 30.1378523650237 & 1500.11328150447 & 111.650951213797\\
  PLCKERC857 G084.40+43.10 & 245.452907293996 & 55.0761637036682 & ELAIS-N1 & MCG +09-27-025, NGC 6143 & 1107.98315429687 & 75.8414001464843 & 20.0 & 1352.86855125427 & 28.6720377338652 & 1530.61241069054 & 113.872179203101\\
  PLCKERC857 G148.24+52.44 & 163.019517517055 & 58.4170168434623 & Lockman & MCG +10-16-015, NGC 3408 & 812.748474121093 & 100.363174438476 & 15.0 & 1077.04426574707 & 19.9762785673165 & 1170.64404656006 & 98.5036424262128\\
  PCCS1 857 G007.78-77.44 & 359.470914708799 & -31.821911524318 & SGP & MCG -05-01-015 & 564.573608398437 & 205.221511840820 & 8.0 & 629.675000000000 & 18.4520890958178 & 624.664761269465 & 87.8875010433274\\
  PCCS2 857 G246.27-80.51 & 22.2023828342556 & -32.028888558919 & SGP & MCG -05-04-040 & 1012.75720214843 & 280.089538574218 & 8.0 & 478.106999999999 & 19.7784275411368 & 526.109308570623 & 90.0612171365974\\
  PCCS1 857 G354.13-78.58 & 2.15246892824209 & -33.870670188418 & SGP & NGC 0010 & 1353.03625488281 & 253.503448486328 & 9.0 & 1078.68600000000 & 20.4276631801094 & 1718.98798428475 & 126.502130613814\\
  PCCS2 857 G349.11-81.94 & 5.97293468755911 & -32.535545419268 & SGP & NGC 0101 & 1108.068359375 & 193.425857543945 & 7.0 & 557.171 & 17.2998637855909 & 885.712110351771 & 94.3682796392042\\
  PLCKERC857 G340.47-81.55 & 6.68854966844275 & -33.685519412121 & SGP & NGC 0115 & 808.839904785156 & 115.255279541015 & 6.0 & 400.085 & 17.1732802341311 & 502.090593338012 & 88.2316810416841\\
  PCCS1 857 G339.08-82.27 & 7.41624539332167 & -33.262161115595 & SGP & NGC 0131 & 853.259948730468 & 308.324645996093 & 9.0 & 721.84 & 18.3816204127927 & 695.082320868969 & 87.2480419049452\\
  PLCKERC857 G338.28-82.37 & 7.59350574437974 & -33.246430660104 & SGP & NGC 0134 & 23886.99609375 & 438.99560546875 & 4.0 & 6594.51999999999 & 14.0592568438022 & 22166.7202058397 & 1221.86812950391\\
  PLCKERC857 G021.83-86.13 & 8.57059168127201 & -27.807161996791 & SGP & NGC 0150 & 4603.91943359375 & 196.872268676757 & 12.0 & 1963.01 & 23.3499538757574 & 4046.70947604626 & 238.021395406862\\
  PLCKERC857 G355.57-86.04 & 9.24847319246857 & -29.481636084623 & SGP & NGC 0174 & 2142.51538085937 & 139.763076782226 & 10.0 & 2616.78500000000 & 21.4720094541707 & 2418.62685773894 & 158.426444321950\\
  PLCKERC857 G299.12-85.91 & 13.1763085456619 & -31.206216061569 & SGP & NGC 0289, NGC 0289 GROUP & 7416.40771484375 & 174.840438842773 & 10.0 & 2200.294 & 21.5259829740711 & 5405.30211170762 & 309.080725412785\\
  PLCKERC857 G256.92-85.55 & 16.5580329350054 & -30.167935091667 & SGP & NGC 0378, MCG -05-03-025 & 1441.38366699218 & 128.914916992187 & 8.0 & 1128.37999999999 & 19.5995675972711 & 1301.10695482976 & 110.826634038644\\
  PLCKERC857 G250.46-84.78 & 17.6410057179953 & -30.221650157385 & SGP & NGC 0418 & 1684.23559570312 & 95.8829650878906 & 8.0 & 735.644999999999 & 19.6494489235703 & 1476.96065269038 & 117.315097838712\\
  PLCKERC857 G239.77-85.12 & 17.8467768148461 & -29.241895635432 & SGP & NGC 0423 & 1707.85534667968 & 150.224136352539 & 11.0 & 994.053 & 22.8298575335020 & 1065.01361269690 & 103.213586807951\\
  PLCKERC857 G134.22-61.41 & 18.2361635993002 & 0.98613435074136 & Hers & NGC 0428 & 2790.7021484375 & 271.175750732421 & 6.0 & 257.016789999999 & 28.2930480290205 & 2731.25250108806 & 310.633087704108\\
  PCCS1 857 G136.33-63.11 & 18.8779315472678 & -0.8755441992453 & Hers & NGC 0450 & 1955.27648925781 & 483.931304931640 & 4.0 & 186.992891 & 22.4072387987886 & 2271.57424124035 & 240.903077996246\\
  PCCS2 857 G140.57-59.63 & 21.6785795513570 & 2.02493097926242 & Hers & NGC 0550 & 822.692016601562 & 351.170135498046 & 2.0 & 98.53915 & 18.8467203459342 & 0.0 & 0.0\\
  PCCS1 857 G144.85-62.07 & 22.9330701375286 & -0.9272412516492 & Hers & NGC 0585 & 1158.87731933593 & 174.675018310546 & 3.0 & 116.637777 & 20.8225058940797 & 1185.41886761290 & 285.296096653679\\
  PLCKERC857 G229.07-80.28 & 23.5807617721431 & -29.418142609395 & SGP & NGC 0613, NGC 0613:[H66] 24, NGC 0613:[H66] 21, NGC 0613:[H66] ... & 17226.9453125 & 296.309600830078 & 15.0 & 7490.69600000000 & 26.5550879682218 & 17809.2718269284 & 983.377234714265\\
  PCCS1 857 G145.82-60.22 & 24.0018254347564 & 0.65465676540581 & Hers & NGC 0622 & 306.889221191406 & 489.028137207031 & 3.0 & 413.663249999999 & 19.2379891713234 & 277.217450600574 & 196.172771694750\\
  PLCKERC857 G230.65-79.17 & 24.7685895908199 & -29.916201238075 & SGP & NGC 0642, NGC 0639 & 2318.5654296875 & 148.755065917968 & 9.0 & 1375.608 & 19.6073004771182 & 2102.04219528846 & 141.488411351611\\
  PCCS2 857 G155.97-57.96 & 29.6708838930100 & 0.52790176854943 & Hers & NGC 0768 & 820.46875 & 198.021316528320 & 6.0 & 445.467765 & 25.8573334317308 & 863.682556941946 & 217.543684509496\\
  PCCS1 857 G157.99-58.08 & 30.5364880665581 & -0.1121919111659 & Hers & NGC 0800 & 420.132843017578 & 205.362091064453 & 2.0 & 94.23938 & 15.9947095707590 & 601.777854915275 & 185.405874312938\\
  PCCS1 857 G163.10-57.02 & 33.4136792271715 & -0.7146535727786 & Hers & NGC 0856 & 266.760559082031 & 265.65625 & 1.0 & 45.116226 & 13.3208611965434 & 310.782994927620 & 273.127459817045\\
  PCCS1 857 G163.48-56.94 & 33.6307562270137 & -0.7670744853426 & Hers & NGC 0863 & 238.080261230468 & 507.716125488281 & 4.0 & 352.929521999999 & 23.4300479689468 & 317.456576319984 & 268.878306711213\\
  PLCKERC857 G172.21-60.84 & 34.6801135807596 & -6.6253924490689 & XMM-LSS & NGC 0881 & 1825.49108886718 & 122.096633911132 & 11.0 & 386.635478973388 & 26.6173040601623 & 2389.55645009676 & 151.796801118875\\
  PLCKERC857 G171.77-59.54 & 35.4016772430094 & -5.5233104190960 & XMM-LSS & NGC 0895, NGC 0894, (Lens Candidate) & 3736.12622070312 & 155.385192871093 & 8.0 & 1861.83509826660 & 22.9032531529100 & 3606.30125771576 & 212.171621473404\\
  PLCKERC857 G263.34-41.83 & 67.9127564553683 & -54.603018497315 & ADFS & NGC 1617 & 2212.97607421875 & 97.7623138427734 & 41.0 & 2237.64892959594 & 47.6477550753039 & 2282.08358712627 & 146.695151012796\\
  PLCKERC857 G152.29+53.37 & 161.354648565173 & 55.9636701901414 & Lockman & NGC 3353 & 1199.67028808593 & 114.464851379394 & 1.0 & 28.2653980255126 & 8.47418419306133 & 1483.32751484699 & 111.612648824432\\
  PLCKERC857 G149.59+53.66 & 163.649537323092 & 56.9861360915470 & Lockman & NGC 3445, UGC 06021 NOTES01 & 846.481140136718 & 92.0180358886718 & 26.0 & 1277.98277664184 & 28.3877611105428 & 663.732986679101 & 83.1732557800218\\
  PLCKERC857 G147.66+53.84 & 165.362512689286 & 57.6769448001829 & Lockman & NGC 3488 & 745.925170898437 & 103.494903564453 & 27.0 & 1070.08061408996 & 31.6991990619363 & 1121.84176304157 & 96.8848061053150\\
  PLCKERC857 G263.84+57.55 & 173.087712357947 & 0.81032791573236 & G12 & NGC 3719, NGC 3720 & 1668.64514160156 & 167.455642700195 & 8.0 & 2019.33179840536 & 48.9845805024397 & 1902.51544921472 & 137.470398970094\\
  PCCS1 857 G272.55+58.08 & 177.349693218894 & -1.0826642836056 & G12 & NGC 3907B & 806.961486816406 & 521.340637207031 & 6.0 & 931.523048686832 & 33.4071813088144 & 549.392504826188 & 93.4688638075056\\
  PLCKERC857 G277.37+59.21 & 180.099652530057 & -1.1042999192051 & G12 & NGC 4030:[BKB2006] 0044, NGC 4030:[BKB2006] 0015, NGC 4030:[BKB... & 16747.423828125 & 286.839813232421 & 6.0 & 13441.8592559782 & 70.2873499287033 & 13165.6176127642 & 729.655094752019\\
  PCCS1 857 G140.19+86.20 & 191.549036502166 & 30.7486620881658 & NGP & NGC 4676:[BFB2004] 1579, NGC 4676:[BFB2004] 1489, NGC 4676:[BFB... & 618.35986328125 & 251.539352416992 & 9.0 & 1041.65999999999 & 20.5307969645603 & 864.631713867187 & 97.0527186905857\\
  PCCS1 857 G125.67+83.96 & 192.514578382354 & 33.1580731424716 & NGP & NGC 4719 & 460.345672607421 & 199.740844726562 & 7.0 & 678.566999999999 & 18.3461109775341 & 838.027941515669 & 96.3285099960032\\
  PLCKERC857 G294.85+88.35 & 192.602889337271 & 25.4967462417664 & NGP & NGC 4725:[BKB2006] 0101, NGC 4725:[BKB2006] 0055, NGC 4725:[BKB... & 11974.1044921875 & 574.252502441406 & 30.0 & 4682.46999999999 & 35.5039329793193 & 11784.8385812537 & 653.583398704991\\
  PCCS1 857 G125.12+88.34 & 192.787362312095 & 28.7810224978455 & NGP & NGC 4738 & 854.051513671875 & 171.858718872070 & 13.0 & 833.026 & 24.2404304829761 & 627.483967952430 & 90.9470459397938\\
  PLCKERC857 G306.37+88.63 & 192.950245666507 & 25.7691288464973 & NGP & NGC 4747 & 1861.85534667968 & 112.518798828125 & 14.0 & 1211.337 & 24.9451262173595 & 1813.92160071816 & 130.472319095478\\
  PLCKERC857 G101.57+88.05 & 193.666835217349 & 28.9330257439814 & NGP & NGC 4793 & 5551.93896484375 & 139.513793945312 & 6.0 & 2827.12400000000 & 17.1341416184178 & 4950.60827536135 & 284.963192287632\\
  PCCS1 857 G070.45+88.15 & 194.517431029173 & 28.2401880699831 & NGP & NGC 4848 & 442.520111083984 & 216.217941284179 & 7.0 & 712.392 & 18.2080799921353 & 604.365868404507 & 90.2951932094782\\
  PLCKERC857 G050.58+87.80 & 195.226503978063 & 27.7747964832464 & NGP & NGC 4911, CGCG 160-092 & 1105.08068847656 & 136.00048828125 & 11.0 & 1022.33100000000 & 22.4197797268394 & 1087.69733406696 & 103.184407441977\\
  PCCS1 857 G052.56+87.66 & 195.343689413168 & 27.8897896680177 & NGP & NGC 4921 & 335.175231933593 & 211.207809448242 & 11.0 & 549.341 & 22.3904199380002 & 551.874540153890 & 89.4956503837944\\
  PLCKERC857 G077.99+86.90 & 195.363439379512 & 29.2952197031420 & NGP & NGC 4922 NED01, NGC 4922, NGC 4922 NED02 & 899.545776367187 & 165.558471679687 & 13.0 & 1201.606 & 24.2010732613245 & 892.43090903759 & 97.4001502756920\\
  PLCKERC857 G044.43+86.76 & 196.445996937615 & 27.7284748656189 & NGP & NGC 4961 & 1366.76794433593 & 134.138381958007 & 9.0 & 882.914 & 20.4451028121650 & 1136.08644527196 & 104.896524678773\\
  PLCKERC857 G057.61+85.56 & 197.459077053683 & 28.9034705609265 & NGP & NGC 5000 & 842.436218261718 & 95.9056549072265 & 7.0 & 678.072000000000 & 17.2155394338951 & 857.121894832700 & 93.1708777745659\\
  PLCKERC857 G063.78+85.05 & 197.737741126354 & 29.5783648444188 & NGP & NGC 5004A & 1246.70739746093 & 132.528488159179 & 13.0 & 1036.12799999999 & 24.1419915085727 & 748.708760075271 & 93.6506751497974\\
  PLCKERC857 G351.34+83.78 & 197.903183993503 & 22.9140126804950 & NGP & NGC 5012, NGC 0134 & 3810.02026367187 & 102.557182312011 & 6.0 & 1372.476 & 17.2700852053485 & 3350.59361596032 & 202.651590694277\\
  PLCKERC857 G001.00+84.43 & 198.030373030302 & 24.0922720664899 & NGP & NGC 5016 & 1676.15661621093 & 101.387626647949 & 8.0 & 900.66 & 19.5072858952751 & 1404.71574965864 & 114.257175509328\\
  PLCKERC857 G079.49+83.41 & 198.186232786109 & 31.8113914273834 & NGP & NGC 5025 & 1053.15600585937 & 168.136657714843 & 3.0 & 490.759 & 13.0249991554702 & 694.380103878676 & 92.3382664197864\\
  PLCKERC857 G041.82+85.07 & 198.362318284588 & 27.7827253495199 & NGP & NGC 5032B, NGC 5032 & 1140.00048828125 & 144.350662231445 & 13.0 & 845.954 & 23.8812950863222 & 968.453263383358 & 99.3658214450918\\
  PLCKERC857 G069.61+83.37 & 199.052151044354 & 30.9483653484049 & NGP & NGC 5056 & 1332.01538085937 & 131.784454345703 & 15.0 & 1074.77099999999 & 23.9824554622749 & 1176.64390429109 & 102.933640329623\\
  PCCS2 857 G069.35+83.06 & 199.375816122975 & 31.0951933774833 & NGP & NGC 5065, KUG 1315+313 & 609.83154296875 & 253.478103637695 & 10.0 & 815.100999999999 & 19.4842427874423 & 662.120057052001 & 86.9014278899493\\
  PLCKERC857 G047.31+83.73 & 199.771776174740 & 28.5148247302206 & NGP & NGC 5081 & 911.583251953125 & 101.254631042480 & 9.0 & 611.944999999999 & 18.4166472790244 & 906.467826068401 & 92.7147817815126\\
  PLCKERC857 G033.44+82.97 & 200.742262848196 & 26.9710403941271 & NGP & NGC 5116 & 1142.25744628906 & 139.358230590820 & 4.0 & 655.307 & 14.6028126400361 & 842.485363230109 & 95.8707718084763\\
  PCCS2 857 G044.42+82.93 & 200.731770907874 & 28.3161945660778 & NGP & NGC 5117 & 408.308654785156 & 174.797882080078 & 4.0 & 363.368999999999 & 14.6643847126294 & 319.283705882728 & 85.7256760874046\\
  PLCKERC857 G066.66+80.62 & 202.057468140362 & 32.0342049600909 & NGP & NGC 5166 & 1051.15100097656 & 134.637496948242 & 9.0 & 995.322 & 20.0306958940522 & 1041.44697900861 & 100.780474521370\\
  PCCS2 857 G060.66+80.72 & 202.448368482774 & 31.1152470074853 & NGP & NGC 5187 & 580.378967285156 & 307.829620361328 & 6.0 & 654.065 & 17.2751506505732 & 482.078260548412 & 88.5060613267043\\
  PLCKERC857 G037.10+79.78 & 204.351157441295 & 27.4034894234444 & NGP & NGC 5251 & 1252.29919433593 & 107.892028808593 & 16.0 & 925.397999999999 & 26.4660907955821 & 952.083275045733 & 99.0305574029495\\
  PLCKERC857 G042.48+79.19 & 204.985658873599 & 28.3966580720038 & NGP & NGC 5263 & 1877.38024902343 & 86.0373229980468 & 7.0 & 1499.19600000000 & 18.4130420897797 & 1611.61146345734 & 122.309836595787\\
  PCCS1 857 G340.43+55.75 & 212.898164354793 & -1.1650571541196 & G15 & NGC 5496 & 983.73779296875 & 239.524444580078 & 3.0 & 1424.56476852264 & 68.3584947318180 & 1275.68915550410 & 114.102873783773\\
  PLCKERC857 G345.11+54.84 & 215.605471948322 & -0.3947757520474 & G15 & NGC 5584 & 3307.64794921875 & 171.290069580078 & 8.0 & 3101.60769375119 & 61.6790750660221 & 3153.20966356247 & 195.253233320259\\
  PCCS1 857 G060.74+67.53 & 217.376446633621 & 35.4546467436147 & Bootes & NGC 5646 & 668.574890136718 & 183.036849975585 & 14.0 & 832.129236999999 & 27.0201866659921 & 906.627299374507 & 90.9748042183923\\
  PLCKERC857 G060.27+67.38 & 217.605805623954 & 35.3187417551870 & Bootes & NGC 5656 & 2720.89672851562 & 145.631637573242 & 4.0 & 141.353697 & 14.8304892636860 & 2506.92093862658 & 157.481942357919\\
  PLCKERC857 G353.15+54.45 & 219.421766216113 & 2.28787325056857 & G15 & NGC 5690 & 5662.47607421875 & 198.444595336914 & 8.0 & 4965.49198255983 & 59.5237762158954 & 4792.05019582435 & 275.761711670228\\
  PCCS1 857 G350.17+52.42 & 219.461757849978 & -0.4057195027531 & G15 & NGC 5691 & 1124.92578125 & 262.660766601562 & 9.0 & 1382.01770272228 & 37.0491963745504 & 1336.76247682794 & 115.710475305091\\
  PLCKERC857 G350.46+51.85 & 219.962370637557 & -0.7158906119272 & G15 & NGC 5705 & 1537.86096191406 & 196.198318481445 & 6.0 & 1213.40908385091 & 50.7172384106232 & 1193.16234938055 & 109.879521758695\\
  PLCKERC857 G351.01+52.11 & 220.048463309301 & -0.2978993522210 & G15 & NGC 5713N, NGC 5713 & 7124.0458984375 & 221.619201660156 & 5.0 & 5927.50410509675 & 49.6585785539618 & 5877.12685440480 & 333.232770812340\\
  PLCKERC857 G351.22+51.97 & 220.237783044837 & -0.3201127758133 & G15 & NGC 5719 & 4001.26391601562 & 226.319671630859 & 6.0 & 4250.84320018934 & 62.9748126634768 & 4107.96398430317 & 240.049840552665\\
  PLCKERC857 G354.50+52.84 & 221.112904935199 & 1.67628153632543 & G15 & NGC 5740 & 2572.92822265625 & 190.299468994140 & 10.0 & 2460.84297155832 & 44.9108649326641 & 2313.26119498536 & 155.517361006198\\
  PLCKERC857 G354.96+52.95 & 221.237369096451 & 1.95137684438106 & G15 & NGC 5746 & 9795.0458984375 & 306.330902099609 & 7.0 & 7912.39920180437 & 94.9723337556785 & 7965.12483840435 & 447.129852048934\\
  PCCS1 857 G352.89+51.17 & 221.541395796973 & -0.2103662434432 & G15 & NGC 5750 & 666.042602539062 & 269.971984863281 & 4.0 & 1127.15255447212 & 39.3982067739129 & 1151.11181932687 & 109.421897164859\\
  PCCS1 857 G088.83+33.68 & 261.815230423427 & 60.0113517970009 & FLS & NGC 6381, UGC 10870 & 1073.61474609375 & 271.151794433593 & 26.0 & 1344.33556938171 & 37.5873110481604 & 0.0 & 0.0\\
  PLCKERC857 G012.07-57.79 & 336.087067446585 & -33.691906720124 & SGP & NGC 7267 & 1783.87756347656 & 87.9193191528320 & 15.0 & 1347.01799999999 & 32.3058844175484 & 1740.88175895460 & 138.459017648000\\
  PLCKERC857 G016.87-58.16 & 336.545213460709 & -31.146405785216 & SGP & NGC 7277 & 881.394714355468 & 148.490325927734 & 17.0 & 1245.539 & 34.2079070245462 & 1334.24789313226 & 123.713690496537\\
  PLCKERC857 G019.30-61.60 & 340.588930318234 & -30.053507544364 & SGP & NGC 7361 & 1925.4658203125 & 88.8556976318359 & 14.0 & 1425.75399999999 & 25.8940750945076 & 2485.01767349056 & 161.685315140218\\
  PLCKERC857 G015.44-75.68 & 356.964592773811 & -30.526925171621 & SGP & NGC 7755 & 3689.736328125 & 233.370544433593 & 7.0 & 1110.139 & 18.3535366346652 & 3312.28879386186 & 200.684006039953\\
  PLCKERC857 G004.50-77.17 & 359.464075879342 & -32.592337073324 & SGP & NGC 7793:[SL2011] 1\_281, NGC 7793:[SL2011] 1\_287, NGC 7793:[SL2... & 26166.84375 & 805.818725585937 & 25.0 & 9907.88299999999 & 29.5776850344985 & 25235.6873729176 & 1390.19138453328\\
  PCCS2 857 G355.71-77.40 & 0.73412938097876 & -34.223387485876 & SGP & NGC 7812 & 1160.02185058593 & 408.530487060546 & 11.0 & 839.154999999999 & 22.3484759211897 & 703.510340888053 & 92.5501494869550\\
  PLCKERC857 G250.12-80.58 & 21.7549765820703 & -32.539854826118 & SGP & R Sculptoris (Star) & 1292.42749023437 & 138.406860351562 & 6.0 & 859.861000000000 & 17.6896151173506 & 932.799807310104 & 99.5010941177961\\
  PCCS1 857 G226.34+23.23 & 129.495973864250 & -0.5597862129496 & G09 & SDSS J083800.68-003306.0 & 1310.97302246093 & 428.808532714843 & 7.0 & 337.860458626905 & 22.8638571330386 & 600.048461422324 & 93.9058314639514\\
  PCCS1 857 G352.22+83.55 & 198.157055876759 & 22.8272048209371 & NGP & SDSS J131244.75+225011.0  , NGC 5012A & 322.246917724609 & 171.129547119140 & 5.0 & 542.397 & 16.0268836022478 & 618.524291992187 & 91.8890177490422\\
  PLCKERC857 G070.52+80.05 & 202.235918449800 & 32.8799517816553 & NGP & SDSS J132856.58+325243.9 (QSO) & 1167.30920410156 & 107.503021240234 & 11.0 & 896.865 & 22.4459876815434 & 766.689904544502 & 94.2439599482282\\
  PCCS1 857 G135.78-62.78 & 18.7009951548446 & -0.4973647717443 & Hers & UGC 00793 NED01, UGC 00793, UGC 00793 NED02 & 822.600463867187 & 261.015502929687 & 6.0 & 826.387954 & 26.0289144395584 & 626.239119278537 & 186.340121024814\\
  PCCS1 857 G223.87+23.88 & 128.947574972689 & 1.72707783184563 & G09 & UGC 04491 & 460.310424804687 & 287.60693359375 & 3.0 & 618.293414791566 & 48.4047353675237 & 746.424740433692 & 91.1496819083550\\
  PCCS1 857 G232.19+31.64 & 139.373076588464 & -0.6125396435184 & G09 & UGC 04915 & 692.891418457031 & 324.422271728515 & 5.0 & 677.756534760980 & 28.1181659608161 & 399.983470439910 & 92.8677036092587\\
  PCCS1 857 G235.51+42.78 & 150.106666455457 & 3.37179453805327 & COSMOS & UGC 05376 & 1885.06298828125 & 222.405456542968 & 10.0 & 408.933950424194 & 22.2409465549474 & 0.0 & 0.0\\
  PCCS2 857 G268.20+56.69 & 174.631973472987 & -1.1746182687715 & G12 & UGC 06608 & 488.679901123046 & 203.882186889648 & 7.0 & 736.700189679599 & 28.3320683325450 & 558.775331504643 & 87.2200074441232\\
  PCCS1 857 G273.25+60.86 & 178.906777416049 & 1.24844038367633 & G12 & UGC 06903 & 1014.74633789062 & 289.599822998046 & 8.0 & 1058.54602351935 & 46.4495524090383 & 1033.98774366825 & 106.427824674143\\
  PLCKERC857 G108.32+88.72 & 193.225021875547 & 28.3621310776161 & NGP & UGC 08017 & 1182.96484375 & 113.775276184082 & 9.0 & 1258.66500000000 & 18.6291303339688 & 1277.47193129174 & 105.497619328243\\
  PLCKERC857 G101.38+83.79 & 195.568046976818 & 32.8726324376840 & NGP & UGC 08145, MCG +06-29-018a NED01, MCG +06-29-018a & 893.258056640625 & 109.484870910644 & 15.0 & 903.839999999999 & 25.6889924870556 & 758.842840090394 & 94.0282900421998\\
  PLCKERC857 G091.96+84.28 & 196.322362373749 & 31.9844249516101 & NGP & UGC 08179 & 890.019348144531 & 106.963211059570 & 9.0 & 979.225000000000 & 19.2268865914375 & 994.029662626562 & 97.2915301777559\\
  PCCS1 857 G049.28+86.01 & 197.201526228748 & 28.1839393874560 & NGP & UGC 08229 & 675.907836914062 & 338.891845703125 & 12.0 & 725.558 & 23.2713021982011 & 702.303684536367 & 92.4545352595463\\
  PCCS1 857 G094.47+81.88 & 197.524373638318 & 34.1854557001729 & NGP & UGC 08246 & 307.831939697265 & 206.298522949218 & 6.0 & 263.247 & 17.1800355063661 & 266.874472052790 & 85.5133549411722\\
  PCCS1 857 G086.19+81.12 & 199.258660720110 & 34.0950902218995 & NGP & UGC 08352 & 377.604248046875 & 248.663497924804 & 6.0 & 619.17 & 17.2997565878829 & 741.293311815708 & 93.6961815379348\\
  PLCKERC857 G038.66+84.14 & 199.434834645880 & 27.5593980336871 & NGP & UGC 08359 & 1217.96118164062 & 114.330879211425 & 9.0 & 667.601000000000 & 20.4147771479386 & 537.295084945857 & 89.0665825074426\\
  PCCS2 857 G006.30+81.88 & 200.753744817426 & 23.2733766448481 & NGP & UGC 08409 & 705.140075683593 & 157.036529541015 & 11.0 & 489.044999999999 & 22.3091556093008 & 369.196545772254 & 86.3128190984996\\
  PCCS1 857 G063.08+80.40 & 202.603221324719 & 31.6086002436900 & NGP & UGC 08498 & 823.222351074218 & 200.907867431640 & 7.0 & 620.741 & 18.3926905590237 & 788.302746254950 & 94.6841548865233\\
  PCCS2 857 G075.02+78.38 & 203.306087647065 & 34.5252202093738 & NGP & UGC 08536, KUG 1330+348 & 528.043823242187 & 294.668212890625 & 10.0 & 831.252 & 21.6518411457316 & 534.419629454612 & 89.7342464326658\\
  PCCS1 857 G072.04+78.37 & 203.734304960647 & 34.0387262533335 & NGP & UGC 08561, UGC 08561 NOTES01 & 1548.82287597656 & 299.448852539062 & 8.0 & 1449.27000000000 & 19.5643642114943 & 1720.00545105338 & 126.859129574826\\
  PLCKERC857 G075.27+77.67 & 203.962418614424 & 34.9887464258486 & NGP & UGC 08583 & 1026.00744628906 & 128.580841064453 & 10.0 & 775.093999999999 & 21.6081609583046 & 784.485368598252 & 95.0334919668415\\
  PCCS1 857 G056.93+78.78 & 204.845116599887 & 31.1782387250064 & NGP & UGC 08640 & 757.146301269531 & 370.537933349609 & 11.0 & 457.650999999999 & 22.3670388294919 & 259.733585409820 & 85.5546024157402\\
  PCCS2 857 G071.87+76.53 & 205.635153296842 & 35.0089885170568 & NGP & UGC 08681 & 767.960754394531 & 194.138015747070 & 13.0 & 821.684000000000 & 24.4178398921771 & 889.267622694373 & 97.9025534811290\\
  PLCKERC857 G051.72+78.22 & 205.793719568156 & 30.3244425688227 & NGP & UGC 08685 & 902.21533203125 & 116.531143188476 & 9.0 & 1259.23299999999 & 20.5057199093326 & 1191.81486433744 & 106.846153432556\\
  PCCS1 857 G065.77+76.25 & 206.772809009284 & 33.8888419818766 & NGP & UGC 08713, UGC 08715 & 964.721740722656 & 495.507751464843 & 12.0 & 854.891000000000 & 23.6181248620630 & 1035.94900245964 & 102.121114123473\\
  PLCKERC857 G347.77+56.35 & 215.864937612484 & 1.71971865546025 & G15 & UGC 09215 & 1220.68469238281 & 146.010574340820 & 8.0 & 1299.05219368744 & 53.420569484048 & 1486.80813708901 & 115.166719431289\\
  PCCS1 857 G347.54+55.75 & 216.144228785254 & 1.17226394138496 & G15 & UGC 09229 NOTES01, UGC 09229 & 888.322509765625 & 238.488723754882 & 9.0 & 859.493151049389 & 33.1276108405058 & 965.385630819946 & 96.8177810409720\\
  PCCS1 857 G089.40+34.18 & 260.750876651798 & 60.4501129209124 & FLS & UGC 10830 & 1319.07495117187 & 480.874847412109 & 29.0 & 1351.36425590515 & 34.2093194245500 & 0.0 & 0.0\\
  PLCKERC857 G055.79+67.45 & 217.965642105878 & 33.6229926031434 & Bootes & VV 775 NED02, VV 775, VV 775 NED01 & 1009.66278076171 & 183.973281860351 & 17.0 & 1089.83042899999 & 27.8966862511142 & 1537.57483552329 & 111.900265881805\\
  PCCS1 857 G238.20+42.27 & 150.845064457020 & 1.46887604778031 & COSMOS & VVDS 100163697, VVDS 100169379, VVDS 100164361 & 711.656005859375 & 268.705413818359 & 22.0 & 807.949884414672 & 31.7744304186396 & 1431.86449345364 & 107.875042943633\\
\hline\end{tabular}


==> FluxComparison/Table_AllSources <==
\begin{longtable}{lllllllll}
\toprule
    Field &                      NAME &        RA &        DEC &      P$_{Flux}$ &        H$_{Flux}$ &     N &    HS$_{Flux}$ \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
   Bootes &  PLCKERC857 G060.37+66.55 &  14:34:19 &  +35:33:33 &  1241 $\pm$ 151 &  1267 $\pm$ 103.0 &  30.0 &  1081 $\pm$ 14 \\
      EGS &  PLCKERC857 G095.44+58.94 &  14:24:31 &  +52:56:09 &  1141 $\pm$ 176 &       0 $\pm$ 0.0 &  29.0 &  1017 $\pm$ 11 \\
  Lockman &  PLCKERC857 G149.81+50.11 &  10:33:27 &  +59:11:46 &  1249 $\pm$ 131 &  1560 $\pm$ 114.0 &  28.0 &   988 $\pm$ 12 \\
      SGP &  PLCKERC857 G007.34-65.24 &  23:01:28 &  -35:06:10 &   920 $\pm$ 132 &    838 $\pm$ 97.0 &  27.0 &  1055 $\pm$ 34 \\
      FLS &   PCCS1 857 G089.66+36.10 &  17:07:19 &  +60:26:55 &   886 $\pm$ 194 &   1019 $\pm$ 94.0 &  27.0 &   859 $\pm$ 13 \\
      SGP &  PLCKERC857 G017.86-68.67 &  23:15:09 &  -30:35:29 &  1657 $\pm$ 167 &    498 $\pm$ 89.0 &  26.0 &  1046 $\pm$ 33 \\
      NGP &  PLCKERC857 G027.36+84.83 &  13:14:26 &  +26:30:38 &    792 $\pm$ 93 &    719 $\pm$ 93.0 &  25.0 &   873 $\pm$ 32 \\
      SGP &  PLCKERC857 G239.13-78.19 &  01:41:20 &  -31:47:11 &  1110 $\pm$ 145 &    678 $\pm$ 94.0 &  24.0 &   802 $\pm$ 32 \\
      NGP &  PLCKERC857 G042.54+81.51 &  13:29:26 &  +28:13:27 &  1697 $\pm$ 251 &    797 $\pm$ 95.0 &  24.0 &   978 $\pm$ 32 \\
      NGP &  PLCKERC857 G063.13+78.00 &  13:40:41 &  +32:37:17 &   912 $\pm$ 169 &    506 $\pm$ 85.0 &  23.0 &   854 $\pm$ 28 \\
   COSMOS &   PCCS1 857 G238.20+42.27 &  10:03:23 &  +01:28:08 &   712 $\pm$ 269 &  1327 $\pm$ 104.0 &  23.0 &    828 $\pm$ 8 \\
      NGP &  PLCKERC857 G068.89+81.23 &  13:24:54 &  +32:01:39 &  1802 $\pm$ 183 &    641 $\pm$ 88.0 &  23.0 &   913 $\pm$ 29 \\
      SGP &  PLCKERC857 G006.96-67.92 &  23:14:25 &  -34:40:46 &   940 $\pm$ 106 &    520 $\pm$ 89.0 &  22.0 &   800 $\pm$ 31 \\
      SGP &   PCCS1 857 G354.81-79.56 &  00:12:12 &  -33:13:39 &  1014 $\pm$ 233 &    644 $\pm$ 87.0 &  22.0 &   812 $\pm$ 27 \\
      NGP &   PCCS1 857 G058.53+82.57 &  13:22:26 &  +30:07:28 &   827 $\pm$ 197 &    554 $\pm$ 89.0 &  22.0 &   910 $\pm$ 30 \\
     ADFS &  PLCKERC857 G261.89-40.69 &  04:40:40 &  -53:44:02 &   795 $\pm$ 134 &  1304 $\pm$ 104.0 &  22.0 &   980 $\pm$ 11 \\
    HELMS &   PCCS1 857 G126.98-59.24 &  00:59:45 &  +03:33:29 &   383 $\pm$ 234 &   648 $\pm$ 304.0 &  21.0 &   685 $\pm$ 29 \\
      NGP &  PLCKERC857 G077.25+80.72 &  13:23:12 &  +33:23:12 &   1065 $\pm$ 97 &    500 $\pm$ 89.0 &  21.0 &   679 $\pm$ 29 \\
      NGP &   PCCS2 857 G029.94+79.79 &  13:36:55 &  +26:08:21 &   467 $\pm$ 258 &    380 $\pm$ 86.0 &  21.0 &   754 $\pm$ 29 \\
      SGP &   PCCS2 857 G013.36-62.85 &  22:48:24 &  -32:47:53 &   175 $\pm$ 281 &    600 $\pm$ 92.0 &  20.0 &   761 $\pm$ 30 \\
      SGP &  PLCKERC857 G222.32-80.00 &  01:36:18 &  -28:18:43 &   972 $\pm$ 128 &    454 $\pm$ 89.0 &  20.0 &   717 $\pm$ 30 \\
      SGP &   PCCS1 857 G018.31-71.34 &  23:27:28 &  -30:15:23 &   749 $\pm$ 360 &    419 $\pm$ 84.0 &  20.0 &   712 $\pm$ 27 \\
  XMM-LSS &   PCCS2 857 G170.56-57.15 &  02:26:06 &  -03:18:49 &   693 $\pm$ 211 &    962 $\pm$ 93.0 &  20.0 &   700 $\pm$ 11 \\
      NGP &  PLCKERC857 G062.48+78.89 &  13:37:06 &  +32:08:31 &   814 $\pm$ 109 &    573 $\pm$ 90.0 &  19.0 &   738 $\pm$ 28 \\
      NGP &  PLCKERC857 G028.53+83.67 &  13:19:37 &  +26:28:04 &  1301 $\pm$ 166 &    678 $\pm$ 87.0 &  19.0 &   743 $\pm$ 25 \\
      SGP &  PLCKERC857 G221.31-79.84 &  01:37:05 &  -28:08:48 &  1328 $\pm$ 191 &    460 $\pm$ 89.0 &  19.0 &   738 $\pm$ 29 \\
      SGP &   PCCS1 857 G001.66-72.03 &  23:36:11 &  -35:11:00 &   392 $\pm$ 305 &    424 $\pm$ 87.0 &  19.0 &   695 $\pm$ 28 \\
    HELMS &   PCCS1 857 G106.67-60.70 &  00:19:56 &  +01:10:02 &   169 $\pm$ 308 &   590 $\pm$ 392.0 &  19.0 &   691 $\pm$ 28 \\
      NGP &   PCCS1 857 G102.56+85.20 &  12:59:16 &  +31:36:37 &   831 $\pm$ 331 &    604 $\pm$ 90.0 &  19.0 &   632 $\pm$ 28 \\
      NGP &   PCCS1 857 G058.69+81.03 &  13:29:02 &  +30:42:43 &   845 $\pm$ 298 &    490 $\pm$ 88.0 &  19.0 &   800 $\pm$ 28 \\
     CDFS &   PCCS1 857 G222.56-53.84 &  03:34:41 &  -27:07:47 &   227 $\pm$ 185 &    814 $\pm$ 86.0 &  18.0 &    612 $\pm$ 6 \\
      SGP &   PCCS1 857 G014.92-58.26 &  22:26:32 &  -32:10:37 &   302 $\pm$ 239 &   679 $\pm$ 106.0 &  18.0 &   717 $\pm$ 34 \\
      NGP &   PCCS2 857 G044.42+78.90 &  13:41:09 &  +28:47:29 &   649 $\pm$ 288 &    382 $\pm$ 87.0 &  18.0 &   655 $\pm$ 27 \\
      NGP &  PLCKERC857 G014.88+80.31 &  13:31:43 &  +23:46:17 &  1243 $\pm$ 158 &     86 $\pm$ 84.0 &  18.0 &   653 $\pm$ 27 \\
    HELMS &   PCCS1 857 G122.50-59.77 &  00:50:35 &  +03:05:39 &   288 $\pm$ 296 &   475 $\pm$ 342.0 &  18.0 &   672 $\pm$ 27 \\
      G09 &   PCCS1 857 G223.82+24.63 &  08:38:19 &  +02:07:38 &  1622 $\pm$ 282 &  1044 $\pm$ 107.0 &  17.0 &   744 $\pm$ 33 \\
      SGP &   PCCS1 857 G008.30-68.26 &  23:15:28 &  -34:07:09 &    99 $\pm$ 391 &    669 $\pm$ 92.0 &  17.0 &   667 $\pm$ 27 \\
    HELMS &   PCCS2 857 G111.24-58.57 &  00:27:08 &  +03:44:57 &   184 $\pm$ 218 &    88 $\pm$ 389.0 &  17.0 &   570 $\pm$ 26 \\
      SGP &   PCCS1 857 G004.31-80.79 &  00:13:38 &  -31:13:02 &   369 $\pm$ 292 &    576 $\pm$ 90.0 &  17.0 &   637 $\pm$ 26 \\
      SGP &   PCCS1 857 G343.37-84.34 &  00:34:16 &  -31:21:51 &   463 $\pm$ 512 &    434 $\pm$ 87.0 &  17.0 &   601 $\pm$ 26 \\
 ELAIS-N1 &   PCCS2 857 G083.61+44.14 &  16:15:54 &  +54:15:36 &   458 $\pm$ 191 &    622 $\pm$ 81.0 &  16.0 &    574 $\pm$ 6 \\
      SGP &   PCCS1 857 G293.47-84.07 &  00:56:04 &  -32:57:54 &   138 $\pm$ 221 &    394 $\pm$ 87.0 &  15.0 &   486 $\pm$ 25 \\
      NGP &   PCCS2 857 G069.76+76.61 &  13:43:26 &  +34:32:49 &   572 $\pm$ 297 &    335 $\pm$ 86.0 &  15.0 &   539 $\pm$ 25 \\
     CDFS &  PLCKERC857 G224.76-54.44 &  03:32:53 &  -28:29:49 &   807 $\pm$ 102 &  1420 $\pm$ 107.0 &  14.0 &    607 $\pm$ 5 \\
      NGP &   PCCS1 857 G074.62+80.41 &  13:25:37 &  +33:14:25 &   425 $\pm$ 270 &    319 $\pm$ 86.0 &  14.0 &   507 $\pm$ 24 \\
      SGP &   PCCS2 857 G007.68-72.90 &  23:37:20 &  -33:10:01 &   669 $\pm$ 277 &    417 $\pm$ 87.0 &  14.0 &   499 $\pm$ 24 \\
      NGP &   PCCS2 857 G006.30+81.88 &  13:23:01 &  +23:16:24 &   705 $\pm$ 157 &    290 $\pm$ 85.0 &  14.0 &   557 $\pm$ 24 \\
      SGP &   PCCS1 857 G230.86-80.29 &  01:34:00 &  -29:42:44 &   424 $\pm$ 211 &    634 $\pm$ 92.0 &  14.0 &   602 $\pm$ 25 \\
      G12 &   PCCS1 857 G266.28+58.43 &  11:38:36 &  +00:50:29 &   643 $\pm$ 402 &    532 $\pm$ 95.0 &  13.0 &   680 $\pm$ 29 \\
      SGP &  PLCKERC857 G339.76-85.56 &  00:39:04 &  -30:38:52 &  1539 $\pm$ 223 &    300 $\pm$ 83.0 &  13.0 &   440 $\pm$ 22 \\
     HERS &   PCCS2 857 G138.41-61.22 &  01:20:59 &  +00:45:36 &   797 $\pm$ 246 &   760 $\pm$ 246.0 &  12.0 &   460 $\pm$ 25 \\
      G12 &   PCCS2 857 G279.25+59.98 &  12:05:04 &  -00:44:28 &   639 $\pm$ 243 &    501 $\pm$ 94.0 &  11.0 &   502 $\pm$ 27 \\
      NGP &   PCCS1 857 G036.04+80.21 &  13:35:28 &  +27:13:49 &   119 $\pm$ 474 &    172 $\pm$ 84.0 &  10.0 &   338 $\pm$ 20 \\
      G09 &  PLCKERC857 G230.55+31.91 &  09:15:26 &  +00:42:38 &   1216 $\pm$ 86 &    560 $\pm$ 95.0 &  10.0 &   397 $\pm$ 26 \\
     HERS &   PCCS1 857 G144.36-59.69 &  01:33:57 &  +01:23:29 &  1368 $\pm$ 207 &  1588 $\pm$ 278.0 &   9.0 &   381 $\pm$ 23 \\
      G09 &   PCCS1 857 G223.97+26.09 &  08:43:42 &  +02:43:11 &   546 $\pm$ 347 &    613 $\pm$ 96.0 &   9.0 &   548 $\pm$ 34 \\
     HERS &   PCCS1 857 G141.28-60.26 &  01:27:23 &  +01:19:05 &   565 $\pm$ 360 &   969 $\pm$ 272.0 &   8.0 &   294 $\pm$ 22 \\
    HELMS &   PCCS1 857 G115.91-56.23 &  00:35:46 &  +06:25:38 &   128 $\pm$ 378 &   543 $\pm$ 370.0 &   8.0 &   301 $\pm$ 18 \\
     HERS &   PCCS2 857 G156.60-56.71 &  02:02:19 &  +01:26:57 &  1033 $\pm$ 292 &  1051 $\pm$ 258.0 &   4.0 &   166 $\pm$ 16 \\
\end{longtable}


==> FluxComparison/Table_AllSourcesLens <==
\begin{tabular}{lllllllll}
\toprule
Field &                      NAME &        RA &        DEC &      P$_{Flux}$ [mJy] &     H$_{Flux}$ [mJy] &     N &    HS$_{Flux}$ [mJy] \\
\midrule
  NGP &  PLCKERC857 G047.32+82.53 &  13:24:28 &  +28:44:32 &  1303 $\pm$ 152 &   617 $\pm$ 90 &  20.0 &   985 $\pm$ 28 \\
  G12 &   PCCS2 857 G270.56+58.54 &  11:46:35 &  -00:11:14 &  1148 $\pm$ 337 &  988 $\pm$ 105 &  19.0 &  1095 $\pm$ 32 \\
  SGP &   PCCS1 857 G013.73-79.69 &  00:06:27 &  -30:03:53 &   724 $\pm$ 202 &   451 $\pm$ 88 &  16.0 &   570 $\pm$ 26 \\
 HERS &   PCCS2 857 G131.83-60.95 &  01:08:41 &  +01:37:03 &   654 $\pm$ 251 &  678 $\pm$ 281 &  16.0 &  1181 $\pm$ 27 \\
  SGP &  PLCKERC857 G014.99-59.64 &  22:33:02 &  -32:08:20 &   943 $\pm$ 115 &  390 $\pm$ 102 &  16.0 &   769 $\pm$ 32 \\
\bottomrule
\end{tabular}


==> FluxComparison/Table_AllSources_Short <==
\begin{tabular}{lllllllll}
\toprule
    Field &                      NAME &        RA &        DEC &      P$_{Flux} [mJy]$ &      H$_{Flux} [mJy]$ &   N &    HS$_{Flux} [mJy]$ \\
\midrule
   Bootes &  PLCKERC857 G060.37+66.55 &  14:34:19 &  +35:33:33 &  1241 $\pm$ 151 &  1267 $\pm$ 103.0 &  30.0 &  1081 $\pm$ 14 \\
      EGS &  PLCKERC857 G095.44+58.94 &  14:24:31 &  +52:56:09 &  1141 $\pm$ 176 &       0 $\pm$ 0.0 &  29.0 &  1017 $\pm$ 11 \\
  Lockman &  PLCKERC857 G149.81+50.11 &  10:33:27 &  +59:11:46 &  1249 $\pm$ 131 &  1560 $\pm$ 114.0 &  28.0 &   988 $\pm$ 12 \\
      SGP &  PLCKERC857 G007.34-65.24 &  23:01:28 &  -35:06:10 &   920 $\pm$ 132 &    838 $\pm$ 97.0 &  27.0 &  1055 $\pm$ 34 \\
      FLS &   PCCS1 857 G089.66+36.10 &  17:07:19 &  +60:26:55 &   886 $\pm$ 194 &   1019 $\pm$ 94.0 &  27.0 &   859 $\pm$ 13 \\
      SGP &  PLCKERC857 G017.86-68.67 &  23:15:09 &  -30:35:29 &  1657 $\pm$ 167 &    498 $\pm$ 89.0 &  26.0 &  1046 $\pm$ 33 \\
      NGP &  PLCKERC857 G027.36+84.83 &  13:14:26 &  +26:30:38 &    792 $\pm$ 93 &    719 $\pm$ 93.0 &  25.0 &   873 $\pm$ 32 \\
      SGP &  PLCKERC857 G239.13-78.19 &  01:41:20 &  -31:47:11 &  1110 $\pm$ 145 &    678 $\pm$ 94.0 &  24.0 &   802 $\pm$ 32 \\
      NGP &  PLCKERC857 G042.54+81.51 &  13:29:26 &  +28:13:27 &  1697 $\pm$ 251 &    797 $\pm$ 95.0 &  24.0 &   978 $\pm$ 32 \\
      NGP &  PLCKERC857 G063.13+78.00 &  13:40:41 &  +32:37:17 &   912 $\pm$ 169 &    506 $\pm$ 85.0 &  23.0 &   854 $\pm$ 28 \\
   COSMOS &   PCCS1 857 G238.20+42.27 &  10:03:23 &  +01:28:08 &   712 $\pm$ 269 &  1327 $\pm$ 104.0 &  23.0 &    828 $\pm$ 8 \\
      NGP &  PLCKERC857 G068.89+81.23 &  13:24:54 &  +32:01:39 &  1802 $\pm$ 183 &    641 $\pm$ 88.0 &  23.0 &   913 $\pm$ 29 \\
      SGP &  PLCKERC857 G006.96-67.92 &  23:14:25 &  -34:40:46 &   940 $\pm$ 106 &    520 $\pm$ 89.0 &  22.0 &   800 $\pm$ 31 \\
      SGP &   PCCS1 857 G354.81-79.56 &  00:12:12 &  -33:13:39 &  1014 $\pm$ 233 &    644 $\pm$ 87.0 &  22.0 &   812 $\pm$ 27 \\
      NGP &   PCCS1 857 G058.53+82.57 &  13:22:26 &  +30:07:28 &   827 $\pm$ 197 &    554 $\pm$ 89.0 &  22.0 &   910 $\pm$ 30 \\
     ADFS &  PLCKERC857 G261.89-40.69 &  04:40:40 &  -53:44:02 &   795 $\pm$ 134 &  1304 $\pm$ 104.0 &  22.0 &   980 $\pm$ 11 \\
    HELMS &   PCCS1 857 G126.98-59.24 &  00:59:45 &  +03:33:29 &   383 $\pm$ 234 &   648 $\pm$ 304.0 &  21.0 &   685 $\pm$ 29 \\
      NGP &  PLCKERC857 G077.25+80.72 &  13:23:12 &  +33:23:12 &   1065 $\pm$ 97 &    500 $\pm$ 89.0 &  21.0 &   679 $\pm$ 29 \\
      NGP &   PCCS2 857 G029.94+79.79 &  13:36:55 &  +26:08:21 &   467 $\pm$ 258 &    380 $\pm$ 86.0 &  21.0 &   754 $\pm$ 29 \\
      SGP &   PCCS2 857 G013.36-62.85 &  22:48:24 &  -32:47:53 &   175 $\pm$ 281 &    600 $\pm$ 92.0 &  20.0 &   761 $\pm$ 30 \\
      SGP &  PLCKERC857 G222.32-80.00 &  01:36:18 &  -28:18:43 &   972 $\pm$ 128 &    454 $\pm$ 89.0 &  20.0 &   717 $\pm$ 30 \\
      SGP &   PCCS1 857 G018.31-71.34 &  23:27:28 &  -30:15:23 &   749 $\pm$ 360 &    419 $\pm$ 84.0 &  20.0 &   712 $\pm$ 27 \\
  XMM-LSS &   PCCS2 857 G170.56-57.15 &  02:26:06 &  -03:18:49 &   693 $\pm$ 211 &    962 $\pm$ 93.0 &  20.0 &   700 $\pm$ 11 \\
      NGP &  PLCKERC857 G062.48+78.89 &  13:37:06 &  +32:08:31 &   814 $\pm$ 109 &    573 $\pm$ 90.0 &  19.0 &   738 $\pm$ 28 \\
      NGP &  PLCKERC857 G028.53+83.67 &  13:19:37 &  +26:28:04 &  1301 $\pm$ 166 &    678 $\pm$ 87.0 &  19.0 &   743 $\pm$ 25 \\
\bottomrule
\end{tabular}


==> Paper_revised_postreferee (copy)/Discussion/TableSources.tex <==
\begin{tabular}{|l|r|r|l|l|r|r|r|r|r|r|r|}
\hline
  \multicolumn{1}{|c|}{Name} &
  \multicolumn{1}{c|}{RA} &
  \multicolumn{1}{c|}{DEC} &
  \multicolumn{1}{c|}{Field} &
  \multicolumn{1}{c|}{Associations} &
  \multicolumn{1}{c|}{Planck\_Aperflux} &
  \multicolumn{1}{c|}{PlanckAperflux\_err} &
  \multicolumn{1}{c|}{N\_Sources} &
  \multicolumn{1}{c|}{Sum\_Herschel\_Sources} &
  \multicolumn{1}{c|}{Sum\_Herschel\_Sources\_Err} &
  \multicolumn{1}{c|}{Herschel\_Aperture\_Flux} &
  \multicolumn{1}{c|}{Herschel\_Aperture\_Flux\_error} \\
\hline
  PLCKERC857 G261.89-40.69 & 70.1684348814836 & -53.733782579009 & ADFS & (Cluster Candidate) & 794.778381347656 & 133.817794799804 & 22.0 & 899.77174949646 & 27.4542355833619 & 1446.12121017877 & 109.946254031945\\
  PLCKERC857 G060.37+66.55 & 218.578623261217 & 35.5591645712351 & Bootes & (Cluster Candidate) & 1241.43408203125 & 150.806030273437 & 24.0 & 963.561216000000 & 32.7787094320968 & 1414.99830434601 & 108.804046949453\\
  PCCS1 857 G222.56-53.84 & 53.6714840622968 & -27.129584391834 & CDFS & (Cluster Candidate) & 227.254165649414 & 184.522430419921 & 14.0 & 443.169090270996 & 16.7169829445152 & 581.951007315511 & 79.9351738660441\\
  PLCKERC857 G224.76-54.44 & 53.2192774115406 & -28.496873061547 & CDFS & (Cluster Candidate) & 807.061157226562 & 102.111312866210 & 17.0 & 596.270673751831 & 18.1774444944401 & 1284.68376538372 & 101.737453410134\\
  PLCKERC857 G095.44+58.94 & 216.127899349764 & 52.9357383105850 & EGS & (Cluster Candidate) & 1140.99645996093 & 176.373519897460 & 31.0 & 1034.53882789611 & 24.1926829842658 & 0.0 & 0.0\\
  PCCS2 857 G083.61+44.14 & 243.975575403086 & 54.2600270431211 & ELAIS-N1 & (Cluster Candidate) & 457.618072509765 & 190.756927490234 & 14.0 & 474.843969345092 & 20.5921969048933 & 750.202900421666 & 84.0878648688593\\
  PCCS1 857 G085.48+43.36 & 244.656873054259 & 55.7707097121897 & ELAIS-N1 & (Cluster Candidate) & 747.82275390625 & 128.417358398437 & 21.0 & 857.368076324462 & 24.6420335951006 & 1244.38353024333 & 102.557116700892\\
  PCCS1 857 G085.24+46.30 & 239.831238072632 & 54.7117070008195 & ELAIS-N1 & (Cluster Candidate) & 637.029357910156 & 167.762573242187 & 13.0 & 487.209493637084 & 19.9609609707261 & 955.773495385088 & 92.6962503749384\\
  PCCS1 857 G089.66+36.10 & 256.828279626279 & 60.4485740673563 & FLS & (Cluster Candidate) & 886.245056152343 & 194.049926757812 & 16.0 & 584.008153915405 & 25.5229211906784 & 1085.94483351409 & 96.5877876318554\\
  PCCS1 857 G285.70+60.28 & 184.415363859710 & -1.4523076707112 & G12 & (Cluster Candidate) & 462.855682373046 & 185.153610229492 & 11.0 & 413.422209892667 & 27.8400917742740 & 298.654119148850 & 91.7326910900803\\
  PCCS1 857 G279.25+59.97 & 181.268146617031 & -0.7447327265385 & G12 & (Cluster Candidate) & 518.946716308593 & 258.796630859375 & 12.0 & 460.627888432542 & 28.8507629361859 & 435.590729564428 & 92.8945196511507\\
  PCCS1 857 G266.28+58.43 & 174.648193926942 & 0.84139069621084 & G12 & (Cluster Candidate) & 643.172790527343 & 401.66650390625 & 13.0 & 646.730351093645 & 30.2539102596672 & 536.813975308090 & 95.1783817194539\\
  PCCS2 857 G138.41-61.22 & 20.2444762292202 & 0.75995635128703 & Hers & (Cluster Candidate) & 797.49462890625 & 245.823837280273 & 8.0 & 367.063374 & 31.4462025543678 & 940.917037732424 & 250.345469870082\\
  PLCKERC857 G149.81+50.11 & 158.364305340163 & 59.1961427418483 & Lockman & (Cluster Candidate) & 1249.49768066406 & 130.866653442382 & 25.0 & 819.568323135376 & 25.1286761297437 & 1796.25912185700 & 124.273232382758\\
  PCCS1 857 G074.62+80.41 & 201.405917043367 & 33.2403177620437 & NGP & (Cluster Candidate) & 425.062652587890 & 270.2255859375 & 14.0 & 506.771000000000 & 25.1237968866172 & 317.988664492964 & 86.0609199767274\\
  PCCS1 857 G036.04+80.21 & 203.865039914586 & 27.2302707637996 & NGP & (Cluster Candidate) & 118.569610595703 & 473.568908691406 & 6.0 & 245.718000000000 & 16.9347215211824 & 165.301081351935 & 83.6394198371644\\
  PCCS1 857 G058.53+82.57 & 200.606674853476 & 30.1244413052635 & NGP & (Cluster Candidate) & 827.377319335937 & 196.814788818359 & 15.0 & 754.558999999999 & 25.7729264151357 & 571.752951925620 & 89.7923685334506\\
  PCCS1 857 G058.69+81.03 & 202.258204234931 & 30.7118098330279 & NGP & (Cluster Candidate) & 845.204528808593 & 298.120727539062 & 13.0 & 670.377000000000 & 24.2275560674204 & 566.750880433246 & 89.8793952801458\\
  PCCS2 857 G069.76+76.61 & 205.856615569938 & 34.5468536036619 & NGP & (Cluster Candidate) & 571.981628417968 & 296.969787597656 & 10.0 & 431.078000000000 & 21.591075656391 & 272.476363830268 & 85.8619422792169\\
  PLCKERC857 G014.88+80.31 & 202.928757420299 & 23.7713484786122 & NGP & (Cluster Candidate) & 1243.09106445312 & 157.721267700195 & 12.0 & 516.569 & 23.3667059723872 & 138.611399397254 & 84.6033671380594\\
  PLCKERC857 G062.48+78.89 & 204.275873171919 & 32.1419149383755 & NGP & (Cluster Candidate) & 813.656127929687 & 108.920631408691 & 17.0 & 695.464 & 27.3105153191952 & 576.144923573359 & 89.9991954100202\\
  PLCKERC857 G063.13+78.00 & 205.172385360824 & 32.6214161553710 & NGP & (Cluster Candidate) & 912.494750976562 & 168.991821289062 & 20.0 & 785.405 & 27.5005146860926 & 510.955814935267 & 85.0457764642290\\
  PCCS1 857 G029.92+79.80 & 204.218190168989 & 26.1358443272059 & NGP & (Cluster Candidate) & 515.317687988281 & 190.061370849609 & 15.0 & 622.812 & 25.6831019543979 & 421.423761561512 & 87.1450016956933\\
  PLCKERC857 G077.25+80.72 & 200.800839431526 & 33.3866354374969 & NGP & (Cluster Candidate) & 1065.11962890625 & 96.5612106323242 & 12.0 & 466.806 & 23.2324073010095 & 369.313158269971 & 86.7059910001914\\
  PLCKERC857 G102.51+85.22 & 194.813888915784 & 31.5915858538685 & NGP & (Cluster Candidate) & 860.626770019531 & 140.871246337890 & 14.0 & 529.164 & 25.1025373020338 & 297.867936026304 & 85.4867039520186\\
  PCCS1 857 G343.37-84.34 & 8.56772134713321 & -31.364213626808 & SGP & (Cluster Candidate) & 462.691650390625 & 511.874542236328 & 14.0 & 534.262 & 24.9194493719263 & 313.679799452424 & 85.787585890932\\
  PCCS1 857 G354.81-79.56 & 3.04937331448215 & -33.227571429963 & SGP & (Cluster Candidate) & 1013.97845458984 & 233.191314697265 & 15.0 & 648.658999999999 & 23.6574116293393 & 685.061812020372 & 87.9611897868551\\
  PCCS2 857 G020.34-88.13 & 10.8069241805520 & -27.519795365764 & SGP & (Cluster Candidate) & 617.783996582031 & 411.783447265625 & 13.0 & 470.661 & 24.4906809623579 & 390.56982421875 & 87.3961972567843\\
  PCCS1 857 G013.37-62.85 & 342.100004553578 & -32.798138027793 & SGP & (Cluster Candidate) & 392.470092773437 & 246.035812377929 & 17.0 & 694.977999999999 & 28.1479669603330 & 509.303864696994 & 90.3181345744206\\
  PCCS1 857 G293.47-84.07 & 14.0173254265301 & -32.965128419745 & SGP & (Cluster Candidate) & 138.387496948242 & 221.3515625 & 9.0 & 354.462999999999 & 20.4771609848631 & 261.536652263253 & 85.6020589033936\\
  PCCS1 857 G230.86-80.29 & 23.4971317334980 & -29.712345205334 & SGP & (Cluster Candidate) & 424.248901367187 & 211.086730957031 & 12.0 & 555.511 & 23.8262849810875 & 370.594732314348 & 88.0512357400723\\
  PLCKERC857 G239.13-78.19 & 25.3325996784826 & -31.786486966911 & SGP & (Cluster Candidate) & 1109.88854980468 & 144.675369262695 & 12.0 & 531.595 & 24.1569011464633 & 614.709849577397 & 92.2826892937763\\
  PCCS1 857 G004.31-80.79 & 3.40938913945500 & -31.217346341872 & SGP & (Cluster Candidate) & 369.095184326171 & 291.953704833984 & 11.0 & 499.898999999999 & 22.4393074536626 & 423.496916390955 & 87.2215420958672\\
  PLCKERC857 G007.34-65.24 & 345.365628470100 & -35.102732879972 & SGP & (Cluster Candidate) & 920.15185546875 & 132.061950683593 & 22.0 & 942.189 & 31.5033756286528 & 690.228822402656 & 93.4407306613557\\
  PLCKERC857 G014.99-59.64 & 338.259914878371 & -32.138909771451 & SGP & (Cluster Candidate) & 943.417419433593 & 114.829971313476 & 14.0 & 720.271999999999 & 31.0121581319327 & 444.866071820259 & 102.546983659240\\
  PLCKERC857 G017.86-68.67 & 348.789573585237 & -30.591342047164 & SGP & (Cluster Candidate) & 1656.91162109375 & 166.919555664062 & 18.0 & 859.295999999999 & 28.3671052100844 & 650.572136999107 & 92.0556133076051\\
  PLCKERC857 G221.31-79.84 & 24.2726837303431 & -28.146645503413 & SGP & (Cluster Candidate) & 1327.89831542968 & 191.104934692382 & 15.0 & 649.250999999999 & 26.4755862258043 & 436.394314397126 & 88.9708098913028\\
  PLCKERC857 G006.96-67.92 & 348.604194604889 & -34.679349045899 & SGP & (Cluster Candidate) & 939.835998535156 & 106.041282653808 & 13.0 & 604.319 & 24.5305797118616 & 535.391342774848 & 89.8652523553491\\
  PCCS2 857 G170.56-57.15 & 36.5263620515889 & -3.3135133916901 & XMM-LSS & (Cluster Candidate) & 693.299621582031 & 211.362945556640 & 16.0 & 588.790073394775 & 31.4105257037048 & 754.792547393659 & 86.6181983308504\\
  PCCS1 857 G231.57+30.82 & 138.393209730214 & -0.6103902131650 & G09 & (Lens Candidate) & 730.453552246093 & 250.880126953125 & 11.0 & 552.405700971419 & 25.5378631643291 & 636.831004053354 & 96.4000108140599\\
  PCCS1 857 G267.52+59.32 & 175.659242979050 & 1.26395703172685 & G12 & (Lens Candidate) & 333.35791015625 & 447.884979248046 & 14.0 & 576.167865081390 & 31.5898274290949 & 575.221669025719 & 95.6992771640031\\
  PCCS1 857 G151.39-61.73 & 25.9065560505111 & -1.7832754801690 & Hers & (Lens Candidate) & 444.607299804687 & 274.142730712890 & 6.0 & 331.546089 & 27.9245130149842 & 0.0 & 0.0\\
  PCCS1 857 G088.71+81.15 & 198.868921981301 & 34.3137471637601 & NGP & (Lens Candidate) & 427.316253662109 & 158.859924316406 & 8.0 & 375.552 & 17.5663049330244 & 348.603960987180 & 80.6638022374387\\
  PCCS1 857 G044.43+78.90 & 205.288139945378 & 28.7912723173947 & NGP & (Lens Candidate) & 512.08837890625 & 233.325347900390 & 9.0 & 453.138999999999 & 20.5833595168524 & 263.489147886633 & 85.4460184684602\\
  PCCS1 857 G014.92-58.26 & 336.634603878017 & -32.177052768652 & SGP & (Lens Candidate) & 302.219451904296 & 238.781890869140 & 15.0 & 649.511 & 32.2065431706043 & 647.529174804687 & 105.711935328723\\
  PLCKERC857 G013.68-79.70 & 1.61383773976010 & -30.070988993883 & SGP & (Lens Candidate) & 1065.66772460937 & 138.877410888671 & 12.0 & 502.701999999999 & 23.2936389385600 & 360.464415268274 & 86.5260490619429\\
  PCCS2 857 G270.56+58.54 & 176.637264157385 & -0.1871238844100 & G12 & (Lens Candidate) H-ATLAS J114637.9-001132 & 1148.49658203125 & 336.779418945312 & 19.0 & 1010.91637014755 & 33.0927973130105 & 1081.67190504819 & 107.686288050232\\
  PLCKERC857 G047.32+82.53 & 201.116403655163 & 28.7421152976082 & NGP & (Lens Candidate) H-ATLAS J132427.0+284452 & 1302.75158691406 & 151.825454711914 & 13.0 & 822.936 & 24.0045742307586 & 618.663827706128 & 90.5995747895234\\
  PCCS2 857 G148.42+53.62 & 164.478259229056 & 57.5162268747458 & Lockman & (Lens Candidate) HERMES J105751.1+573027 & 223.132980346679 & 382.138488769531 & 3.0 & 99.9673767089843 & 10.816471707919 & 375.665180514807 & 77.4425442727387\\
  PCCS1 857 G076.18+79.96 & 201.638701377592 & 33.7316343557593 & NGP & (Lens Candidate) SDSS J132630.26+334406.5 & 281.641540527343 & 397.424285888671 & 5.0 & 421.102000000000 & 15.9369099890788 & 499.161379085853 & 88.7693940318084\\
  PCCS2 857 G052.27+77.90 & 206.125127624447 & 30.5057926510397 & NGP & (Lens candidate) H-ATLAS J134429.4+303036 & 354.921966552734 & 250.207153320312 & 5.0 & 603.947000000000 & 16.1063874596384 & 296.038993097841 & 86.1852547232845\\
  PCCS1 857 G020.48-64.90 & 344.404523934828 & -29.622178730146 & SGP & (Star) Fomalhaut & 985.878601074218 & 243.609024047851 & 10.0 & 1031.25 & 21.8552913043958 & 1303.41924694553 & 111.649126401067\\
  PLCKERC857 G167.74-57.97 & 34.8362090067661 & -2.9703878665471 & XMM-LSS & (Star) omicron Cet & 4750.98193359375 & 167.368789672851 & 2.0 & 67.0706939697265 & 12.8969897722401 & 4144.01541995469 & 240.301635131066\\
  PCCS1 857 G272.66-83.32 & 16.8561230381995 & -32.834669370213 & SGP & 2MASX J01072341-3249443 & 863.31494140625 & 665.857849121093 & 2.0 & 569.988 & 11.6145700307846 & 608.681347087025 & 91.0762276082970\\
  PCCS2 857 G134.60-61.96 & 18.3181142782606 & 0.41552187569318 & Hers & 2MASX J01131527+00261367 & 963.583618164062 & 315.869659423828 & 5.0 & 365.567135 & 24.0312857162547 & 908.745530835475 & 198.097413112187\\
  PLCKERC857 G138.92-60.96 & 20.5436005594301 & 0.94566373279972 & Hers & 2MASX J01221811+0100262 & 2074.06713867187 & 124.070281982421 & 5.0 & 445.972765000000 & 26.2425590504733 & 2229.91014797876 & 306.823014249871\\
  PCCS1 857 G160.59-56.74 & 32.4316989802617 & 0.28535202533377 & Hers & 2MASX J02094125+0015587 & 876.816711425781 & 374.748352050781 & 6.0 & 1086.888677 & 26.3038321600429 & 0.0 & 0.0\\
  PCCS1 857 G086.97+83.70 & 197.220354540703 & 32.1545173044768 & NGP & 2MASX J13085045+3209540 & 637.67626953125 & 381.957855224609 & 10.0 & 944.216 & 20.0252048678659 & 847.246245654299 & 92.8340649501018\\
  PCCS1 857 G072.04+80.82 & 201.310807573232 & 32.6614073035029 & NGP & 2MASX J13251511+3240167 & 418.416229248046 & 247.248474121093 & 15.0 & 826.081999999999 & 25.7803108592584 & 654.204441413283 & 91.5738648762053\\
  PCCS1 857 G071.93+78.54 & 203.575533002817 & 33.9245576394579 & NGP & 2MASX J13342124+3356185, KUG 1331+342 & 930.659240722656 & 230.435821533203 & 15.0 & 1144.42 & 26.0299638877966 & 884.885873757302 & 97.7619596371343\\
  PCCS1 857 G083.03+45.68 & 241.641837474 & 53.4437181189889 & ELAIS-N1 & 2MASX J16063296+5326319 & 473.348571777343 & 315.501647949218 & 6.0 & 330.607177734375 & 14.3324864851161 & 0.0 & 0.0\\
  PCCS2 857 G006.33-68.95 & 349.882055829536 & -34.655675764801 & SGP & 2MASX J23192682-3437467 & 423.222747802734 & 249.201049804687 & 12.0 & 721.01 & 23.5083502398615 & 459.745987020432 & 88.4127789561701\\
  PCCS2 857 G357.79-75.05 & 357.949016147388 & -34.937657950505 & SGP & 2MASX J23514878-3455460, ESO 349- G 002 & 574.001708984375 & 251.914474487304 & 12.0 & 1089.271 & 23.2740241041380 & 849.748092427849 & 96.2168356953409\\
  PCCS1 857 G223.04-78.74 & 25.4919223406917 & -28.535865094082 & SGP & 2MFGC 01281 & 773.984741210937 & 431.003753662109 & 13.0 & 996.291 & 24.9717204653584 & 922.495421789586 & 99.9203800417838\\
  PLCKERC857 G307.24-86.67 & 12.5696185478453 & -30.442452942214 & SGP & AM 0047-304 & 1051.87329101562 & 179.165466308593 & 14.0 & 689.006000000000 & 23.4726295075775 & 678.690033569932 & 88.8841798410574\\
  PCCS1 857 G249.29-87.97 & 14.7131684875383 & -28.317577598159 & SGP & AM 0056-283 NED01, AM 0056-283 NED02 & 260.855255126953 & 392.785827636718 & 8.0 & 756.942000000000 & 19.4367545644842 & 667.758719299919 & 91.9160321220230\\
  PLCKERC857 G219.43-78.58 & 25.7086818779900 & -27.834826297718 & SGP & AM 0140-280 & 870.839477539062 & 123.214431762695 & 10.0 & 845.707999999999 & 22.2189175703948 & 693.177334800362 & 94.3015430564441\\
  PCCS1 857 G225.10-55.12 & 52.4795840522367 & -28.775832693775 & CDFS & AM 0327-285, ESO 418- G 007, ESO 418- G 007, ESO 418- G 007 NOT... & 248.739334106445 & 208.308731079101 & 16.0 & 878.657508850097 & 21.2079237494201 & 518.010783946206 & 78.5447288854368\\
  PLCKERC857 G274.04+60.90 & 179.271482842255 & 1.11529015202508 & G12 & CGCG 013-009, CGCG 013-010 & 1447.92370605468 & 109.531173706054 & 7.0 & 1392.18305519631 & 30.7530350534707 & 1275.42566443979 & 114.259454374811\\
  PLCKERC857 G280.29+58.41 & 181.218059967704 & -2.3966863686975 & G12 & CGCG 013-066, NGC 4079 & 2204.3076171875 & 150.308578491210 & 9.0 & 1993.52163305661 & 42.9761835788149 & 1918.67763031274 & 137.573272085662\\
  PLCKERC857 G281.52+60.68 & 182.564202851404 & -0.4628567506387 & G12 & CGCG 013-092 & 1237.08898925781 & 172.721878051757 & 11.0 & 736.495680093332 & 30.1730106220774 & 971.245700221508 & 97.3255922655497\\
  PCCS2 857 G341.22+56.12 & 213.069615022859 & -0.6166269626344 & G15 & CGCG 018-077 & 1027.3701171875 & 337.719696044921 & 8.0 & 1028.90517938856 & 32.9069157624958 & 733.389260105788 & 98.2815066452568\\
  PCCS1 857 G344.28+57.82 & 213.471801967380 & 1.73050250121489 & G15 & CGCG 018-084 & 628.426879882812 & 406.575164794921 & 14.0 & 979.318337655350 & 31.3033578550289 & 698.605921268463 & 97.4333745083826\\
  PCCS1 857 G223.97+26.09 & 130.926044902151 & 2.71985845575213 & G09 & CGCG 033-001 & 545.821960449218 & 347.284912109375 & 12.0 & 529.952219569392 & 34.1361459160228 & 663.648432649672 & 97.5138483149604\\
  PLCKERC857 G064.15+86.19 & 196.580098135082 & 29.0510406500537 & NGP & CGCG 160-137, NGC 4966 & 1157.83447265625 & 135.161956787109 & 13.0 & 909.458000000000 & 23.2734576288096 & 897.855321289971 & 95.3116328400021\\
  PLCKERC857 G066.56+83.87 & 198.766633334953 & 30.3937118592013 & NGP & CGCG 160-170 & 1056.26574707031 & 151.803619384765 & 12.0 & 688.026999999999 & 23.2841590786525 & 608.686684107407 & 90.5485613667076\\
  PCCS1 857 G060.81+67.75 & 217.103258712337 & 35.4213738941845 & Bootes & CGCG 192-027, (Lens Candidate) 1HERMES S250 J142823.9+352619 & 423.940582275390 & 322.944183349609 & 16.0 & 790.113745000000 & 28.9741132549040 & 612.041186040830 & 83.1690097114804\\
  PCCS1 857 G085.81+43.85 & 243.701672333028 & 55.8589217997059 & ELAIS-N1 & CGCG 276-004 & 649.75439453125 & 160.351165771484 & 23.0 & 985.832632064819 & 27.6163864469844 & 987.075545147148 & 93.7162248260152\\
  PCCS1 857 G137.65-62.31 & 19.6391958025167 & -0.2216171597411 & Hers & CGCG 385-062, CGCG 385-062 NED02, CGCG 385-062 NED01, CGCG 385-062 & 996.777221679687 & 383.822601318359 & 13.0 & 988.185705 & 37.3448112305081 & 1013.62113008767 & 194.718878268745\\
  PLCKERC857 G227.75+30.24 & 136.179655197674 & 1.88570212238121 & G09 & Cirrus & 3524.02270507812 & 481.571807861328 & 10.0 & 418.345890474140 & 26.4245917470828 & 1632.46246170438 & 121.052432854548\\
  PLCKERC857 G230.55+31.91 & 138.859161181136 & 0.71063895586971 & G09 & Cirrus & 1216.17211914062 & 86.2462310791015 & 12.0 & 408.110031920610 & 29.0972841172505 & 518.567663013935 & 94.8159716475020\\
  PLCKERC857 G230.97+32.31 & 139.380653184572 & 0.61442335350175 & G09 & Cirrus & 1538.84948730468 & 280.215454101562 & 11.0 & 372.742478086749 & 27.8096769308814 & 642.498311955481 & 96.6365362633428\\
  PLCKERC857 G224.33+24.38 & 129.582759448063 & 1.60154142072681 & G09 & Cirrus & 2927.81787109375 & 420.526519775390 & 10.0 & 321.815566397199 & 26.8306707892292 & 906.580778969451 & 103.186839934831\\
  PLCKERC857 G226.70+24.89 & 131.101463051832 & -0.0134782872889 & G09 & Cirrus & 2089.59326171875 & 194.145675659179 & 16.0 & 600.858610044109 & 33.2196498325915 & 914.499256052076 & 103.240223794730\\
  PLCKERC857 G224.73+23.79 & 129.253141018362 & 0.99826253091120 & G09 & Cirrus & 2289.181640625 & 293.210601806640 & 7.0 & 250.126194157978 & 22.7602137292249 & 845.598898362368 & 93.8036058016530\\
  PLCKERC857 G224.70+24.60 & 129.939657374357 & 1.41494712471145 & G09 & Cirrus & 2905.30102539062 & 317.491119384765 & 12.0 & 514.819708562076 & 29.0769970595314 & 1358.95917755365 & 117.039267821015\\
  PLCKERC857 G227.26+24.72 & 131.206420178363 & -0.5401599562316 & G09 & Cirrus & 3180.07421875 & 438.260192871093 & 11.0 & 402.316002675122 & 28.0507195807879 & 353.996468603611 & 92.1546918951948\\
  PLCKERC857 G231.43+32.10 & 139.413140397474 & 0.17253483082052 & G09 & Cirrus & 2806.98608398437 & 430.055297851562 & 22.0 & 1091.73559138323 & 38.7372402088739 & 2024.77513520419 & 143.076686398045\\
  PLCKERC857 G231.25+32.05 & 139.284387413411 & 0.27936612708333 & G09 & Cirrus & 1803.81701660156 & 324.198852539062 & 18.0 & 801.765759552377 & 35.2705068718894 & 983.527135234326 & 105.589874474187\\
  PLCKERC857 G223.40+22.96 & 127.934743506943 & 1.65897212615582 & G09 & Cirrus & 2072.2646484375 & 313.929138183593 & 7.0 & 302.839601323701 & 22.8403092360852 & 1580.58239573985 & 124.173415634858\\
  PLCKERC857 G227.24+24.51 & 131.017514475656 & -0.6285590085344 & G09 & Cirrus & 2761.44409179687 & 387.436737060546 & 14.0 & 545.568311788445 & 31.2786627271691 & 1291.97365970164 & 114.776292526539\\
  PLCKERC857 G227.58+24.57 & 131.221615157319 & -0.8629732786220 & G09 & Cirrus & 3135.98217773437 & 276.499237060546 & 14.0 & 561.704294314774 & 31.2942721755914 & 1171.83295615017 & 110.848475130270\\
  PCCS1 857 G228.60+29.58 & 135.998343119109 & 0.91941706859254 & G09 & Cirrus & 1416.72924804687 & 348.369537353515 & 11.0 & 500.466487361500 & 27.8435634572875 & 1080.55251239985 & 107.363893310964\\
  PLCKERC857 G231.38+32.24 & 139.510716665112 & 0.29073886648945 & G09 & Cirrus & 2476.7802734375 & 435.253173828125 & 14.0 & 662.826274813091 & 31.3688691699270 & 715.762972310185 & 98.3508044943910\\
  PLCKERC857 G226.98+26.25 & 132.398090008380 & 0.45408257654530 & G09 & Cirrus & 2374.84057617187 & 314.941253662109 & 11.0 & 388.240989431286 & 28.0510354889084 & 789.273822724819 & 100.239025228224\\
  PCCS1 857 G229.23+33.59 & 139.709545513751 & 2.53175514992687 & G09 & Cirrus & 1991.06958007812 & 529.965637207031 & 10.0 & 523.353916606831 & 26.7977630782869 & 817.316073268652 & 100.473824456024\\
  PCCS1 857 G223.82+24.63 & 129.579873128244 & 2.12713729057284 & G09 & Cirrus & 1621.90588378906 & 281.697967529296 & 19.0 & 682.721323971046 & 36.2552006476312 & 1017.09207443543 & 106.197206816995\\
  PCCS1 857 G223.74+24.66 & 129.571664548357 & 2.21268764388471 & G09 & Cirrus & 2091.0771484375 & 653.86181640625 & 15.0 & 584.942877614741 & 32.4077166273713 & 648.254490874707 & 97.2702951723070\\
  PLCKERC857 G287.82+60.54 & 185.490855832826 & -1.4633556888992 & G12 & Cirrus & 2124.11547851562 & 240.490280151367 & 21.0 & 813.084348213294 & 38.0032395329661 & 1136.26018620654 & 109.701399370732\\
  PLCKERC857 G266.26+58.99 & 174.940419047252 & 1.32315295245128 & G12 & Cirrus & 1276.52734375 & 210.749481201171 & 7.0 & 294.888644140841 & 22.7770810245738 & 858.509387068159 & 101.657188541085\\
  PLCKERC857 G145.33-60.97 & 23.5128697885885 & 0.02797639265208 & Hers & Cirrus & 1786.02038574218 & 279.638031005859 & 6.0 & 212.624355 & 25.8175463604356 & 1746.44748767151 & 208.108435138366\\
  PCCS1 857 G140.38-62.74 & 20.7561574532986 & -0.9484795624538 & Hers & Cirrus & 1380.42956542968 & 439.614807128906 & 5.0 & 230.145131000000 & 25.9925224115220 & 1586.03578825626 & 284.185999811612\\
  PCCS1 857 G141.28-60.26 & 21.8478371892435 & 1.31798404968516 & Hers & Cirrus & 564.728393554687 & 359.986389160156 & 7.0 & 271.120782 & 30.6052238293885 & 758.571779368304 & 272.412423305197\\
  PLCKERC857 G131.56-63.86 & 16.6503188801177 & -1.2508628434371 & Hers & Cirrus & 5437.56982421875 & 921.43408203125 & 7.0 & 316.086111 & 30.4841485027304 & 5684.18044071702 & 392.651468899876\\
  PLCKERC857 G131.96-63.35 & 16.8980826910407 & -0.7699274161102 & Hers & Cirrus & 1666.37048339843 & 252.126296997070 & 7.0 & 261.492943999999 & 27.8697053131740 & 2401.51370204209 & 210.661632628424\\
  PLCKERC857 G147.26-60.62 & 24.5212805422662 & 0.02202021911053 & Hers & Cirrus & 2196.2099609375 & 238.062850952148 & 6.0 & 216.393456 & 27.2897494120710 & 2365.69141292755 & 274.687911686870\\
  PLCKERC857 G159.09-55.91 & 32.1745226275860 & 1.43251425081342 & Hers & Cirrus & 1421.85925292968 & 239.953887939453 & 6.0 & 245.788192 & 27.6875728838716 & 1683.21028167525 & 242.262893816285\\
  PLCKERC857 G126.90-63.28 & 14.6441511293538 & -0.4731449337870 & Hers & Cirrus & 2763.31958007812 & 313.402984619140 & 7.0 & 289.980094 & 30.2115027998976 & 3299.90019250149 & 300.999445943673\\
  PCCS1 857 G131.85-64.10 & 16.7445047385371 & -1.5066174993653 & Hers & Cirrus & 3258.68432617187 & 1192.36193847656 & 5.0 & 177.797310000000 & 25.9572619793168 & 3036.26554164495 & 287.906690521892\\
  PCCS1 857 G134.53-63.43 & 18.0206095907507 & -1.0261153442415 & Hers & Cirrus & 1365.24145507812 & 1889.2744140625 & 5.0 & 214.598454 & 25.7302047046475 & 2703.86267628822 & 295.904628435929\\
  PCCS1 857 G139.80-62.24 & 20.6273929810562 & -0.3952720312431 & Hers & Cirrus & 1591.7841796875 & 939.885559082031 & 8.0 & 334.030247000000 & 29.5002922431565 & 1860.77831082035 & 210.158441592147\\
  PCCS1 857 G131.08-64.08 & 16.4153650608363 & -1.4355434627805 & Hers & Cirrus & 2187.85986328125 & 709.384643554687 & 2.0 & 66.748936 & 17.2908057063601 & 2242.82815803262 & 272.012567568843\\
  PCCS1 857 G138.16-60.62 & 20.2649389102910 & 1.36719000969500 & Hers & Cirrus & 599.984985351562 & 374.305389404296 & 3.0 & 156.121123 & 20.5392510139575 & 894.424730372116 & 284.295000047518\\
  PCCS2 857 G156.60-56.71 & 30.5807707045216 & 1.44842232436700 & Hers & Cirrus & 1032.77673339843 & 291.753723144531 & 4.0 & 166.243735 & 23.4403419500933 & 971.733525199924 & 259.443466883904\\
  PLCKERC857 G144.37-59.70 & 23.4879030806208 & 1.38545681042065 & Hers & Cirrus & 1752.78564453125 & 125.069389343261 & 8.0 & 358.347463999999 & 32.0821753619069 & 1785.94783668991 & 285.536420273113\\
  PLCKERC857 G136.06-63.48 & 18.6815036443119 & -1.2099822138134 & Hers & Cirrus & 5602.98095703125 & 394.982391357421 & 2.0 & 75.326728 & 17.1492520983913 & 5922.61718791017 & 418.531297384643\\
  PLCKERC857 G126.80-63.90 & 14.5637617879550 & -1.0799868095037 & Hers & Cirrus & 2996.52099609375 & 368.950042724609 & 3.0 & 236.521842 & 22.0977225394533 & 0.0 & 0.0\\
  PLCKERC857 G139.61-62.17 & 20.5624752363463 & -0.3024679405608 & Hers & Cirrus & 3444.69384765625 & 362.984588623046 & 5.0 & 184.742298999999 & 23.6756217383465 & 3502.88013334571 & 267.277734137966\\
  PLCKERC857 G126.28-63.31 & 14.3632290779309 & -0.4777629150239 & Hers & Cirrus & 4489.302734375 & 469.141906738281 & 5.0 & 232.088767 & 26.3898651031712 & 4585.85670331413 & 342.656651324562\\
  PLCKERC857 G027.36+84.83 & 198.607993457569 & 26.5104362394166 & NGP & Cirrus & 792.045288085937 & 92.8774490356445 & 18.0 & 713.237 & 27.9916507551805 & 531.641102343797 & 88.8705507925571\\
  PLCKERC857 G028.53+83.67 & 199.904651564355 & 26.4676637299920 & NGP & Cirrus & 1300.63244628906 & 166.429031372070 & 15.0 & 653.362000000000 & 23.0741022577260 & 561.500300992280 & 84.1355434552471\\
  PLCKERC857 G042.54+81.51 & 202.358498378794 & 28.2242824603162 & NGP & Cirrus & 1696.83251953125 & 250.724731445312 & 21.0 & 908.614000000000 & 30.4621505314381 & 774.174027331173 & 94.4744272463680\\
  PLCKERC857 G068.89+81.23 & 201.226231152155 & 32.0273782708726 & NGP & Cirrus & 1801.75915527343 & 183.202423095703 & 15.0 & 730.413999999999 & 24.0843374208218 & 662.712449226528 & 88.4056485859136\\
  PLCKERC857 G070.09+80.54 & 201.793800362115 & 32.5549678850692 & NGP & Cirrus & 1692.23193359375 & 239.748992919921 & 17.0 & 804.107 & 25.6673821999829 & 874.781794331967 & 93.9702769345455\\
  PCCS1 857 G338.93-84.48 & 9.06259436327692 & -31.534645390207 & SGP & Cirrus & 400.106872558593 & 243.995239257812 & 12.0 & 507.897 & 23.3465777791949 & 373.124888308346 & 86.8013460914132\\
  PLCKERC857 G259.96-87.61 & 14.7168690416016 & -28.862360957095 & SGP & Cirrus & 2320.04956054687 & 329.410980224609 & 11.0 & 414.666000000000 & 22.3563063362443 & 597.153843358159 & 90.0497285644507\\
  PLCKERC857 G257.09-87.10 & 15.2326433871961 & -29.122001112221 & SGP & Cirrus & 2403.23876953125 & 197.540161132812 & 20.0 & 768.834999999999 & 26.8914470603573 & 687.103256909176 & 88.0245276041601\\
  PLCKERC857 G244.96-80.43 & 22.4033305237628 & -31.874045845187 & SGP & Cirrus & 1367.16735839843 & 164.618728637695 & 11.0 & 394.432 & 22.2842864817341 & 337.781893581151 & 86.5527685743914\\
  PLCKERC857 G339.76-85.56 & 9.76774975080467 & -30.647834401970 & SGP & Cirrus & 1539.4658203125 & 222.564331054687 & 9.0 & 349.366 & 19.4711149398281 & 387.014883101917 & 84.0197883460426\\
  PLCKERC857 G272.23-87.16 & 14.5254453396206 & -29.559675865773 & SGP & Cirrus & 1843.48547363281 & 323.967590332031 & 12.0 & 493.423000000000 & 23.3542977843479 & 481.799032477661 & 88.6984732635797\\
  PLCKERC857 G251.68-86.96 & 15.5691879246600 & -29.004733564707 & SGP & Cirrus & 2100.56494140625 & 361.756774902343 & 15.0 & 573.502999999999 & 26.1929658496322 & 534.011391016654 & 89.7679113002466\\
  PLCKERC857 G249.60-85.50 & 17.0068013408746 & -29.748817675506 & SGP & Cirrus & 1389.6259765625 & 215.112594604492 & 9.0 & 358.43 & 20.6208024819598 & 350.836610171943 & 86.9078459859943\\
  PCCS1 857 G252.98-85.59 & 16.7490048463562 & -29.909791757096 & SGP & Cirrus & 619.443664550781 & 817.460388183593 & 18.0 & 725.882999999999 & 28.5512217251731 & 561.978132506832 & 90.3266437459935\\
  PCCS1 857 G008.30-68.26 & 348.868278162408 & -34.119278500269 & SGP & Cirrus & 98.7950363159179 & 390.674346923828 & 11.0 & 531.273 & 22.6286095905161 & 453.663319848477 & 88.5139283190477\\
  PLCKERC857 G222.32-80.00 & 24.0736472858123 & -28.311932113875 & SGP & Cirrus & 971.944213867187 & 128.258438110351 & 16.0 & 626.811000000000 & 27.3517343691401 & 475.303364489227 & 89.6232117924126\\
  PCCS1 857 G311.06-73.30 & 9.64026906857268 & -43.622250149622 & ELAIS-S1 & ESO 242- G 021 & 901.016662597656 & 288.038665771484 & 4.0 & 127.673055648803 & 12.0209494845090 & 1083.06154133997 & 97.0903115523812\\
  PCCS1 857 G310.95-73.87 & 9.81662433984342 & -43.064443602454 & ELAIS-S1 & ESO 242- G 023 & 1400.224609375 & 212.262817382812 & 16.0 & 1260.87343978881 & 21.3641032459826 & 1371.25441577290 & 107.119162498042\\
  PCCS1 857 G357.76-75.78 & 358.749271623851 & -34.601801398255 & SGP & ESO 349- G 005 & 542.855346679687 & 284.972991943359 & 9.0 & 864.75 & 19.0759095196008 & 782.488557415083 & 91.1012836891545\\
  PCCS1 857 G356.25-76.69 & 359.916843030254 & -34.480501329200 & SGP & ESO 349- G 015, ESO 349- G 016 & 761.628479003906 & 198.772933959960 & 12.0 & 870.535 & 23.1918573426105 & 637.623988792300 & 91.1280290134258\\
  PCCS1 857 G353.76-79.19 & 2.80890060056760 & -33.594169159213 & SGP & ESO 349- G 038 & 426.270629882812 & 214.080001831054 & 7.0 & 594.800999999999 & 17.1249095764036 & 650.464368466287 & 87.7524608364427\\
  PCCS1 857 G259.62-82.44 & 18.9956285450550 & -32.491105362059 & SGP & ESO 352- G 030 & 821.906127929687 & 421.333312988281 & 15.0 & 866.928000000000 & 26.0055053594426 & 810.538060881197 & 95.6901079257705\\
  PCCS1 857 G254.41-81.05 & 20.8247371016961 & -32.825591793018 & SGP & ESO 352- G 063 & 487.249694824218 & 382.004364013671 & 10.0 & 959.305000000000 & 21.6218806998836 & 851.4086208269 & 97.1372382834257\\
  PCCS1 857 G255.18-80.62 & 21.1383365026818 & -33.184412442048 & SGP & ESO 352- G 071 & 592.479309082031 & 280.899261474609 & 14.0 & 929.917999999999 & 25.1858900180239 & 805.253424663096 & 95.9246850527802\\
  PLCKERC857 G249.83-79.43 & 22.9420292080645 & -33.109223491821 & SGP & ESO 353- G 009 & 2089.44262695312 & 154.972351074218 & 11.0 & 1199.65799999999 & 21.2557896348265 & 1540.96704390272 & 117.375776851970\\
  PLCKERC857 G014.32-65.00 & 344.602243440285 & -32.225314899447 & SGP & ESO 406- G 035 & 1014.15716552734 & 133.250335693359 & 11.0 & 882.600999999999 & 21.2831004790185 & 965.127568503376 & 97.1672419795677\\
  PLCKERC857 G009.50-65.08 & 344.980760746780 & -34.238306888944 & SGP & ESO 406- G 039 & 1309.26721191406 & 107.912231445312 & 14.0 & 1436.70899999999 & 25.4602420844735 & 1221.57544936239 & 108.597081059663\\
  PLCKERC857 G006.28-68.56 & 349.425700838103 & -34.773997056498 & SGP & ESO 407- G 014 & 1297.87512207031 & 112.861938476562 & 13.0 & 959.651 & 24.5644318069846 & 1042.60742305964 & 102.394100182131\\
  PCCS2 857 G010.95-86.53 & 9.20403065873973 & -28.378601933404 & SGP & ESO 410- G 027 & 438.357208251953 & 324.321136474609 & 10.0 & 633.88 & 21.5820399638217 & 556.392204884439 & 89.5656591121211\\
  PLCKERC857 G359.78-81.31 & 4.32363788409928 & -31.616599170889 & SGP & ESO 410-IG 006 & 953.021667480468 & 134.535018920898 & 13.0 & 900.153 & 23.9702718173991 & 910.821553211659 & 97.7954868323968\\
  PCCS1 857 G319.26-85.76 & 11.4669675450997 & -31.190239853059 & SGP & ESO 411- G 010 & 583.370849609375 & 168.530349731445 & 11.0 & 538.439999999999 & 22.4639624064856 & 427.081102829426 & 87.3805448504734\\
  PCCS1 857 G294.36-85.05 & 13.7274947012738 & -32.017353745984 & SGP & ESO 411- G 030, ESO 411- G 029, AM 0052-321 & 654.666870117187 & 287.853363037109 & 13.0 & 1338.55299999999 & 24.1763808085494 & 1065.67277225106 & 102.689610304524\\
  PCCS1 857 G253.13-83.53 & 18.6324097419184 & -31.185540183600 & SGP & ESO 412- G 021 & 1130.83862304687 & 293.395782470703 & 16.0 & 1269.271 & 24.9486713874707 & 1105.37821348011 & 101.136726482969\\
  PLCKERC857 G247.41-81.38 & 21.2116192444459 & -31.758466977377 & SGP & ESO 413- G 004 & 1174.833984375 & 175.572799682617 & 15.0 & 738.338000000000 & 26.2518678764007 & 926.338612549006 & 99.2473307165668\\
  PLCKERC857 G224.07-79.17 & 24.9878396758533 & -28.697467197735 & SGP & ESO 413- G 016 & 1064.91174316406 & 111.796478271484 & 11.0 & 1015.322 & 21.5100301487468 & 955.658854611218 & 97.2971675403396\\
  PCCS1 857 G220.52-79.20 & 24.9989781162361 & -28.030653301097 & SGP & ESO 413- G 018 & 662.473571777343 & 172.401428222656 & 11.0 & 958.031 & 21.5197584094245 & 1077.10445275902 & 101.213009415299\\
  PLCKERC857 G016.48-57.99 & 336.338499556597 & -31.349576301631 & SGP & ESO 467-IG 055, ESO 467-IG 055 NED01, ESO 467-IG 055 NED02 & 1532.98950195312 & 129.553253173828 & 11.0 & 1332.78900000000 & 28.1728373792914 & 1337.79089355468 & 123.861196693311\\
  PLCKERC857 G018.03-66.69 & 346.485228550831 & -30.615730877654 & SGP & ESO 469- G 011 & 1120.31018066406 & 139.212097167968 & 11.0 & 927.794 & 22.6692329601157 & 779.658592231571 & 95.3832445544393\\
  PCCS1 857 G015.37-71.81 & 352.512597343467 & -31.131052004144 & SGP & ESO 470- G 013, (Lens Candidate) 2MASX J23300478-3107468 & 606.292907714843 & 289.868133544921 & 9.0 & 839.265000000000 & 20.6162761428925 & 971.368648294359 & 99.9297571957205\\
  PCCS1 857 G014.42-76.50 & 357.957753441135 & -30.619438550373 & SGP & ESO 471- G 028 & 929.214965820312 & 196.229705810546 & 16.0 & 952.971999999999 & 26.6316835367199 & 829.889602907933 & 95.8506302330647\\
  PCCS2 857 G221.37-54.48 & 52.8300136250143 & -26.557541296191 & CDFS & ESO 482- G 001 & 749.10400390625 & 301.406677246093 & 13.0 & 851.408851623535 & 15.9265388381002 & 1223.14071097725 & 99.5686437236491\\
  PCCS1 857 G354.65+51.85 & 221.871451331813 & 1.03479334236612 & G15 & FGC 1806 & 826.847229003906 & 307.862091064453 & 11.0 & 774.678301932124 & 36.3908705859038 & 546.949372708797 & 94.3745974105001\\
  PCCS1 857 G231.90+31.90 & 139.457021375888 & -0.2665752484655 & G09 & IC 0531 & 722.972534179687 & 196.435684204101 & 8.0 & 745.981689362675 & 31.5694764289812 & 722.920825986191 & 98.6638866600368\\
  PCCS1 857 G140.74+87.22 & 191.881302870995 & 29.767998259321 & NGP & IC 0821 & 730.034423828125 & 156.005798339843 & 13.0 & 672.789999999999 & 24.2224671328087 & 596.392356965690 & 90.3858658743981\\
  PCCS1 857 G002.19+85.13 & 197.459054621257 & 24.5660378797922 & NGP & IC 0854 & 389.026000976562 & 233.040283203125 & 7.0 & 592.286 & 18.3638069582535 & 315.223157592117 & 85.7300822752209\\
  PLCKERC857 G008.90+84.11 & 198.767689469048 & 24.6109648178756 & NGP & IC 0860 & 2051.61767578125 & 156.499725341796 & 17.0 & 2176.09199999999 & 27.2240685607423 & 1778.40766917914 & 128.899423509758\\
  PLCKERC857 G082.93+80.60 & 200.138465827809 & 34.1326495617089 & NGP & IC 0883 & 2553.11547851562 & 147.372756958007 & 13.0 & 2768.33699999999 & 24.2961041938826 & 2200.53513591736 & 147.526156295889\\
  PLCKERC857 G339.69-83.51 & 8.27500254055224 & -32.248959419103 & SGP & IC 1554 & 1159.24291992187 & 103.499389648437 & 9.0 & 1015.744 & 20.4514347907426 & 902.653217393904 & 97.5897751626152\\
  PCCS1 857 G251.82-84.57 & 17.7543899650863 & -30.447848148590 & SGP & IC 1637 & 560.050048828125 & 213.865951538085 & 8.0 & 825.218000000000 & 18.4794991274114 & 1147.90387142077 & 102.673685037733\\
  PLCKERC857 G262.57-82.60 & 18.5368759134403 & -32.645076802388 & SGP & IC 1657, ESO-LV 3520242, ESO-LV 3520241 & 1847.79077148437 & 180.092102050781 & 12.0 & 1579.47100000000 & 21.8413544680727 & 2055.78412442468 & 138.818444706394\\
  PLCKERC857 G225.15-79.05 & 25.0949600620052 & -28.911402828170 & SGP & IC 1720 & 1834.95874023437 & 165.348739624023 & 14.0 & 1224.65099999999 & 25.4161993028068 & 1523.14753797277 & 119.363439189844\\
  PCCS1 857 G057.74+87.73 & 195.192445865713 & 28.0608194332605 & NGP & IC 4040, NGC 4908 GROUP, IC 4051 & 433.958129882812 & 182.404953002929 & 8.0 & 658.779000000000 & 19.3769342260327 & 355.621226198971 & 86.4162182203486\\
  PLCKERC857 G010.62-64.19 & 343.833905212076 & -33.887058683663 & SGP & IC 5262, MCG -06-50-011, v2MCG 79 & 1032.45422363281 & 102.745300292968 & 19.0 & 1442.749 & 29.6793218251360 & 1105.09862317889 & 105.103085439398\\
  PLCKERC857 G010.78-64.76 & 344.509118488156 & -33.744199744195 & SGP & IC 5271 & 3848.01318359375 & 142.237121582031 & 10.0 & 1498.17199999999 & 21.9983926230986 & 3184.78141731768 & 194.816344016697\\
  PCCS2 857 G326.23-88.15 & 12.0285180428906 & -28.816577736818 & SGP & IRAS F00456-2904NE & 69.3863677978515 & 237.743133544921 & 6.0 & 570.857000000000 & 17.1284791502339 & 232.269726552069 & 85.3439966846791\\
  PLCKERC857 G054.78+83.32 & 199.971908515046 & 29.4322246461036 & NGP & KUG 1317+296 & 1212.89880371093 & 136.556198120117 & 22.0 & 956.482 & 28.8100531412213 & 769.806535374838 & 91.0466486298966\\
  PCCS1 857 G071.66+80.96 & 201.211116356620 & 32.5308413113046 & NGP & KUG 1322+328 & 701.956848144531 & 308.087280273437 & 7.0 & 597.538000000000 & 17.4826689038029 & 389.104806978255 & 84.6685412353363\\
  PLCKERC857 G052.87+68.36 & 217.091090944403 & 32.3971234982807 & Bootes & KUG 1426+326 & 1256.8212890625 & 111.902008056640 & 11.0 & 665.392218000000 & 24.5126548976122 & 0.0 & 0.0\\
  PLCKERC857 G059.17+66.46 & 218.821587717897 & 35.1141694022986 & Bootes & KUG 1433+353 & 999.050048828125 & 112.322486877441 & 1.0 & 31.34081 & 9.56506491275566 & 1080.77014154804 & 95.5095439423376\\
  PCCS1 857 G131.83-60.95 & 17.1680924028736 & 1.61878477761794 & Hers & LBQS 0106+0119 (QSO) & 656.981811523437 & 268.581024169921 & 2.0 & 268.89847 & 17.4139748764058 & 536.182421748328 & 281.607528076181\\
  PCCS1 857 G062.57+78.53 & 204.656622204193 & 32.3031755090510 & NGP & MCG +06-30-064 & 786.864685058593 & 402.267303466796 & 13.0 & 733.597999999999 & 23.8605256647878 & 427.519744351506 & 86.3495449340010\\
  PCCS1 857 G054.16+67.86 & 217.596337028036 & 32.9442954237591 & Bootes & MCG +06-32-051, MCG +06-32-052 & 448.324829101562 & 159.483245849609 & 20.0 & 786.463694999999 & 31.8986439174241 & 864.964300992957 & 89.7250737261871\\
  PLCKERC857 G060.85+67.13 & 217.836483999550 & 35.5984667938567 & Bootes & MCG +06-32-056 & 1018.02447509765 & 97.8320007324218 & 20.0 & 1281.47083499999 & 30.1378523650237 & 1500.11328150447 & 111.650951213797\\
  PLCKERC857 G084.40+43.10 & 245.452907293996 & 55.0761637036682 & ELAIS-N1 & MCG +09-27-025, NGC 6143 & 1107.98315429687 & 75.8414001464843 & 20.0 & 1352.86855125427 & 28.6720377338652 & 1530.61241069054 & 113.872179203101\\
  PLCKERC857 G148.24+52.44 & 163.019517517055 & 58.4170168434623 & Lockman & MCG +10-16-015, NGC 3408 & 812.748474121093 & 100.363174438476 & 15.0 & 1077.04426574707 & 19.9762785673165 & 1170.64404656006 & 98.5036424262128\\
  PCCS1 857 G007.78-77.44 & 359.470914708799 & -31.821911524318 & SGP & MCG -05-01-015 & 564.573608398437 & 205.221511840820 & 8.0 & 629.675000000000 & 18.4520890958178 & 624.664761269465 & 87.8875010433274\\
  PCCS2 857 G246.27-80.51 & 22.2023828342556 & -32.028888558919 & SGP & MCG -05-04-040 & 1012.75720214843 & 280.089538574218 & 8.0 & 478.106999999999 & 19.7784275411368 & 526.109308570623 & 90.0612171365974\\
  PCCS1 857 G354.13-78.58 & 2.15246892824209 & -33.870670188418 & SGP & NGC 0010 & 1353.03625488281 & 253.503448486328 & 9.0 & 1078.68600000000 & 20.4276631801094 & 1718.98798428475 & 126.502130613814\\
  PCCS2 857 G349.11-81.94 & 5.97293468755911 & -32.535545419268 & SGP & NGC 0101 & 1108.068359375 & 193.425857543945 & 7.0 & 557.171 & 17.2998637855909 & 885.712110351771 & 94.3682796392042\\
  PLCKERC857 G340.47-81.55 & 6.68854966844275 & -33.685519412121 & SGP & NGC 0115 & 808.839904785156 & 115.255279541015 & 6.0 & 400.085 & 17.1732802341311 & 502.090593338012 & 88.2316810416841\\
  PCCS1 857 G339.08-82.27 & 7.41624539332167 & -33.262161115595 & SGP & NGC 0131 & 853.259948730468 & 308.324645996093 & 9.0 & 721.84 & 18.3816204127927 & 695.082320868969 & 87.2480419049452\\
  PLCKERC857 G338.28-82.37 & 7.59350574437974 & -33.246430660104 & SGP & NGC 0134 & 23886.99609375 & 438.99560546875 & 4.0 & 6594.51999999999 & 14.0592568438022 & 22166.7202058397 & 1221.86812950391\\
  PLCKERC857 G021.83-86.13 & 8.57059168127201 & -27.807161996791 & SGP & NGC 0150 & 4603.91943359375 & 196.872268676757 & 12.0 & 1963.01 & 23.3499538757574 & 4046.70947604626 & 238.021395406862\\
  PLCKERC857 G355.57-86.04 & 9.24847319246857 & -29.481636084623 & SGP & NGC 0174 & 2142.51538085937 & 139.763076782226 & 10.0 & 2616.78500000000 & 21.4720094541707 & 2418.62685773894 & 158.426444321950\\
  PLCKERC857 G299.12-85.91 & 13.1763085456619 & -31.206216061569 & SGP & NGC 0289, NGC 0289 GROUP & 7416.40771484375 & 174.840438842773 & 10.0 & 2200.294 & 21.5259829740711 & 5405.30211170762 & 309.080725412785\\
  PLCKERC857 G256.92-85.55 & 16.5580329350054 & -30.167935091667 & SGP & NGC 0378, MCG -05-03-025 & 1441.38366699218 & 128.914916992187 & 8.0 & 1128.37999999999 & 19.5995675972711 & 1301.10695482976 & 110.826634038644\\
  PLCKERC857 G250.46-84.78 & 17.6410057179953 & -30.221650157385 & SGP & NGC 0418 & 1684.23559570312 & 95.8829650878906 & 8.0 & 735.644999999999 & 19.6494489235703 & 1476.96065269038 & 117.315097838712\\
  PLCKERC857 G239.77-85.12 & 17.8467768148461 & -29.241895635432 & SGP & NGC 0423 & 1707.85534667968 & 150.224136352539 & 11.0 & 994.053 & 22.8298575335020 & 1065.01361269690 & 103.213586807951\\
  PLCKERC857 G134.22-61.41 & 18.2361635993002 & 0.98613435074136 & Hers & NGC 0428 & 2790.7021484375 & 271.175750732421 & 6.0 & 257.016789999999 & 28.2930480290205 & 2731.25250108806 & 310.633087704108\\
  PCCS1 857 G136.33-63.11 & 18.8779315472678 & -0.8755441992453 & Hers & NGC 0450 & 1955.27648925781 & 483.931304931640 & 4.0 & 186.992891 & 22.4072387987886 & 2271.57424124035 & 240.903077996246\\
  PCCS2 857 G140.57-59.63 & 21.6785795513570 & 2.02493097926242 & Hers & NGC 0550 & 822.692016601562 & 351.170135498046 & 2.0 & 98.53915 & 18.8467203459342 & 0.0 & 0.0\\
  PCCS1 857 G144.85-62.07 & 22.9330701375286 & -0.9272412516492 & Hers & NGC 0585 & 1158.87731933593 & 174.675018310546 & 3.0 & 116.637777 & 20.8225058940797 & 1185.41886761290 & 285.296096653679\\
  PLCKERC857 G229.07-80.28 & 23.5807617721431 & -29.418142609395 & SGP & NGC 0613, NGC 0613:[H66] 24, NGC 0613:[H66] 21, NGC 0613:[H66] ... & 17226.9453125 & 296.309600830078 & 15.0 & 7490.69600000000 & 26.5550879682218 & 17809.2718269284 & 983.377234714265\\
  PCCS1 857 G145.82-60.22 & 24.0018254347564 & 0.65465676540581 & Hers & NGC 0622 & 306.889221191406 & 489.028137207031 & 3.0 & 413.663249999999 & 19.2379891713234 & 277.217450600574 & 196.172771694750\\
  PLCKERC857 G230.65-79.17 & 24.7685895908199 & -29.916201238075 & SGP & NGC 0642, NGC 0639 & 2318.5654296875 & 148.755065917968 & 9.0 & 1375.608 & 19.6073004771182 & 2102.04219528846 & 141.488411351611\\
  PCCS2 857 G155.97-57.96 & 29.6708838930100 & 0.52790176854943 & Hers & NGC 0768 & 820.46875 & 198.021316528320 & 6.0 & 445.467765 & 25.8573334317308 & 863.682556941946 & 217.543684509496\\
  PCCS1 857 G157.99-58.08 & 30.5364880665581 & -0.1121919111659 & Hers & NGC 0800 & 420.132843017578 & 205.362091064453 & 2.0 & 94.23938 & 15.9947095707590 & 601.777854915275 & 185.405874312938\\
  PCCS1 857 G163.10-57.02 & 33.4136792271715 & -0.7146535727786 & Hers & NGC 0856 & 266.760559082031 & 265.65625 & 1.0 & 45.116226 & 13.3208611965434 & 310.782994927620 & 273.127459817045\\
  PCCS1 857 G163.48-56.94 & 33.6307562270137 & -0.7670744853426 & Hers & NGC 0863 & 238.080261230468 & 507.716125488281 & 4.0 & 352.929521999999 & 23.4300479689468 & 317.456576319984 & 268.878306711213\\
  PLCKERC857 G172.21-60.84 & 34.6801135807596 & -6.6253924490689 & XMM-LSS & NGC 0881 & 1825.49108886718 & 122.096633911132 & 11.0 & 386.635478973388 & 26.6173040601623 & 2389.55645009676 & 151.796801118875\\
  PLCKERC857 G171.77-59.54 & 35.4016772430094 & -5.5233104190960 & XMM-LSS & NGC 0895, NGC 0894, (Lens Candidate) & 3736.12622070312 & 155.385192871093 & 8.0 & 1861.83509826660 & 22.9032531529100 & 3606.30125771576 & 212.171621473404\\
  PLCKERC857 G263.34-41.83 & 67.9127564553683 & -54.603018497315 & ADFS & NGC 1617 & 2212.97607421875 & 97.7623138427734 & 41.0 & 2237.64892959594 & 47.6477550753039 & 2282.08358712627 & 146.695151012796\\
  PLCKERC857 G152.29+53.37 & 161.354648565173 & 55.9636701901414 & Lockman & NGC 3353 & 1199.67028808593 & 114.464851379394 & 1.0 & 28.2653980255126 & 8.47418419306133 & 1483.32751484699 & 111.612648824432\\
  PLCKERC857 G149.59+53.66 & 163.649537323092 & 56.9861360915470 & Lockman & NGC 3445, UGC 06021 NOTES01 & 846.481140136718 & 92.0180358886718 & 26.0 & 1277.98277664184 & 28.3877611105428 & 663.732986679101 & 83.1732557800218\\
  PLCKERC857 G147.66+53.84 & 165.362512689286 & 57.6769448001829 & Lockman & NGC 3488 & 745.925170898437 & 103.494903564453 & 27.0 & 1070.08061408996 & 31.6991990619363 & 1121.84176304157 & 96.8848061053150\\
  PLCKERC857 G263.84+57.55 & 173.087712357947 & 0.81032791573236 & G12 & NGC 3719, NGC 3720 & 1668.64514160156 & 167.455642700195 & 8.0 & 2019.33179840536 & 48.9845805024397 & 1902.51544921472 & 137.470398970094\\
  PCCS1 857 G272.55+58.08 & 177.349693218894 & -1.0826642836056 & G12 & NGC 3907B & 806.961486816406 & 521.340637207031 & 6.0 & 931.523048686832 & 33.4071813088144 & 549.392504826188 & 93.4688638075056\\
  PLCKERC857 G277.37+59.21 & 180.099652530057 & -1.1042999192051 & G12 & NGC 4030:[BKB2006] 0044, NGC 4030:[BKB2006] 0015, NGC 4030:[BKB... & 16747.423828125 & 286.839813232421 & 6.0 & 13441.8592559782 & 70.2873499287033 & 13165.6176127642 & 729.655094752019\\
  PCCS1 857 G140.19+86.20 & 191.549036502166 & 30.7486620881658 & NGP & NGC 4676:[BFB2004] 1579, NGC 4676:[BFB2004] 1489, NGC 4676:[BFB... & 618.35986328125 & 251.539352416992 & 9.0 & 1041.65999999999 & 20.5307969645603 & 864.631713867187 & 97.0527186905857\\
  PCCS1 857 G125.67+83.96 & 192.514578382354 & 33.1580731424716 & NGP & NGC 4719 & 460.345672607421 & 199.740844726562 & 7.0 & 678.566999999999 & 18.3461109775341 & 838.027941515669 & 96.3285099960032\\
  PLCKERC857 G294.85+88.35 & 192.602889337271 & 25.4967462417664 & NGP & NGC 4725:[BKB2006] 0101, NGC 4725:[BKB2006] 0055, NGC 4725:[BKB... & 11974.1044921875 & 574.252502441406 & 30.0 & 4682.46999999999 & 35.5039329793193 & 11784.8385812537 & 653.583398704991\\
  PCCS1 857 G125.12+88.34 & 192.787362312095 & 28.7810224978455 & NGP & NGC 4738 & 854.051513671875 & 171.858718872070 & 13.0 & 833.026 & 24.2404304829761 & 627.483967952430 & 90.9470459397938\\
  PLCKERC857 G306.37+88.63 & 192.950245666507 & 25.7691288464973 & NGP & NGC 4747 & 1861.85534667968 & 112.518798828125 & 14.0 & 1211.337 & 24.9451262173595 & 1813.92160071816 & 130.472319095478\\
  PLCKERC857 G101.57+88.05 & 193.666835217349 & 28.9330257439814 & NGP & NGC 4793 & 5551.93896484375 & 139.513793945312 & 6.0 & 2827.12400000000 & 17.1341416184178 & 4950.60827536135 & 284.963192287632\\
  PCCS1 857 G070.45+88.15 & 194.517431029173 & 28.2401880699831 & NGP & NGC 4848 & 442.520111083984 & 216.217941284179 & 7.0 & 712.392 & 18.2080799921353 & 604.365868404507 & 90.2951932094782\\
  PLCKERC857 G050.58+87.80 & 195.226503978063 & 27.7747964832464 & NGP & NGC 4911, CGCG 160-092 & 1105.08068847656 & 136.00048828125 & 11.0 & 1022.33100000000 & 22.4197797268394 & 1087.69733406696 & 103.184407441977\\
  PCCS1 857 G052.56+87.66 & 195.343689413168 & 27.8897896680177 & NGP & NGC 4921 & 335.175231933593 & 211.207809448242 & 11.0 & 549.341 & 22.3904199380002 & 551.874540153890 & 89.4956503837944\\
  PLCKERC857 G077.99+86.90 & 195.363439379512 & 29.2952197031420 & NGP & NGC 4922 NED01, NGC 4922, NGC 4922 NED02 & 899.545776367187 & 165.558471679687 & 13.0 & 1201.606 & 24.2010732613245 & 892.43090903759 & 97.4001502756920\\
  PLCKERC857 G044.43+86.76 & 196.445996937615 & 27.7284748656189 & NGP & NGC 4961 & 1366.76794433593 & 134.138381958007 & 9.0 & 882.914 & 20.4451028121650 & 1136.08644527196 & 104.896524678773\\
  PLCKERC857 G057.61+85.56 & 197.459077053683 & 28.9034705609265 & NGP & NGC 5000 & 842.436218261718 & 95.9056549072265 & 7.0 & 678.072000000000 & 17.2155394338951 & 857.121894832700 & 93.1708777745659\\
  PLCKERC857 G063.78+85.05 & 197.737741126354 & 29.5783648444188 & NGP & NGC 5004A & 1246.70739746093 & 132.528488159179 & 13.0 & 1036.12799999999 & 24.1419915085727 & 748.708760075271 & 93.6506751497974\\
  PLCKERC857 G351.34+83.78 & 197.903183993503 & 22.9140126804950 & NGP & NGC 5012, NGC 0134 & 3810.02026367187 & 102.557182312011 & 6.0 & 1372.476 & 17.2700852053485 & 3350.59361596032 & 202.651590694277\\
  PLCKERC857 G001.00+84.43 & 198.030373030302 & 24.0922720664899 & NGP & NGC 5016 & 1676.15661621093 & 101.387626647949 & 8.0 & 900.66 & 19.5072858952751 & 1404.71574965864 & 114.257175509328\\
  PLCKERC857 G079.49+83.41 & 198.186232786109 & 31.8113914273834 & NGP & NGC 5025 & 1053.15600585937 & 168.136657714843 & 3.0 & 490.759 & 13.0249991554702 & 694.380103878676 & 92.3382664197864\\
  PLCKERC857 G041.82+85.07 & 198.362318284588 & 27.7827253495199 & NGP & NGC 5032B, NGC 5032 & 1140.00048828125 & 144.350662231445 & 13.0 & 845.954 & 23.8812950863222 & 968.453263383358 & 99.3658214450918\\
  PLCKERC857 G069.61+83.37 & 199.052151044354 & 30.9483653484049 & NGP & NGC 5056 & 1332.01538085937 & 131.784454345703 & 15.0 & 1074.77099999999 & 23.9824554622749 & 1176.64390429109 & 102.933640329623\\
  PCCS2 857 G069.35+83.06 & 199.375816122975 & 31.0951933774833 & NGP & NGC 5065, KUG 1315+313 & 609.83154296875 & 253.478103637695 & 10.0 & 815.100999999999 & 19.4842427874423 & 662.120057052001 & 86.9014278899493\\
  PLCKERC857 G047.31+83.73 & 199.771776174740 & 28.5148247302206 & NGP & NGC 5081 & 911.583251953125 & 101.254631042480 & 9.0 & 611.944999999999 & 18.4166472790244 & 906.467826068401 & 92.7147817815126\\
  PLCKERC857 G033.44+82.97 & 200.742262848196 & 26.9710403941271 & NGP & NGC 5116 & 1142.25744628906 & 139.358230590820 & 4.0 & 655.307 & 14.6028126400361 & 842.485363230109 & 95.8707718084763\\
  PCCS2 857 G044.42+82.93 & 200.731770907874 & 28.3161945660778 & NGP & NGC 5117 & 408.308654785156 & 174.797882080078 & 4.0 & 363.368999999999 & 14.6643847126294 & 319.283705882728 & 85.7256760874046\\
  PLCKERC857 G066.66+80.62 & 202.057468140362 & 32.0342049600909 & NGP & NGC 5166 & 1051.15100097656 & 134.637496948242 & 9.0 & 995.322 & 20.0306958940522 & 1041.44697900861 & 100.780474521370\\
  PCCS2 857 G060.66+80.72 & 202.448368482774 & 31.1152470074853 & NGP & NGC 5187 & 580.378967285156 & 307.829620361328 & 6.0 & 654.065 & 17.2751506505732 & 482.078260548412 & 88.5060613267043\\
  PLCKERC857 G037.10+79.78 & 204.351157441295 & 27.4034894234444 & NGP & NGC 5251 & 1252.29919433593 & 107.892028808593 & 16.0 & 925.397999999999 & 26.4660907955821 & 952.083275045733 & 99.0305574029495\\
  PLCKERC857 G042.48+79.19 & 204.985658873599 & 28.3966580720038 & NGP & NGC 5263 & 1877.38024902343 & 86.0373229980468 & 7.0 & 1499.19600000000 & 18.4130420897797 & 1611.61146345734 & 122.309836595787\\
  PCCS1 857 G340.43+55.75 & 212.898164354793 & -1.1650571541196 & G15 & NGC 5496 & 983.73779296875 & 239.524444580078 & 3.0 & 1424.56476852264 & 68.3584947318180 & 1275.68915550410 & 114.102873783773\\
  PLCKERC857 G345.11+54.84 & 215.605471948322 & -0.3947757520474 & G15 & NGC 5584 & 3307.64794921875 & 171.290069580078 & 8.0 & 3101.60769375119 & 61.6790750660221 & 3153.20966356247 & 195.253233320259\\
  PCCS1 857 G060.74+67.53 & 217.376446633621 & 35.4546467436147 & Bootes & NGC 5646 & 668.574890136718 & 183.036849975585 & 14.0 & 832.129236999999 & 27.0201866659921 & 906.627299374507 & 90.9748042183923\\
  PLCKERC857 G060.27+67.38 & 217.605805623954 & 35.3187417551870 & Bootes & NGC 5656 & 2720.89672851562 & 145.631637573242 & 4.0 & 141.353697 & 14.8304892636860 & 2506.92093862658 & 157.481942357919\\
  PLCKERC857 G353.15+54.45 & 219.421766216113 & 2.28787325056857 & G15 & NGC 5690 & 5662.47607421875 & 198.444595336914 & 8.0 & 4965.49198255983 & 59.5237762158954 & 4792.05019582435 & 275.761711670228\\
  PCCS1 857 G350.17+52.42 & 219.461757849978 & -0.4057195027531 & G15 & NGC 5691 & 1124.92578125 & 262.660766601562 & 9.0 & 1382.01770272228 & 37.0491963745504 & 1336.76247682794 & 115.710475305091\\
  PLCKERC857 G350.46+51.85 & 219.962370637557 & -0.7158906119272 & G15 & NGC 5705 & 1537.86096191406 & 196.198318481445 & 6.0 & 1213.40908385091 & 50.7172384106232 & 1193.16234938055 & 109.879521758695\\
  PLCKERC857 G351.01+52.11 & 220.048463309301 & -0.2978993522210 & G15 & NGC 5713N, NGC 5713 & 7124.0458984375 & 221.619201660156 & 5.0 & 5927.50410509675 & 49.6585785539618 & 5877.12685440480 & 333.232770812340\\
  PLCKERC857 G351.22+51.97 & 220.237783044837 & -0.3201127758133 & G15 & NGC 5719 & 4001.26391601562 & 226.319671630859 & 6.0 & 4250.84320018934 & 62.9748126634768 & 4107.96398430317 & 240.049840552665\\
  PLCKERC857 G354.50+52.84 & 221.112904935199 & 1.67628153632543 & G15 & NGC 5740 & 2572.92822265625 & 190.299468994140 & 10.0 & 2460.84297155832 & 44.9108649326641 & 2313.26119498536 & 155.517361006198\\
  PLCKERC857 G354.96+52.95 & 221.237369096451 & 1.95137684438106 & G15 & NGC 5746 & 9795.0458984375 & 306.330902099609 & 7.0 & 7912.39920180437 & 94.9723337556785 & 7965.12483840435 & 447.129852048934\\
  PCCS1 857 G352.89+51.17 & 221.541395796973 & -0.2103662434432 & G15 & NGC 5750 & 666.042602539062 & 269.971984863281 & 4.0 & 1127.15255447212 & 39.3982067739129 & 1151.11181932687 & 109.421897164859\\
  PCCS1 857 G088.83+33.68 & 261.815230423427 & 60.0113517970009 & FLS & NGC 6381, UGC 10870 & 1073.61474609375 & 271.151794433593 & 26.0 & 1344.33556938171 & 37.5873110481604 & 0.0 & 0.0\\
  PLCKERC857 G012.07-57.79 & 336.087067446585 & -33.691906720124 & SGP & NGC 7267 & 1783.87756347656 & 87.9193191528320 & 15.0 & 1347.01799999999 & 32.3058844175484 & 1740.88175895460 & 138.459017648000\\
  PLCKERC857 G016.87-58.16 & 336.545213460709 & -31.146405785216 & SGP & NGC 7277 & 881.394714355468 & 148.490325927734 & 17.0 & 1245.539 & 34.2079070245462 & 1334.24789313226 & 123.713690496537\\
  PLCKERC857 G019.30-61.60 & 340.588930318234 & -30.053507544364 & SGP & NGC 7361 & 1925.4658203125 & 88.8556976318359 & 14.0 & 1425.75399999999 & 25.8940750945076 & 2485.01767349056 & 161.685315140218\\
  PLCKERC857 G015.44-75.68 & 356.964592773811 & -30.526925171621 & SGP & NGC 7755 & 3689.736328125 & 233.370544433593 & 7.0 & 1110.139 & 18.3535366346652 & 3312.28879386186 & 200.684006039953\\
  PLCKERC857 G004.50-77.17 & 359.464075879342 & -32.592337073324 & SGP & NGC 7793:[SL2011] 1\_281, NGC 7793:[SL2011] 1\_287, NGC 7793:[SL2... & 26166.84375 & 805.818725585937 & 25.0 & 9907.88299999999 & 29.5776850344985 & 25235.6873729176 & 1390.19138453328\\
  PCCS2 857 G355.71-77.40 & 0.73412938097876 & -34.223387485876 & SGP & NGC 7812 & 1160.02185058593 & 408.530487060546 & 11.0 & 839.154999999999 & 22.3484759211897 & 703.510340888053 & 92.5501494869550\\
  PLCKERC857 G250.12-80.58 & 21.7549765820703 & -32.539854826118 & SGP & R Sculptoris (Star) & 1292.42749023437 & 138.406860351562 & 6.0 & 859.861000000000 & 17.6896151173506 & 932.799807310104 & 99.5010941177961\\
  PCCS1 857 G226.34+23.23 & 129.495973864250 & -0.5597862129496 & G09 & SDSS J083800.68-003306.0 & 1310.97302246093 & 428.808532714843 & 7.0 & 337.860458626905 & 22.8638571330386 & 600.048461422324 & 93.9058314639514\\
  PCCS1 857 G352.22+83.55 & 198.157055876759 & 22.8272048209371 & NGP & SDSS J131244.75+225011.0  , NGC 5012A & 322.246917724609 & 171.129547119140 & 5.0 & 542.397 & 16.0268836022478 & 618.524291992187 & 91.8890177490422\\
  PLCKERC857 G070.52+80.05 & 202.235918449800 & 32.8799517816553 & NGP & SDSS J132856.58+325243.9 (QSO) & 1167.30920410156 & 107.503021240234 & 11.0 & 896.865 & 22.4459876815434 & 766.689904544502 & 94.2439599482282\\
  PCCS1 857 G135.78-62.78 & 18.7009951548446 & -0.4973647717443 & Hers & UGC 00793 NED01, UGC 00793, UGC 00793 NED02 & 822.600463867187 & 261.015502929687 & 6.0 & 826.387954 & 26.0289144395584 & 626.239119278537 & 186.340121024814\\
  PCCS1 857 G223.87+23.88 & 128.947574972689 & 1.72707783184563 & G09 & UGC 04491 & 460.310424804687 & 287.60693359375 & 3.0 & 618.293414791566 & 48.4047353675237 & 746.424740433692 & 91.1496819083550\\
  PCCS1 857 G232.19+31.64 & 139.373076588464 & -0.6125396435184 & G09 & UGC 04915 & 692.891418457031 & 324.422271728515 & 5.0 & 677.756534760980 & 28.1181659608161 & 399.983470439910 & 92.8677036092587\\
  PCCS1 857 G235.51+42.78 & 150.106666455457 & 3.37179453805327 & COSMOS & UGC 05376 & 1885.06298828125 & 222.405456542968 & 10.0 & 408.933950424194 & 22.2409465549474 & 0.0 & 0.0\\
  PCCS2 857 G268.20+56.69 & 174.631973472987 & -1.1746182687715 & G12 & UGC 06608 & 488.679901123046 & 203.882186889648 & 7.0 & 736.700189679599 & 28.3320683325450 & 558.775331504643 & 87.2200074441232\\
  PCCS1 857 G273.25+60.86 & 178.906777416049 & 1.24844038367633 & G12 & UGC 06903 & 1014.74633789062 & 289.599822998046 & 8.0 & 1058.54602351935 & 46.4495524090383 & 1033.98774366825 & 106.427824674143\\
  PLCKERC857 G108.32+88.72 & 193.225021875547 & 28.3621310776161 & NGP & UGC 08017 & 1182.96484375 & 113.775276184082 & 9.0 & 1258.66500000000 & 18.6291303339688 & 1277.47193129174 & 105.497619328243\\
  PLCKERC857 G101.38+83.79 & 195.568046976818 & 32.8726324376840 & NGP & UGC 08145, MCG +06-29-018a NED01, MCG +06-29-018a & 893.258056640625 & 109.484870910644 & 15.0 & 903.839999999999 & 25.6889924870556 & 758.842840090394 & 94.0282900421998\\
  PLCKERC857 G091.96+84.28 & 196.322362373749 & 31.9844249516101 & NGP & UGC 08179 & 890.019348144531 & 106.963211059570 & 9.0 & 979.225000000000 & 19.2268865914375 & 994.029662626562 & 97.2915301777559\\
  PCCS1 857 G049.28+86.01 & 197.201526228748 & 28.1839393874560 & NGP & UGC 08229 & 675.907836914062 & 338.891845703125 & 12.0 & 725.558 & 23.2713021982011 & 702.303684536367 & 92.4545352595463\\
  PCCS1 857 G094.47+81.88 & 197.524373638318 & 34.1854557001729 & NGP & UGC 08246 & 307.831939697265 & 206.298522949218 & 6.0 & 263.247 & 17.1800355063661 & 266.874472052790 & 85.5133549411722\\
  PCCS1 857 G086.19+81.12 & 199.258660720110 & 34.0950902218995 & NGP & UGC 08352 & 377.604248046875 & 248.663497924804 & 6.0 & 619.17 & 17.2997565878829 & 741.293311815708 & 93.6961815379348\\
  PLCKERC857 G038.66+84.14 & 199.434834645880 & 27.5593980336871 & NGP & UGC 08359 & 1217.96118164062 & 114.330879211425 & 9.0 & 667.601000000000 & 20.4147771479386 & 537.295084945857 & 89.0665825074426\\
  PCCS2 857 G006.30+81.88 & 200.753744817426 & 23.2733766448481 & NGP & UGC 08409 & 705.140075683593 & 157.036529541015 & 11.0 & 489.044999999999 & 22.3091556093008 & 369.196545772254 & 86.3128190984996\\
  PCCS1 857 G063.08+80.40 & 202.603221324719 & 31.6086002436900 & NGP & UGC 08498 & 823.222351074218 & 200.907867431640 & 7.0 & 620.741 & 18.3926905590237 & 788.302746254950 & 94.6841548865233\\
  PCCS2 857 G075.02+78.38 & 203.306087647065 & 34.5252202093738 & NGP & UGC 08536, KUG 1330+348 & 528.043823242187 & 294.668212890625 & 10.0 & 831.252 & 21.6518411457316 & 534.419629454612 & 89.7342464326658\\
  PCCS1 857 G072.04+78.37 & 203.734304960647 & 34.0387262533335 & NGP & UGC 08561, UGC 08561 NOTES01 & 1548.82287597656 & 299.448852539062 & 8.0 & 1449.27000000000 & 19.5643642114943 & 1720.00545105338 & 126.859129574826\\
  PLCKERC857 G075.27+77.67 & 203.962418614424 & 34.9887464258486 & NGP & UGC 08583 & 1026.00744628906 & 128.580841064453 & 10.0 & 775.093999999999 & 21.6081609583046 & 784.485368598252 & 95.0334919668415\\
  PCCS1 857 G056.93+78.78 & 204.845116599887 & 31.1782387250064 & NGP & UGC 08640 & 757.146301269531 & 370.537933349609 & 11.0 & 457.650999999999 & 22.3670388294919 & 259.733585409820 & 85.5546024157402\\
  PCCS2 857 G071.87+76.53 & 205.635153296842 & 35.0089885170568 & NGP & UGC 08681 & 767.960754394531 & 194.138015747070 & 13.0 & 821.684000000000 & 24.4178398921771 & 889.267622694373 & 97.9025534811290\\
  PLCKERC857 G051.72+78.22 & 205.793719568156 & 30.3244425688227 & NGP & UGC 08685 & 902.21533203125 & 116.531143188476 & 9.0 & 1259.23299999999 & 20.5057199093326 & 1191.81486433744 & 106.846153432556\\
  PCCS1 857 G065.77+76.25 & 206.772809009284 & 33.8888419818766 & NGP & UGC 08713, UGC 08715 & 964.721740722656 & 495.507751464843 & 12.0 & 854.891000000000 & 23.6181248620630 & 1035.94900245964 & 102.121114123473\\
  PLCKERC857 G347.77+56.35 & 215.864937612484 & 1.71971865546025 & G15 & UGC 09215 & 1220.68469238281 & 146.010574340820 & 8.0 & 1299.05219368744 & 53.420569484048 & 1486.80813708901 & 115.166719431289\\
  PCCS1 857 G347.54+55.75 & 216.144228785254 & 1.17226394138496 & G15 & UGC 09229 NOTES01, UGC 09229 & 888.322509765625 & 238.488723754882 & 9.0 & 859.493151049389 & 33.1276108405058 & 965.385630819946 & 96.8177810409720\\
  PCCS1 857 G089.40+34.18 & 260.750876651798 & 60.4501129209124 & FLS & UGC 10830 & 1319.07495117187 & 480.874847412109 & 29.0 & 1351.36425590515 & 34.2093194245500 & 0.0 & 0.0\\
  PLCKERC857 G055.79+67.45 & 217.965642105878 & 33.6229926031434 & Bootes & VV 775 NED02, VV 775, VV 775 NED01 & 1009.66278076171 & 183.973281860351 & 17.0 & 1089.83042899999 & 27.8966862511142 & 1537.57483552329 & 111.900265881805\\
  PCCS1 857 G238.20+42.27 & 150.845064457020 & 1.46887604778031 & COSMOS & VVDS 100163697, VVDS 100169379, VVDS 100164361 & 711.656005859375 & 268.705413818359 & 22.0 & 807.949884414672 & 31.7744304186396 & 1431.86449345364 & 107.875042943633\\
\hline\end{tabular}


==> Paper_revised_postreferee (copy)/FluxComparison/Table_AllSources <==
\begin{longtable}{lllllllll}
\toprule
    Field &                      NAME &        RA &        DEC &      P$_{Flux}$ &        H$_{Flux}$ &     N &    HS$_{Flux}$ \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
   Bootes &  PLCKERC857 G060.37+66.55 &  14:34:19 &  +35:33:33 &  1241 $\pm$ 151 &  1267 $\pm$ 103.0 &  30.0 &  1081 $\pm$ 14 \\
      EGS &  PLCKERC857 G095.44+58.94 &  14:24:31 &  +52:56:09 &  1141 $\pm$ 176 &       0 $\pm$ 0.0 &  29.0 &  1017 $\pm$ 11 \\
  Lockman &  PLCKERC857 G149.81+50.11 &  10:33:27 &  +59:11:46 &  1249 $\pm$ 131 &  1560 $\pm$ 114.0 &  28.0 &   988 $\pm$ 12 \\
      SGP &  PLCKERC857 G007.34-65.24 &  23:01:28 &  -35:06:10 &   920 $\pm$ 132 &    838 $\pm$ 97.0 &  27.0 &  1055 $\pm$ 34 \\
      FLS &   PCCS1 857 G089.66+36.10 &  17:07:19 &  +60:26:55 &   886 $\pm$ 194 &   1019 $\pm$ 94.0 &  27.0 &   859 $\pm$ 13 \\
      SGP &  PLCKERC857 G017.86-68.67 &  23:15:09 &  -30:35:29 &  1657 $\pm$ 167 &    498 $\pm$ 89.0 &  26.0 &  1046 $\pm$ 33 \\
      NGP &  PLCKERC857 G027.36+84.83 &  13:14:26 &  +26:30:38 &    792 $\pm$ 93 &    719 $\pm$ 93.0 &  25.0 &   873 $\pm$ 32 \\
      SGP &  PLCKERC857 G239.13-78.19 &  01:41:20 &  -31:47:11 &  1110 $\pm$ 145 &    678 $\pm$ 94.0 &  24.0 &   802 $\pm$ 32 \\
      NGP &  PLCKERC857 G042.54+81.51 &  13:29:26 &  +28:13:27 &  1697 $\pm$ 251 &    797 $\pm$ 95.0 &  24.0 &   978 $\pm$ 32 \\
      NGP &  PLCKERC857 G063.13+78.00 &  13:40:41 &  +32:37:17 &   912 $\pm$ 169 &    506 $\pm$ 85.0 &  23.0 &   854 $\pm$ 28 \\
   COSMOS &   PCCS1 857 G238.20+42.27 &  10:03:23 &  +01:28:08 &   712 $\pm$ 269 &  1327 $\pm$ 104.0 &  23.0 &    828 $\pm$ 8 \\
      NGP &  PLCKERC857 G068.89+81.23 &  13:24:54 &  +32:01:39 &  1802 $\pm$ 183 &    641 $\pm$ 88.0 &  23.0 &   913 $\pm$ 29 \\
      SGP &  PLCKERC857 G006.96-67.92 &  23:14:25 &  -34:40:46 &   940 $\pm$ 106 &    520 $\pm$ 89.0 &  22.0 &   800 $\pm$ 31 \\
      SGP &   PCCS1 857 G354.81-79.56 &  00:12:12 &  -33:13:39 &  1014 $\pm$ 233 &    644 $\pm$ 87.0 &  22.0 &   812 $\pm$ 27 \\
      NGP &   PCCS1 857 G058.53+82.57 &  13:22:26 &  +30:07:28 &   827 $\pm$ 197 &    554 $\pm$ 89.0 &  22.0 &   910 $\pm$ 30 \\
     ADFS &  PLCKERC857 G261.89-40.69 &  04:40:40 &  -53:44:02 &   795 $\pm$ 134 &  1304 $\pm$ 104.0 &  22.0 &   980 $\pm$ 11 \\
    HELMS &   PCCS1 857 G126.98-59.24 &  00:59:45 &  +03:33:29 &   383 $\pm$ 234 &   648 $\pm$ 304.0 &  21.0 &   685 $\pm$ 29 \\
      NGP &  PLCKERC857 G077.25+80.72 &  13:23:12 &  +33:23:12 &   1065 $\pm$ 97 &    500 $\pm$ 89.0 &  21.0 &   679 $\pm$ 29 \\
      NGP &   PCCS2 857 G029.94+79.79 &  13:36:55 &  +26:08:21 &   467 $\pm$ 258 &    380 $\pm$ 86.0 &  21.0 &   754 $\pm$ 29 \\
      SGP &   PCCS2 857 G013.36-62.85 &  22:48:24 &  -32:47:53 &   175 $\pm$ 281 &    600 $\pm$ 92.0 &  20.0 &   761 $\pm$ 30 \\
      SGP &  PLCKERC857 G222.32-80.00 &  01:36:18 &  -28:18:43 &   972 $\pm$ 128 &    454 $\pm$ 89.0 &  20.0 &   717 $\pm$ 30 \\
      SGP &   PCCS1 857 G018.31-71.34 &  23:27:28 &  -30:15:23 &   749 $\pm$ 360 &    419 $\pm$ 84.0 &  20.0 &   712 $\pm$ 27 \\
  XMM-LSS &   PCCS2 857 G170.56-57.15 &  02:26:06 &  -03:18:49 &   693 $\pm$ 211 &    962 $\pm$ 93.0 &  20.0 &   700 $\pm$ 11 \\
      NGP &  PLCKERC857 G062.48+78.89 &  13:37:06 &  +32:08:31 &   814 $\pm$ 109 &    573 $\pm$ 90.0 &  19.0 &   738 $\pm$ 28 \\
      NGP &  PLCKERC857 G028.53+83.67 &  13:19:37 &  +26:28:04 &  1301 $\pm$ 166 &    678 $\pm$ 87.0 &  19.0 &   743 $\pm$ 25 \\
      SGP &  PLCKERC857 G221.31-79.84 &  01:37:05 &  -28:08:48 &  1328 $\pm$ 191 &    460 $\pm$ 89.0 &  19.0 &   738 $\pm$ 29 \\
      SGP &   PCCS1 857 G001.66-72.03 &  23:36:11 &  -35:11:00 &   392 $\pm$ 305 &    424 $\pm$ 87.0 &  19.0 &   695 $\pm$ 28 \\
    HELMS &   PCCS1 857 G106.67-60.70 &  00:19:56 &  +01:10:02 &   169 $\pm$ 308 &   590 $\pm$ 392.0 &  19.0 &   691 $\pm$ 28 \\
      NGP &   PCCS1 857 G102.56+85.20 &  12:59:16 &  +31:36:37 &   831 $\pm$ 331 &    604 $\pm$ 90.0 &  19.0 &   632 $\pm$ 28 \\
      NGP &   PCCS1 857 G058.69+81.03 &  13:29:02 &  +30:42:43 &   845 $\pm$ 298 &    490 $\pm$ 88.0 &  19.0 &   800 $\pm$ 28 \\
     CDFS &   PCCS1 857 G222.56-53.84 &  03:34:41 &  -27:07:47 &   227 $\pm$ 185 &    814 $\pm$ 86.0 &  18.0 &    612 $\pm$ 6 \\
      SGP &   PCCS1 857 G014.92-58.26 &  22:26:32 &  -32:10:37 &   302 $\pm$ 239 &   679 $\pm$ 106.0 &  18.0 &   717 $\pm$ 34 \\
      NGP &   PCCS2 857 G044.42+78.90 &  13:41:09 &  +28:47:29 &   649 $\pm$ 288 &    382 $\pm$ 87.0 &  18.0 &   655 $\pm$ 27 \\
      NGP &  PLCKERC857 G014.88+80.31 &  13:31:43 &  +23:46:17 &  1243 $\pm$ 158 &     86 $\pm$ 84.0 &  18.0 &   653 $\pm$ 27 \\
    HELMS &   PCCS1 857 G122.50-59.77 &  00:50:35 &  +03:05:39 &   288 $\pm$ 296 &   475 $\pm$ 342.0 &  18.0 &   672 $\pm$ 27 \\
      G09 &   PCCS1 857 G223.82+24.63 &  08:38:19 &  +02:07:38 &  1622 $\pm$ 282 &  1044 $\pm$ 107.0 &  17.0 &   744 $\pm$ 33 \\
      SGP &   PCCS1 857 G008.30-68.26 &  23:15:28 &  -34:07:09 &    99 $\pm$ 391 &    669 $\pm$ 92.0 &  17.0 &   667 $\pm$ 27 \\
    HELMS &   PCCS2 857 G111.24-58.57 &  00:27:08 &  +03:44:57 &   184 $\pm$ 218 &    88 $\pm$ 389.0 &  17.0 &   570 $\pm$ 26 \\
      SGP &   PCCS1 857 G004.31-80.79 &  00:13:38 &  -31:13:02 &   369 $\pm$ 292 &    576 $\pm$ 90.0 &  17.0 &   637 $\pm$ 26 \\
      SGP &   PCCS1 857 G343.37-84.34 &  00:34:16 &  -31:21:51 &   463 $\pm$ 512 &    434 $\pm$ 87.0 &  17.0 &   601 $\pm$ 26 \\
 ELAIS-N1 &   PCCS2 857 G083.61+44.14 &  16:15:54 &  +54:15:36 &   458 $\pm$ 191 &    622 $\pm$ 81.0 &  16.0 &    574 $\pm$ 6 \\
      SGP &   PCCS1 857 G293.47-84.07 &  00:56:04 &  -32:57:54 &   138 $\pm$ 221 &    394 $\pm$ 87.0 &  15.0 &   486 $\pm$ 25 \\
      NGP &   PCCS2 857 G069.76+76.61 &  13:43:26 &  +34:32:49 &   572 $\pm$ 297 &    335 $\pm$ 86.0 &  15.0 &   539 $\pm$ 25 \\
     CDFS &  PLCKERC857 G224.76-54.44 &  03:32:53 &  -28:29:49 &   807 $\pm$ 102 &  1420 $\pm$ 107.0 &  14.0 &    607 $\pm$ 5 \\
      NGP &   PCCS1 857 G074.62+80.41 &  13:25:37 &  +33:14:25 &   425 $\pm$ 270 &    319 $\pm$ 86.0 &  14.0 &   507 $\pm$ 24 \\
      SGP &   PCCS2 857 G007.68-72.90 &  23:37:20 &  -33:10:01 &   669 $\pm$ 277 &    417 $\pm$ 87.0 &  14.0 &   499 $\pm$ 24 \\
      NGP &   PCCS2 857 G006.30+81.88 &  13:23:01 &  +23:16:24 &   705 $\pm$ 157 &    290 $\pm$ 85.0 &  14.0 &   557 $\pm$ 24 \\
      SGP &   PCCS1 857 G230.86-80.29 &  01:34:00 &  -29:42:44 &   424 $\pm$ 211 &    634 $\pm$ 92.0 &  14.0 &   602 $\pm$ 25 \\
      G12 &   PCCS1 857 G266.28+58.43 &  11:38:36 &  +00:50:29 &   643 $\pm$ 402 &    532 $\pm$ 95.0 &  13.0 &   680 $\pm$ 29 \\
      SGP &  PLCKERC857 G339.76-85.56 &  00:39:04 &  -30:38:52 &  1539 $\pm$ 223 &    300 $\pm$ 83.0 &  13.0 &   440 $\pm$ 22 \\
     HERS &   PCCS2 857 G138.41-61.22 &  01:20:59 &  +00:45:36 &   797 $\pm$ 246 &   760 $\pm$ 246.0 &  12.0 &   460 $\pm$ 25 \\
      G12 &   PCCS2 857 G279.25+59.98 &  12:05:04 &  -00:44:28 &   639 $\pm$ 243 &    501 $\pm$ 94.0 &  11.0 &   502 $\pm$ 27 \\
      NGP &   PCCS1 857 G036.04+80.21 &  13:35:28 &  +27:13:49 &   119 $\pm$ 474 &    172 $\pm$ 84.0 &  10.0 &   338 $\pm$ 20 \\
      G09 &  PLCKERC857 G230.55+31.91 &  09:15:26 &  +00:42:38 &   1216 $\pm$ 86 &    560 $\pm$ 95.0 &  10.0 &   397 $\pm$ 26 \\
     HERS &   PCCS1 857 G144.36-59.69 &  01:33:57 &  +01:23:29 &  1368 $\pm$ 207 &  1588 $\pm$ 278.0 &   9.0 &   381 $\pm$ 23 \\
      G09 &   PCCS1 857 G223.97+26.09 &  08:43:42 &  +02:43:11 &   546 $\pm$ 347 &    613 $\pm$ 96.0 &   9.0 &   548 $\pm$ 34 \\
     HERS &   PCCS1 857 G141.28-60.26 &  01:27:23 &  +01:19:05 &   565 $\pm$ 360 &   969 $\pm$ 272.0 &   8.0 &   294 $\pm$ 22 \\
    HELMS &   PCCS1 857 G115.91-56.23 &  00:35:46 &  +06:25:38 &   128 $\pm$ 378 &   543 $\pm$ 370.0 &   8.0 &   301 $\pm$ 18 \\
     HERS &   PCCS2 857 G156.60-56.71 &  02:02:19 &  +01:26:57 &  1033 $\pm$ 292 &  1051 $\pm$ 258.0 &   4.0 &   166 $\pm$ 16 \\
\end{longtable}


==> Paper_revised_postreferee (copy)/FluxComparison/Table_AllSourcesLens <==
\begin{tabular}{lllllllll}
\toprule
Field &                      NAME &        RA &        DEC &      P$_{Flux}$ [mJy] &     H$_{Flux}$ [mJy] &     N &    HS$_{Flux}$ [mJy] \\
\midrule
  NGP &  PLCKERC857 G047.32+82.53 &  13:24:28 &  +28:44:32 &  1303 $\pm$ 152 &   617 $\pm$ 90 &  20.0 &   985 $\pm$ 28 \\
  G12 &   PCCS2 857 G270.56+58.54 &  11:46:35 &  -00:11:14 &  1148 $\pm$ 337 &  988 $\pm$ 105 &  19.0 &  1095 $\pm$ 32 \\
  SGP &   PCCS1 857 G013.73-79.69 &  00:06:27 &  -30:03:53 &   724 $\pm$ 202 &   451 $\pm$ 88 &  16.0 &   570 $\pm$ 26 \\
 HERS &   PCCS2 857 G131.83-60.95 &  01:08:41 &  +01:37:03 &   654 $\pm$ 251 &  678 $\pm$ 281 &  16.0 &  1181 $\pm$ 27 \\
  SGP &  PLCKERC857 G014.99-59.64 &  22:33:02 &  -32:08:20 &   943 $\pm$ 115 &  390 $\pm$ 102 &  16.0 &   769 $\pm$ 32 \\
\bottomrule
\end{tabular}


==> Paper_revised_postreferee (copy)/FluxComparison/Table_AllSources_Short <==
\begin{tabular}{lllllllll}
\toprule
    Field &                      NAME &        RA &        DEC &      P$_{Flux} [mJy]$ &      H$_{Flux} [mJy]$ &   N &    HS$_{Flux} [mJy]$ \\
\midrule
   Bootes &  PLCKERC857 G060.37+66.55 &  14:34:19 &  +35:33:33 &  1241 $\pm$ 151 &  1267 $\pm$ 103.0 &  30.0 &  1081 $\pm$ 14 \\
      EGS &  PLCKERC857 G095.44+58.94 &  14:24:31 &  +52:56:09 &  1141 $\pm$ 176 &       0 $\pm$ 0.0 &  29.0 &  1017 $\pm$ 11 \\
  Lockman &  PLCKERC857 G149.81+50.11 &  10:33:27 &  +59:11:46 &  1249 $\pm$ 131 &  1560 $\pm$ 114.0 &  28.0 &   988 $\pm$ 12 \\
      SGP &  PLCKERC857 G007.34-65.24 &  23:01:28 &  -35:06:10 &   920 $\pm$ 132 &    838 $\pm$ 97.0 &  27.0 &  1055 $\pm$ 34 \\
      FLS &   PCCS1 857 G089.66+36.10 &  17:07:19 &  +60:26:55 &   886 $\pm$ 194 &   1019 $\pm$ 94.0 &  27.0 &   859 $\pm$ 13 \\
      SGP &  PLCKERC857 G017.86-68.67 &  23:15:09 &  -30:35:29 &  1657 $\pm$ 167 &    498 $\pm$ 89.0 &  26.0 &  1046 $\pm$ 33 \\
      NGP &  PLCKERC857 G027.36+84.83 &  13:14:26 &  +26:30:38 &    792 $\pm$ 93 &    719 $\pm$ 93.0 &  25.0 &   873 $\pm$ 32 \\
      SGP &  PLCKERC857 G239.13-78.19 &  01:41:20 &  -31:47:11 &  1110 $\pm$ 145 &    678 $\pm$ 94.0 &  24.0 &   802 $\pm$ 32 \\
      NGP &  PLCKERC857 G042.54+81.51 &  13:29:26 &  +28:13:27 &  1697 $\pm$ 251 &    797 $\pm$ 95.0 &  24.0 &   978 $\pm$ 32 \\
      NGP &  PLCKERC857 G063.13+78.00 &  13:40:41 &  +32:37:17 &   912 $\pm$ 169 &    506 $\pm$ 85.0 &  23.0 &   854 $\pm$ 28 \\
   COSMOS &   PCCS1 857 G238.20+42.27 &  10:03:23 &  +01:28:08 &   712 $\pm$ 269 &  1327 $\pm$ 104.0 &  23.0 &    828 $\pm$ 8 \\
      NGP &  PLCKERC857 G068.89+81.23 &  13:24:54 &  +32:01:39 &  1802 $\pm$ 183 &    641 $\pm$ 88.0 &  23.0 &   913 $\pm$ 29 \\
      SGP &  PLCKERC857 G006.96-67.92 &  23:14:25 &  -34:40:46 &   940 $\pm$ 106 &    520 $\pm$ 89.0 &  22.0 &   800 $\pm$ 31 \\
      SGP &   PCCS1 857 G354.81-79.56 &  00:12:12 &  -33:13:39 &  1014 $\pm$ 233 &    644 $\pm$ 87.0 &  22.0 &   812 $\pm$ 27 \\
      NGP &   PCCS1 857 G058.53+82.57 &  13:22:26 &  +30:07:28 &   827 $\pm$ 197 &    554 $\pm$ 89.0 &  22.0 &   910 $\pm$ 30 \\
     ADFS &  PLCKERC857 G261.89-40.69 &  04:40:40 &  -53:44:02 &   795 $\pm$ 134 &  1304 $\pm$ 104.0 &  22.0 &   980 $\pm$ 11 \\
    HELMS &   PCCS1 857 G126.98-59.24 &  00:59:45 &  +03:33:29 &   383 $\pm$ 234 &   648 $\pm$ 304.0 &  21.0 &   685 $\pm$ 29 \\
      NGP &  PLCKERC857 G077.25+80.72 &  13:23:12 &  +33:23:12 &   1065 $\pm$ 97 &    500 $\pm$ 89.0 &  21.0 &   679 $\pm$ 29 \\
      NGP &   PCCS2 857 G029.94+79.79 &  13:36:55 &  +26:08:21 &   467 $\pm$ 258 &    380 $\pm$ 86.0 &  21.0 &   754 $\pm$ 29 \\
      SGP &   PCCS2 857 G013.36-62.85 &  22:48:24 &  -32:47:53 &   175 $\pm$ 281 &    600 $\pm$ 92.0 &  20.0 &   761 $\pm$ 30 \\
      SGP &  PLCKERC857 G222.32-80.00 &  01:36:18 &  -28:18:43 &   972 $\pm$ 128 &    454 $\pm$ 89.0 &  20.0 &   717 $\pm$ 30 \\
      SGP &   PCCS1 857 G018.31-71.34 &  23:27:28 &  -30:15:23 &   749 $\pm$ 360 &    419 $\pm$ 84.0 &  20.0 &   712 $\pm$ 27 \\
  XMM-LSS &   PCCS2 857 G170.56-57.15 &  02:26:06 &  -03:18:49 &   693 $\pm$ 211 &    962 $\pm$ 93.0 &  20.0 &   700 $\pm$ 11 \\
      NGP &  PLCKERC857 G062.48+78.89 &  13:37:06 &  +32:08:31 &   814 $\pm$ 109 &    573 $\pm$ 90.0 &  19.0 &   738 $\pm$ 28 \\
      NGP &  PLCKERC857 G028.53+83.67 &  13:19:37 &  +26:28:04 &  1301 $\pm$ 166 &    678 $\pm$ 87.0 &  19.0 &   743 $\pm$ 25 \\
\bottomrule
\end{tabular}


==> Paper_revised_postreferee (copy)/Introduction/Table_Surveysizes <==
\begin{tabular}{lllll}
\toprule
 & & \multicolumn{2}{c}{\textit{Planck} source count} \\
\toprule
Field &  Area [deg$^2$] & 857GHz & 545GHz \\
\midrule
NGP     &     170.0 & 82 & 21 \\
SGP     &     285.0 & 91 & 35  \\
GAMA09 &    53.4 & 26 & 13 \\
GAMA12    &         53.6 & 15 & 5 \\
GAMA15             &         54.6 & 16 & 13\\
ADFS             &    7.5 & 3 & 3 \\
BOOTES            &    11.3 & 11 & 2 \\
CDFS-SWIRE           &    10.9 & 5 & 1\\
COSMOS HerMES         &       4.4 & 2 & 1 \\
EGS HerMES          &     2.7 & 1 & 0 \\
ELAIS N1 SWIRE          &     12.3 & 6 & 2 \\
ELAIS S1 SWIRE       &    7.9 & 2 & 0 \\
FLS       &      6.7 & 5 & 3 \\
GOODS-North & 13.5 & 0 & 0 \\
LOCKMAN-SWIRE            &      16.1 & 6 & 3 \\
XMM-LSS-SWIRE            &    18.9 & 4 & 2 \\
HERS          &     79.0 & 38 & 14 \\
\midrule
\textbf{Total} & 808.4 & 313 & 118 \\
\bottomrule
\end{tabular}


==> Paper_revised_postreferee (copy)/SelectionMethods/Table_SourceIdentifier <==
\begin{tabular}{l|ll}
\toprule
Detected in catagloue  & 857Ghz & 545Ghz \\
\midrule
ERCSC only & 52 & 14 \\
PCCS1 only & 68 & 39 \\
PCCS2 only & 28 & 4 \\
ERCSC-PCCS1 & 23 & 4 \\
ERCSC-PCCS2& 4 & 0 \\
PCCS1-PCCS2& 55 & 24 \\
All Three & 81 & 32 \\
\midrule
\textbf{Total} & 311 & 117 \\
\bottomrule
\end{tabular}


==> SelectionMethods/Table_SourceIdentifier <==
\begin{tabular}{l|ll}
\toprule
Detected in catagloue  & 857Ghz & 545Ghz \\
\midrule
ERCSC only & 52 & 14 \\
PCCS1 only & 68 & 39 \\
PCCS2 only & 28 & 4 \\
ERCSC-PCCS1 & 23 & 4 \\
ERCSC-PCCS2& 4 & 0 \\
PCCS1-PCCS2& 55 & 24 \\
All Three & 81 & 32 \\
\midrule
\textbf{Total} & 311 & 117 \\
\bottomrule
\end{tabular}

